Byzantine Consensus is \Theta(n^2): The Dolev-Reischuk Bound is Tight even in Partial Synchrony! [Extended Version]

The Dolev-Reischuk bound says that any deterministic Byzantine consensus protocol has (at least) quadratic communication complexity in the worst case. While it has been shown that the bound is tight in synchronous environments, it is still unknown whether a consensus protocol with quadratic communication complexity can be obtained in partial synchrony. Until now, the most efficient known solutions for Byzantine consensus in partially synchronous settings had cubic communication complexity (e.g., HotStuff, binary DBFT). This paper closes the existing gap by introducing SQuad, a partially synchronous Byzantine consensus protocol with quadratic worst-case communication complexity. In addition, SQuad is optimally-resilient and achieves linear worst-case latency complexity. The key technical contribution underlying SQuad lies in the way we solve view synchronization, the problem of bringing all correct processes to the same view with a correct leader for sufficiently long. Concretely, we present RareSync, a view synchronization protocol with quadratic communication complexity and linear latency complexity, which we utilize in order to obtain SQuad.

==> depricated/introduction.tex <==
\section{Introduction} \label{section:introduction}

Byzantine consensus~\cite{LamportSP82} is a fundamental problem of distributed computing.
Intuitively, Byzantine consensus enables processes to agree on a common value despite arbitrary (Byzantine) failures. % Introduce a few sentences for motivation on Consensus protocols (cryptocurrencies, etc.)
Formally, each process is either correct or faulty; correct processes follow a prescribed protocol, whereas faulty processes (up to $f$) can arbitrarily deviate from it.
Each correct process initially \emph{proposes} a value, and should eventually \emph{decide} a value.
The following properties are guaranteed:
\begin{compactitem}
    \item \emph{Validity:} If all processes are correct, then a value decided by a process was previously proposed.
    
    \item \emph{Agreement:} No two correct processes decide different values.
    
    \item \emph{Termination:} All correct processes eventually decide.
\end{compactitem}

The celebrated Dolev-Reischuk bound~\cite{DolevR82} shows that any deterministic solution of the Byzantine consensus problem requires correct processes to exchange (at least) a quadratic number of bits of information.
Recently, Momose and Ren~\cite{MomoseR21} have illustrated that the bound is tight in synchronous environments.
However, it is still unknown whether the bound is tight in partially synchronous environments~\cite{DworkLS88} in which the network becomes synchronous only after some unknown Global Stabilization Time ($\mathit{GST}$).\footnote{No deterministic protocol solves Byzantine consensus in a completely asynchronous environment~\cite{FischerLP83}.}
The most efficient known solutions in partially synchronous environments have cubic communication complexity (e.g., HotStuff~\cite{YinMRGA19}, binary DBFT~\cite{CrainGLR18}).

This paper closes the existing gap by introducing \name, an optimally-resilient partially synchronous Byzantine consensus protocol optimized for the worst-case communication complexity.
\name achieves quadratic communication complexity while tolerating up to a third of Byzantine failures (i.e., $n = 3f + 1$~\cite{LamportSP82}).

\medskip
\noindent \textbf{State-of-the-art.}
State-of-the-art ``leader-based'' consensus protocols~\cite{YinMRGA19, diembft,CastroL99,tendermint} operate in \emph{views}, each with a designated leader whose responsibility is to drive the system towards a decision.
If a process does not decide in a view, it moves to the next view with a different leader and tries again.
Once all correct processes overlap in the same view with a correct leader for sufficiently long, a decision is reached.
Unfortunately, ensuring such an overlap is non-trivial; for example, processes can start executing the protocol at different times or their local clocks may drift before $\mathit{GST}$, thus placing them in views which are arbitrarily far apart.

Roughly speaking, these protocols contain two independent modules:
\begin{compactenum}
    \item View \core: The core of the protocol, responsible for executing the protocol logic of each view.
    
    \item View synchronizer: Auxiliary to the view core, responsible for ``moving'' processes to new views with the goal of ensuring a sufficiently long overlap to allow the view core to decide.
\end{compactenum}
Immediately after $\mathit{GST}$, the view synchronizer brings all correct processes together to the view of the most advanced correct process and keeps them in that view for sufficiently long.
At this point, if the leader of the view is correct, the processes decide.
Otherwise, they ``synchronously'' transit to the next view with a different leader and try again.
In summary, the communication complexity of such protocols can be approximated by $\text{\#}V \cdot C_V + S$, where:
\begin{compactitem}
    \item $\text{\#}V$ denotes the number of views the view core executes after $\mathit{GST}$, 
    
    \item $C_V$ denotes the communication complexity of the view core executing a \emph{single} view, and
    
    \item $S$ denotes the communication complexity of the view synchronizer from $\mathit{GST}$ until every correct process decides.
\end{compactitem}

Given that the adversary can corrupt up to $f$ processes, the number of views through which correct processes must transit before reaching a correct leader is, in the worst case, $\text{\#}V = \Omega(f) = \Omega(n)$.
In fact, PBFT~\cite{CastroL99} and HotStuff~\cite{YinMRGA19} show that $\text{\#}V = \Theta(f) = \Theta(n)$.
Furthermore, HotStuff achieves $C_V = O(n)$ via the ``leader-to-all, all-to-leader'' communication pattern it employs in each view.
Unfortunately, $S = \text{\#}V \cdot O(n^2) = O(n^3)$ in HotStuff due to the ``all-to-all'' communication pattern exploited by its view synchronizer in \emph{every} view.\footnote{While HotStuff~\cite{YinMRGA19} does not explicitly state how the view synchronization is achieved, we have that $S = O(n^3)$ in Diem BFT~\cite{diembft}, which is a mature implementation of the HotStuff protocol.} 
Thus, $S = O(n^3)$ dominates the communication complexity of HotStuff, preventing it from matching the Dolev-Reischuk lower bound.
% thus dominating the communication complexity and preventing it from matching the Dolev-Reischuk lower bound.
If we could design a consensus algorithm for which $S \leq O(n^2)$ while preserving $\text{\#}V = O(n)$ and $C_V = O(n)$, we would obtain a Byzantine consensus protocol with optimal communication complexity.
The question is if such a view synchronizer exists.

\medskip
\noindent \textbf{View doubling synchronizer.} % Rename to (choices): Strawman, Special considerations, Latency
Aside from communication complexity, it is also necessary to take into account the latency of such algorithms.
For example, one simple solution to the synchronization problem is the well-known \emph{view doubling synchronizer}~\cite{NBMS20, CastroL99}.
In the view doubling synchronizer, processes advance sequentially through each view solely by relying on their local clock.
Specifically, each view is associated with a maximum duration; after a process reaches this duration, the process moves to the next view and doubles the maximum duration.
This exponential increase in time allows delayed processes to eventually catch up to the view of the most advanced process without any communication (i.e., $S = 0$).

However, the problem with this approach is that the time needed to achieve synchronization is unbounded~\cite{NBMS20}. 
Essentially, since the maximum duration of a view can become arbitrarily large before GST, the latency of synchronization after GST is similarly unbounded.
The ``view-doubling'' variant of HotStuff employing this simple synchronizer, while indeed achieving optimal communication complexity, has unbounded latency complexity. 
The real question is if there exists a \emph{bounded-latency} view synchronizer with quadratic worst-case communication complexity.

\medskip
\noindent \textbf{\rare.}
Our main contribution is \rare, a view synchronizer that achieves synchronization within $O(f)$ time and has $O(n^2)$ worst-case communication complexity.
\jovan{\rare strikes a balance between two approaches. The first approach has all-to-all communication in every view, leading to cubic complexity overall. The other approach does not have any communication, leading to unbounded latency. \rare is a hybrid between the two achieving best of both worlds.}
The main issue with existing view synchronizers is that they keep processes synchronized at each view solely by relying on ``all-to-all'' communications.
This induces an average-per-view communication cost of $O(n^2)$.
Given that, in the worst case, processes must transit through $f = \Omega(n)$ views, each with a quadratic synchonizer-related communication cost, ``leader-based'' consensus protocols utilizing existing view synchronizers have (at least) cubic communication complexity.

In contrast to existing approaches, \rare minimizes the usage of ``all-to-all'' communications.
Namely, \rare groups views into \emph{epochs}; each epoch contains $f + 1$ sequential views.
Instead of performing ``all-to-all'' communication in each view, \rare performs a \emph{single} ``all-to-all'' communication step per epoch.
Specifically, \emph{only} at the beginning of each epoch, do all correct processes communicate to allow slow processes to ``catch up''.
Once a process has entered an epoch, it relies solely on its local clock (without any communication) to move forward to the next view within the epoch.
In summary, \rare uses communication to synchronize processes, while relying on local timeouts (and not communication!) to keep them synchronized.

\medskip
\noindent \textbf{\name.}
The second contribution of our work is \name, an optimally-resilient partially synchronous Byzantine consensus protocol with optimal worst-case communication complexity.
The view core module of \name is the same as in HotStuff, thus ensuring $C_V = O(n)$ in \name.
As its view synchronizer, \name uses \rare, which ensures $S = O(n^2)$.
Following the previously introduced complexity formula, \name achieves $O(n) \cdot O(n) + O(n^2) = O(n^2)$ communication complexity.
Combined with the Dolev-Reischuk lower bound, this shows that the communication complexity of Byzantine consensus is $\Theta(n^2)$.

\medskip
\noindent \textbf{Roadmap.}


\iffalse
******************

If we could limit the communication complexity of HotStuff's view synchronizer to $O(n^2)$, we would obtain a consensus protocol with quadratic communication complexity.


The only missing ingredient to achieve quadratic communication complexity is $S$.
Indeed, if we devise a view synchronizer $\mathcal{V}$ that ensures $S = O(n^2)$, we would be able to obtain a quadratic communication complexity by employing $\mathcal{V}$ as the view synchronizer of the HotStuff protocol. 


Most deterministic leader-based BFT consensus algorithms proceed in rounds.
In each round, processes collectively execute a \emph{round} sub-routine: one process acts as leader, the remaining processes act as followers and together they attempt to agree on a value.
If ``the stars align'', a value is agreed upon in this round and is then decided by every correct process.
This happens when i) the leader is correct and ii) all correct processes \emph{synchronously} execute the round for a sufficiently long period of time $T$, which depends on the specific algorithm being used.
Intuitively, this \emph{round} sub-routine can be regarded as its own abstraction solving a simpler version of the problem, with a weaker termination guarantee, i.e.:

\begin{compactitem}
    \item \emph{Good Case Termination:} If ``the stars align'', then all correct processes decide.
\end{compactitem}


As a majority of ``leader-based'' consensus protocols, an execution of \name unfolds in \emph{views}, each with a designated leader whose responsibility is to drive the system towards a decision.
The safety of \name is guaranteed always: if any correct process decides a value in a view, no correct process will decide a different value in any future view.
On the other hand, the liveness of \name is ensured only if all correct processes overlap in a same view with a correct leader for long enough.
Ensuring such an overlap is the responsibility of \name's \emph{view synchronizer} -- \rare.






Views are grouped into \emph{epochs}; each epoch contains $f + 1$ sequential views.
The safety of \name is guaranteed always, whereas its liveness relies on the fact that correct processes overlap in a same view with a correct leader for long enough to reach a decision.
Such an overlap is achieved through \emph{view synchronization}.

\rare is \name's view synchronizer and it operates with quadratic communication cost per epoch.


The intuition behind \rare is simple: processes communicate \emph{once} to synchronize at the beginning of each epoch and remain synchronized throughout the entire epoch only by ``listening'' to local clocks (without any communication).
Specifically, at the beginning of each epoch, processes communicate in the ``all-to-all'' manner to synchronize; then, processes transit to new rounds of the same epoch only by means of local timeouts.
Therefore, \rare wastes quadratic communication per epoch.



\rare is simple: 
\begin{compactitem}
    \item In order to synchronize to the first round of an epoch after $\mathit{GST}$, processes communicate in the ``all-to-all'' manner.
    
    \item 
\end{compactitem}

\rare exploits one ``all-to-all'' communication pattern per epoch

\rare is 

\rare operates with quadratic communication and linear latency in the worst case.


Liveness of \name is guaranteed if all correct processes overlap in a same view with a correct leader for long enough to reach a decision.
Ensuring that such an overlap eventually happens is a responsibility of \rare, the \name's \emph{view synchronizer}.



Ensuring that such an overlap eventually happens is a responsibility of \rare, a \emph{view synchronizer} exp


Essentially, \name optimizes its \emph{view synchronizer} sub-routine, a sub-routine ensuring that eventually all correct processes overlap in a same view with a correct leader for sufficiently long.
Specifically, \name utilizes \rare, a view synchronizer that operates with quadratic communication and linear latency.
\rare exploits a simple strategy: it requires 






To devise \name, we focused on the \emph{view synchronization} problem, a problem of bringing all correct processes to a view with a correct leader for long enough to reach a decision.
Specifically, most ``leader-based'' consensus algorithms un

Specifically, we observe that a view synchronizer with (1) quadratic communication cost, and (2) linear latency cost allows for a Byzantine consensus protocol with quadratic communication and linear latency cost.


To devise \name, we focused on the \emph{view synchronization} problem, a problem of bringing all correct processes to the same view with a correct leader for sufficiently long.
While studying the state-of-the-art ``leader-based'' consensus protocols, we noticed that quadratic communication complexity for view synchronization is paid \emph{every} view.
Given that, in the worst case, $f + 1 = O(n)$ views must be executed after $\mathit{GST}$, the communication complexity of the view synchronization complexity is $O(n) \cdot O(n^2) = O(n^3)$.

We introduce \rare, a view synchronizer whose communication complexity is $O(n^2)$, and whose latency complexity is $O(n)$.
The crucial idea behind \rare is to ensure that processes communicate in the ``all-to-all'' fashion only \emph{once} per $f + 1$ rounds.
Such a communication brings them together, while their local timeouts keep them together for the next $f$ rounds (after $\mathit{GST}$).
\fi

==> depricated/intuiton.tex <==
In this section, we demonstrate that optimal view synchronization allows for an optimal Byzantine consensus.
Specifically, we formally define the \emph{view executor} and \emph{view synchronization} distributed abstractions.
Next, we show that a simple composition of these abstractions solves the Byzantine consensus problem.
Finally, we show that the complexity of the aforementioned composition depends (primarily) on the complexity of view synchronization.
% Next, we give a simple Byzantine consensus protocol built upon these two abstractions.
% Finally, we show that the complexity of the aforementioned consensus protocol depends (primarily) on the complexity of view synchronization.

% In this section, we demonstrate that view synchronization represents a promising ``optimization point'' in Byzantine consensus protocols.
% Specifically, we formally define the \emph{view} component and the \emph{view synchronization} (or simply synchronization) component.
% Furthermore, we give a composition of these two components solving the Byzantine consensus problem and show how the complexity of the composition depends on the complexity of the building components.


% Specifically, we present an algorithmic skeleton of traditional ``leader-based'' Byzantine consensus protocols that consists of two components: view, and view synchronization.
% Moreover, we prove that the communication (resp., latency) complexity of consensus protocols following the aforementioned skeleton is dominated by the communication (resp., latency) complexity of the view synchronization component, thus illustrating that an optimized view synchronization allows for an optimal Byzantine consensus protocol.

% Executions of most ``leader-based'' consensus protocols~\cite{yin2019hotstuff,castro1999practical,buchman2018latest,gueta2019sbft} unfold in \emph{views}.
% Each view has a designated \emph{leader} that, under preferable conditions (e.g., timely communication), ensures that all processes decide.
% Transition between views is a responsibility of the \emph{view synchronization} (or simply ``synchronization) module that notifies processes when to transit to a new view.
% Hence, we identify view and synchronization as the components constructing a traditional ``leader-based'' Byzantine consensus protocol.
% Before we formally introduce these two components, we introduce some preliminaries.

\medskip 
\noindent \textbf{Preliminaries.}
We denote by $\mathsf{Views} = \{1, 2, ...\}$ the set of \emph{views}.
For each view $v \in \mathsf{Views}$, we define $\mathsf{leader}(v)$ as a process that is the \emph{leader} of the view $v$.

\subsection{View Executor}

The view executor abstraction is associated with a predefined constant $c_e \in \mathbb{N}$.
At each process, view executor is initialized with a value $\mathit{v} \in \mathsf{Values}$; if view executor is initialized with a value $v$ at a correct process, we say that the process proposes $v$.
% The view module is initialized with a value $\mathit{proposal} \in \mathsf{Values}$.
Furthermore, the view executor abstraction provides the following interface:
\begin{compactitem}
    \item Request $\mathsf{start}(v \in \mathsf{Views})$: a process starts executing view $v$.
    This request can be invoked multiple times.
    
    \item Indication $\mathsf{pre\_decide}(\mathit{value} \in \mathsf{Values})$:
    a process pre-decides $\mathit{value}$.
\end{compactitem}
We say that a correct process \emph{executes view $v \in \mathsf{Views}$} between the time $t$ at which the process invokes $\mathsf{start}(v)$ and the time at which the process invokes $\mathsf{start}(v' \neq v)$ after time $t$.
If the process never invokes $\mathsf{start}(v' \neq v)$ after time $t$, then the process executes the view $v$ from time $t$ onward.

Finally, the view executor abstraction ensures the following guarantees:
\begin{compactitem}
    \item \emph{Agreement:} If a correct process pre-decides $v$ and another correct process pre-decides $v'$, then $v = v'$.
    
    \item \emph{Integrity:} A correct process pre-decides at most once.
    
    \item \emph{Termination:} Let there exist a view $v \in \mathsf{Views}$ and a time period $\mathcal{T} = [t_1, t_2]$ such that (1) $t_2 - t_1 \geq c_e \cdot \delta$, (2) $t_1 \geq \mathit{GST}$, (3) all correct processes execute $v$ during $\mathcal{T}$, and (4) $\mathsf{leader}(v)$ is correct.
    Then, all correct processes pre-decide.
\end{compactitem}

\subsection{View Synchronization}\label{subsection:view_synchronization}

Similarly to the view executor abstraction, the view synchronization abstraction is associated with a predefined constant $c_s \in \mathbb{N}$.
It provides the following interface:
\begin{compactitem}
    \item Indication $\mathsf{advance}(v \in \mathsf{Views})$: The process advances to a view $v$.
\end{compactitem}
We say that a correct process \emph{is in view} $v \in \mathsf{Views}$ between the time $t$ at which the process receives the $\mathsf{advance}(v)$ indication and the time at which the process receives the $\mathsf{advance}(v' \neq v)$ indication after time $t$.
If the process never receives $\mathsf{advance}(v' \neq v)$, then the process remains in the view $v$ from time $t$ onward.

Next, we define a synchronization time as a time at which all correct processes are in the same view with a correct leader for sufficiently long.
The similar definition can be found in~\cite{NK20}.

\begin{definition} [Synchronization Time]
Time $t_s$ is a \emph{synchronization time} if (1) all correct processes are in the same view $v$ from time $t_s$ to (at least) time $t_s + c_s\cdot\delta$, and (2) $\mathsf{leader}(v)$ is correct.
\end{definition}
Finally, view synchronization satisfies the \emph{eventual synchronization} property which states that there exists a synchronization time after $\mathit{GST}$.

\subsection{View Executor + View Synchronization = Consensus}

\medskip
\noindent \textbf{Composition.}
Finally, \Cref{algorithm:composition} shows how the view and the synchronization components collaborate in order to solve Byzantine consensus.

\begin{algorithm}
\caption{View + Synchronization = Byzantine Consensus}
\label{algorithm:composition}
\begin{multicols}{2}
\begin{algorithmic} [1]
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\texttt{View.}\mathsf{init(}\mathit{proposal}\mathsf{)}$

\medskip
\State \textbf{upon} $\texttt{Synchronization.}\mathsf{advance(}v\mathsf{)}$:
\State \hskip2em $\texttt{View.}\mathsf{start(}v\mathsf{)}$

\columnbreak
\medskip
\State \textbf{upon} $\texttt{View.}\mathsf{decide(}v\mathsf{)}$:
\State \hskip2em \textbf{trigger} $\mathsf{decide(}v\mathsf{)}$
\end{algorithmic}
\end{multicols}
\end{algorithm} 

We prove the correctness of \Cref{algorithm:composition}.

\begin{theorem}
\Cref{algorithm:composition} solves the Byzantine consensus problem.
\end{theorem}
\begin{proof}
The agreement property of Byzantine consensus follows directly from the agreement property of the view module.
By the eventual view synchronization property of the view synchronization component, there exists a synchronization point after $\mathit{GST}$.
Therefore, the precondition of the termination property of the view component holds, which implies that all correct processes decide.
The theorem holds.
\end{proof}

Finally, we prove the complexity of \Cref{algorithm:composition}.

\begin{theorem}
The communication complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{com\_per\_view} + \mathit{sync\_com}$.
The latency complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{latency\_per\_view} + \mathit{sync\_latency}$.
\end{theorem}

==> depricated/quadstuff.tex <==
\section{\name}

This section presents \name.



First, we give the utility functions (\Cref{algorithm:utilities}) and variables and constants (\Cref{algorithm:variable_constants}) of processes.
The \name protocol is divided into two parts:
\begin{compactenum}
    \item Round protocol (\cref{algorithm:round_1,algorithm:round_2}): An execution of \name unfolds in rounds (like many other ``PBFT-like'' protocols).
    This part of the \name protocol presents the pseudocode of a round.
    
    \item Wrapper protocol (\Cref{algorithm:wrapper}): This part of \name describes the ``wrapper'' of the round protocol.
    Roughly speaking, it includes (1) the round synchronization logic, and (2) the decision making logic.
\end{compactenum}
In the rest of the paper, we refer to \cref{algorithm:round_1,algorithm:round_2} as the ``round protocol'', whereas we refer to \Cref{algorithm:wrapper} as the ``wrapper protocol''.

\begin{algorithm}
\caption{Utilities (for process $P_i$)}
\label{algorithm:utilities}
\begin{algorithmic} [1]
\State \textbf{function} \texttt{msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{round}$\texttt{)}:
\State \hskip2em $m.\mathit{type} \gets \mathit{type}$; $m.\mathit{value} \gets \mathit{value}$; $m.\mathit{qc} \gets \mathit{qc}$; $m.\mathit{epoch} \gets \mathit{epoch}$; $m.\mathit{round} \gets \mathit{round}$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{vote\_msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{round}$\texttt{)}:
\State \hskip2em $m \gets \texttt{msg(}\mathit{type}, \mathit{value}, \mathit{qc}, \mathit{epoch}, \mathit{round}\texttt{)}$
\State \hskip2em $m.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m.\mathit{type}, m.\mathit{value}, m.\mathit{epoch}, m.\mathit{round}])$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{qc(Set(Vote\_Message)} $M$\texttt{)}: \Comment{All the messages from $M$ have the same type, value, epoch and round}
\State \hskip2em $\mathit{qc}.\mathit{type} \gets m.\mathit{type}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{value} \gets m.\mathit{value}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{epoch} \gets m.\mathit{epoch}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{round} \gets m.\mathit{round}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{sig} \gets \mathit{Combine}(\{\mathit{partial\_sig} \,|\, \exists m \in M: m.\mathit{partial\_sig} = \mathit{partial\_sig}\})$
\State \hskip2em \textbf{return} $\mathit{qc}$

\medskip
\State \textbf{function} \texttt{matching\_msg(Message} $m$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{round}$\texttt{)}:
\State \hskip2em \textbf{return} $m.\mathit{type} = \mathit{type}$ and $m.\mathit{epoch} = \mathit{epoch}$ and $m.\mathit{round} = \mathit{round}$

\medskip
\State \textbf{function} \texttt{matching\_qc(Quorum\_Certificate} $\mathit{qc}$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{round}$\texttt{)}:
\State \hskip2em \textbf{return} $\mathit{qc}.\mathit{type} = \mathit{type}$ and $\mathit{qc}.\mathit{epoch} = \mathit{epoch}$ and $\mathit{qc}.\mathit{round} = \mathit{round}$

\medskip
\State \textbf{function} \texttt{global\_round(Quorum\_Certificate} $\mathit{qc}$\texttt{)}:
\State \hskip2em \textbf{return} $(\mathit{qc}.\mathit{epoch} - 1) \cdot (f + 1) + \mathit{qc}.\mathit{round}$
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}
\caption{Variables and constants (for process $P_i$)}
\label{algorithm:variable_constants}
\begin{algorithmic} [1]
\State \textbf{Variables:}
\State \texttt{Integer} $\mathit{epoch} \gets 1$
\State \texttt{Integer} $\mathit{round} \gets 1$
\State \texttt{Quorum\_Certificate} $\mathit{prepareQC} \gets \bot$
\State \texttt{Quorum\_Certificate} $\mathit{lockedQC} \gets \bot$
\State \texttt{Timer} $\mathit{round\_timer}$
\State \texttt{Timer} $\mathit{sync\_timer}$
\State \texttt{Signature} $\mathit{epoch\_over\_sig} \gets \bot$

\medskip
\State \textbf{Constants:}
\State \texttt{Time} $\mathit{round\_duration} = 10\delta$
\end{algorithmic}
\end{algorithm} 

\begin{algorithm} 
\caption{\name (Round protocol): Pseudocode for process $P_i$}
\label{algorithm:round_1}
\begin{algorithmic} [1]
\State \textbf{upon} \texttt{start\_round}:
\State \hskip2em start reacting to events of the round protocol
\State \hskip2em $\mathit{round\_timer}$\texttt{.measure($\mathit{round\_duration}$)} \label{line:round_timer_measure}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{View-Change phase}
\State \hskip2em \texttt{send} \texttt{msg(}\textsc{view-change}, $\bot$, $\mathit{prepareQC}$, $\mathit{epoch}$, $\mathit{round}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Prepare phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ \textsc{view-change} messages: $M \gets \{m \,|\, \texttt{matching\_msg(}m, \textsc{view-change}, \mathit{epoch}, \mathit{round}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{highQC} \gets \mathit{qc}$ with the highest $\texttt{global\_round(}\mathit{qc}\texttt{)}$ in $M$
\State \hskip4em \texttt{Integer} $\mathit{proposal} \gets \mathit{highQC}.\mathit{value}$
\State \hskip4em \textbf{if} $\mathit{proposal} = \bot$:
\State \hskip6em $\mathit{proposal} \gets \mathit{proposal}_i$ \Comment{$\mathit{proposal}_i$ denotes the proposal of $P_i$}
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{prepare}, $\mathit{proposal}$, $\mathit{highQC}$, $\mathit{epoch}$, $\mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_msg(}$m$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{round}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}
\State \hskip4em \textbf{if} $m.\mathit{qc}.\mathit{value} = m.\mathit{value}$ and ($\mathit{lockedQC}.\mathit{value} = m.\mathit{value}$ or $\texttt{global\_round(}\mathit{qc}\texttt{)} > \mathit{lockedQC}.\mathit{round}$):
\State \hskip6em \texttt{send} \texttt{vote\_msg(}\textsc{prepare}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{round}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Precommit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{prepare}, \mathit{epoch}, \mathit{round}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{precommit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{round}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}
\State \hskip4em $\mathit{prepareQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{precommit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{round}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Commit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{precommit}, \mathit{epoch}, \mathit{round}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{commit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{precommit}, $\mathit{epoch}$, $\mathit{round}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}
\State \hskip4em $\mathit{lockedQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{commit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{round}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Decide phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{commit}, \mathit{epoch}, \mathit{round}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{decide}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{round}$\texttt{)} \label{line:broadcast_decide_message}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{commit}, $\mathit{epoch}$, $\mathit{round}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{round}$\texttt{)}
% \State \hskip4em $\mathit{round\_timer}$\texttt{.cancel()} \Comment{timer's expiration event is canceled}
\State \hskip4em \texttt{finalize\_decision(}$m.\mathit{qc}$\texttt{)}
\algstore{alg:example}
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}
\caption{\name (Round): Pseudocode for process $P_i$}
\label{algorithm:round_2}
\begin{algorithmic} [1]
\algrestore{alg:example}
\State \textbf{upon} \texttt{terminate\_round}:
\State \hskip2em $\mathit{round\_timer}$\texttt{.cancel()} \Comment{timer's expiration event is canceled}
\State \hskip2em stop reacting to events of the round protocol

\medskip
\LineComment{This rule is activated only after all received messages of the round protocol have been processed} \label{line:rule}
\State \textbf{upon} $\mathit{round\_timer}$ \textbf{expires}: \label{line:upon_round_timer}
\State \hskip2em \textbf{trigger} \texttt{round\_expired}
\State \hskip2em stop reacting to events of the round protocol
\end{algorithmic}
\end{algorithm} 


\begin{algorithm}
\caption{\name (Wrapper): Pseudocode for process $P_i$}
\label{algorithm:wrapper}
\begin{algorithmic} [1]

\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm} \label{line:start_algorithm}
\State \hskip2em start epoch $1$ \Comment{enter epoch $1$} \label{line:start_epoch_1}
\State \hskip2em \textbf{trigger} \texttt{start\_round} \label{line:start_round_1} \Comment{start the first round of the first epoch}

\medskip

\State \textbf{function} \texttt{finalize\_decision(Quorum\_Certificate} $\mathit{qc}$\texttt{)}: \label{line:finalize_decision_function}
\State \hskip2em \texttt{broadcast} $\langle \textsc{decision}, \mathit{qc} \rangle$ \Comment{disseminate the quorum certificate} \label{line:broadcast_qc}
\State \hskip2em \textbf{trigger} \texttt{decide(}$\mathit{qc}.\mathit{value}$\texttt{)} \Comment{decision is made} \label{line:decide}
\State \hskip2em stop reacting to all events \label{line:stop_all_events} \Comment{``end'' of the algorithm}

\medskip
\State \textbf{upon} reception of $\langle \textsc{decision}, \texttt{Quorum\_Certificate} \text{ } \mathit{qc} \rangle$:
\State \hskip2em \texttt{finalize\_decision(}$\mathit{qc}$\texttt{)} \label{line:invoke_finalize_decision}

\medskip
\State \textbf{upon} \texttt{round\_expired}: \label{line:rule_round_expired}
\State \hskip2em \textbf{if} $\mathit{round} \neq f + 1$:
\State \hskip4em $\mathit{round} \gets \mathit{round} + 1$
\State \hskip4em \textbf{trigger} \texttt{start\_round} \Comment{start the next round of the current epoch}
\State \hskip2em \textbf{else:}
\State \hskip4em \texttt{broadcast} $\langle \textsc{epoch-over}, \mathit{epoch}, \mathit{ShareSign}_i(\mathit{epoch}) \rangle$ \label{line:broadcast_epoch_over}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ from $2f + 1$ processes such that $e \geq \mathit{epoch}$: \label{line:receive_epoch_over}
\State \hskip2em \textbf{trigger} \texttt{terminate\_round}
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{Combine}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in an } \textsc{epoch-over} \text{ message}\})$
\State \hskip2em $\mathit{epoch} \gets e + 1$ \Comment{enter $\mathit{epoch}$} \label{line:update_epoch_1}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over-complete}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ such that $e \geq \mathit{epoch}$: \label{line:receive_epoch_over_complete}
\State \hskip2em \textbf{trigger} \texttt{terminate\_round}
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{sig}$
\State \hskip2em $\mathit{epoch} \gets e + 1$ \Comment{enter $\mathit{epoch}$} \label{line:update_epoch_2}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)}

\medskip
\State \textbf{upon} $\mathit{sync\_timer}$ \textbf{expires}: \label{line:sync_timer_expires}
\State \hskip2em \texttt{broadcast} $\langle \textsc{epoch-over-complete}, \mathit{epoch} - 1, \mathit{epoch\_over\_sig} \rangle$ \label{line:broadcast_epoch_over_complete}
\State \hskip2em $\mathit{round} \gets 1$
\State \hskip2em start $\mathit{epoch}$ \label{line:start_epoch}
\State \hskip2em \textbf{trigger} \texttt{start\_round} \label{line:start_round_2} \Comment{start the first round of the next epoch}
\end{algorithmic}
\end{algorithm}

\subsection{Proof of Correctness}
We now prove the correctness of \name.
In order to do so, we need to prove that \name (\cref{algorithm:round_1,algorithm:round_2,algorithm:wrapper}) satisfies validity, termination and agreement.
Whenever we reference lines of the pseudocode in the rest of the subsection, we refer to the lines of \Cref{algorithm:wrapper} (if not explicitly stated otherwise).

\paragraph{Termination}
First, we prove that all correct processes decide if a correct process decides.

\begin{lemma} \label{lemma:one_decides_all_decide}
Let a correct process decide a value.
Then, every correct process eventually decides a value.
\end{lemma}
\begin{proof}
Let $P_i$ be the correct process that decides.
Before deciding (line~\ref{line:decide}), $P_i$ disseminates the obtained quorum certificate (line~\ref{line:broadcast_qc}).
Eventually, every correct process receives the broadcast \textsc{decision} message, enters the \texttt{finalize\_decision} function (line~\ref{line:invoke_finalize_decision}) and decides (line~\ref{line:decide}).
\end{proof}

% We say that a correct process $P_i$ \emph{enters} an epoch $e$ (at time $t$) if and only if $P_i$ sets its $\mathit{epoch}$ variable to $e$ (at time $t$).
% Observe that $P_i$ updates its $\mathit{epoch}$ variable at the following places: (1) line~\ref{line:start_algorithm} (when $P_i$ starts executing the algorithm), (2) line~\ref{line:update_epoch_1}, and (3) line~\ref{line:update_epoch_2}.

A correct process $P_i$ \emph{starts} an epoch $e$ (at time $t$) if and only if $P_i$ executes (1) line~\ref{line:start_epoch_1} (at time $t$) in the case of $e = 1$, or (2) line~\ref{line:start_epoch} with $\mathit{epoch} = e$ (at time $t$) in the case of $e > 1$.
The next lemma shows that, if a correct process sends an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}), then the process has previously started $e$.

\begin{lemma} \label{lemma:epoch_over_previously_started}
Let a correct process $P_i$ broadcast an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}) at some time $t$.
Then, $P_i$ has started $e$ at some time $t' < t$.
\end{lemma}
\begin{proof}
At the moment of broadcasting the message, the following holds: (1) $\mathit{epoch} = e$ at $P_i$, and (2) $\mathit{round} = f + 1$ at $P_i$.
Therefore, all $f + 1$ rounds of the epoch $e$ have expired (otherwise, $P_i$ would have decided at line~\ref{line:decide} and stopped executing the protocol at line~\ref{line:stop_all_events}).
When the first (out of the aforementioned $f + 1$) round started (at line~\ref{line:start_round_1} or at line~\ref{line:start_round_2}), the epoch $e$ has already started (by line~\ref{line:start_epoch_1} of line~\ref{line:start_epoch}).
Moreover, the epoch $e$ has started before the broadcasting of the message since, for each round of the epoch, $\mathit{round\_timer}$ measures $\mathit{round\_duration}$ time (line~\ref{line:round_timer_measure} of \Cref{algorithm:round_1}) and we assume that the timer expires after some non-zero real time when measuring $\mathit{round\_duration}$ (even before $\mathit{GST}$).
% Therefore, the lemma holds.
\end{proof}

Next, we prove that, if an epoch $e > 1$ is started by a correct process at some time $t$, then epoch $e - 1$ is started by a (potentially different) correct process at some time $t' < t$. 

\begin{lemma} \label{lemma:epoch_previously_started}
Let a correct process start an epoch $e > 1$ at time $t$.
Then, epoch $e - 1$ is started by a correct process at some time $t' < t$.
\end{lemma}
\begin{proof}
Let a correct process $P_i$ start an epoch $e > 1$ at time $t$.
That means that $P_i$ executes line~\ref{line:start_epoch} at time $t$.
Hence, either the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} has been previously activated at process $P_i$.
Therefore, (at least) $f + 1$ correct processes have sent an $\textsc{epoch-over}$ message for $e - 1$ before time $t$.
By \Cref{lemma:epoch_over_previously_started}, these correct processes have started epoch $e - 1$ before sending the \textsc{epoch-over} messages, which concludes the proof.
\end{proof}

The next lemma shows that, if no correct process ever decides, all epochs are eventually started. 
In other words, correct processes keep transiting to new epochs forever.

\begin{lemma} \label{lemma:no_decision_constantly_next_epoch}
Let no correct process ever decide.
Then, every epoch $e \in \mathbb{N}$ is eventually started by a correct process. 
\end{lemma}
\begin{proof}
Epoch $1$ is started by a correct process since every correct process initially starts the epoch (at line~\ref{line:start_epoch_1}, upon executing the \texttt{start} rule).
Therefore, it is left to prove that all epochs greater than $1$ are started by a correct process.

By contradiction, let $e + 1 \in \mathbb{N}$ be the smallest epoch that is never started by a correct process, where $e \geq 1$.
% Given that all correct processes start epoch $1$ once they start executing the protocol (line~\ref{line:start_epoch_1} of \Cref{algorithm:wrapper}), $e > 1$.
\Cref{lemma:epoch_previously_started} shows that no epoch $e' > e + 1$ is ever started by a correct process.

Since epochs greater than $e$ are never started, no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$ (by \Cref{lemma:epoch_over_previously_started}).
Hence, the $\mathit{epoch}$ variable at a correct process cannot contain a value greater than $e + 1$ (see the rules at lines~\ref{line:receive_epoch_over} and~\ref{line:receive_epoch_over_complete}).
Moreover, if the $\mathit{epoch}$ variable at a correct process becomes $e + 1$ (at line~\ref{line:update_epoch_1} or at line~\ref{line:update_epoch_2}), the epoch $e + 1$ is started at that process because (1) \textsc{epoch-over} messages are not sent for epochs greater than $e$, and (2) $\mathit{sync\_timer}$ eventually expires (and the rule at line~\ref{line:sync_timer_expires} activates).
Given that epoch $e + 1$ is never started, no correct process sets its $\mathit{epoch}$ variable to $e + 1$.

Since epoch $e$ is started by a correct process, every correct process eventually sets its $\mathit{epoch}$ variable to $e$: (1) if $e = 1$, that happens as soon as the process starts executing the protocol, or (2) otherwise, every correct process receives an \textsc{epoch-over-complete} message for $e - 1$ and, since the $\mathit{epoch}$ variable cannot have a value greater than $e$, starts $e$ eventually.
Given that (1) no correct process ever decides, and (2) no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$, every correct process receives the \texttt{round\_expired} event for each round of the epoch $e$ (line~\ref{line:rule_round_expired}).
Once that happens, a correct process broadcasts an \textsc{epoch-over} message for the epoch $e$ (line~\ref{line:broadcast_epoch_over}).
Therefore, once a correct process receives the \textsc{epoch-over} messages from all correct processes (and the rule at line~\ref{line:receive_epoch_over} activates), the process updates its $\mathit{epoch}$ variable to $e + 1$ (at line~\ref{line:update_epoch_1}).
Hence, we reach contradiction and the lemma holds.
\end{proof}

The following lemma proves that, if the first correct process to start an epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ before time $t + \mathit{epoch\_duration}$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{round\_duration}$.

\begin{lemma} \label{lemma:no_epoch_over_for_epoch_duration}
Let $t$ be time such that (1) $t \geq \mathit{GST}$, (2) a correct process starts an epoch $e$ at time $t$, and (3) no correct process has started $e$ before time $t$.
Then, no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) before time $t + \mathit{epoch\_duration}$.
\end{lemma}
\begin{proof}
First, no correct process sends an \textsc{epoch-over} message for epoch $e$ before time $t + \mathit{epoch\_duration}$ since the first process to start $e$ does so at time $t \geq \mathit{GST}$.
Therefore, epoch $e + 1$ cannot be started by a correct process by time $t + \mathit{epoch\_duration}$.

By contradiction, suppose that a correct process sends an \textsc{epoch-over} message for an epoch $e' > e$ before time $t + \mathit{epoch\_duration}$.
By \cref{lemma:epoch_over_previously_started,lemma:epoch_previously_started}, epoch $e + 1$ has started before time $t + \mathit{epoch\_duration}$, which is a contradiction with the fact that epoch $e + 1$ does not start by time $t + \mathit{epoch\_duration}$.
Therefore, the lemma stands.
\end{proof}

\Cref{lemma:no_epoch_over_for_epoch_duration} has the following consequence: if the first correct process that starts a new epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process ``leaves'' epoch $e$ by time $t + \mathit{epoch\_duration}$.
Finally, we prove the termination property.

\begin{theorem} [Termination] \label{theorem:termination}
\name satisfies termination.
\end{theorem}
\begin{proof}
We prove the theorem by contradiction.
Let there exist a correct process $P_i$ that never decides.
By \Cref{lemma:one_decides_all_decide}, if a correct process decides, all correct processes (including $P_i$) decide.
Therefore, no correct process decides.


% We separate the proof into two parts:
% \begin{compactenum}
%     \item Let a correct process decide:
%     In this case, all correct processes decide by \Cref{lemma:one_decides_all_decide}.
    
%     \item 
% Let no correct process decide:
Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$.
Let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.
Note that $t_{\mathit{final}}$ exists (by \Cref{lemma:no_decision_constantly_next_epoch}) and $t_{\mathit{final}} > \mathit{GST}$.
Furthermore, \Cref{lemma:no_epoch_over_for_epoch_duration} guarantees that no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e_{\mathit{max}} + 1$ before time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
    
Next, the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} is activated at each correct process by time $t_{\mathit{final}} + \delta$ (recall that $t_{\mathit{final}} > \mathit{GST}$).
Hence, every correct process starts the epoch $e_{\mathit{max}} + 1$ by time $t_{\mathit{final}} + 2\delta$ (due to the $\mathit{sync\_timer}$).
    
Finally, in each round of the epoch $e_{\mathit{max}} + 1$, all correct processes overlap for (at least) $8\delta$ time (given that $\mathit{round\_duration} = 10\delta$ and the biggest ``delay'' between epoch starts is $2\delta$; recall that hardware clocks of processes do not drift after $\mathit{GST}$).
Given that (1) at least one round of the epoch $e_{\mathit{max}} + 1$ has a correct leader (since there are $f + 1$ rounds in $e_{\mathit{max}} + 1$), (2) $8\delta$ time is sufficient for a decision in each round of the epoch $e_{\mathit{max}} + 1$ after the last correct process has started the round (if the round has a correct leader), and (3) the last correct process starts the $(f + 1)$-st round of the epoch by time $t_{\mathit{final}} + f\cdot\mathit{round\_duration} + 2\delta$, every correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
Recall that the rule at line~\ref{line:upon_round_timer} of \Cref{algorithm:round_2} is activated only after all received messages of the round protocol have been processed, which implies that, in a round of the epoch with a correct leader, the rule at line~\ref{line:upon_round_timer} of \Cref{algorithm:round_2} is not activated at a correct process before the process decides\footnote{Observe that, in the case the correct process decides, the rule at line~\ref{line:upon_round_timer} of \Cref{algorithm:round_2} will never get activated because of line~\ref{line:stop_all_events} of \Cref{algorithm:wrapper}.}.
Therefore, we reach a contradiction with the fact that no correct process decides, which implies that termination is satisfied by \name.
% \end{compactenum}
% Termination is satisfied by \name.
\end{proof}

\paragraph{Communication complexity.}
First, we show that each process sends at most $O(n)$ words within any epoch.
Formally, we say that a correct process $P_i$ is \emph{in epoch $e$} between the time $t$ when it starts $e$ and the time $t'$ when it starts some other epoch.
If it does not start some other epoch, $P_i$ remains in $e$ forever.

\begin{lemma} \label{lemma:linear_in_an_epoch}
For any epoch $e$ and any correct process $P_i$, process $P_i$ sends at most $O(n)$ words while being in $e$.
\end{lemma}
\begin{proof}
Let us consider all messages that $P_i$ can send while being in epoch $e$:
\begin{compactitem}
    \item \textsc{decision} messages (sent at line~\ref{line:broadcast_qc}):
    These messages are sent by $P_i$ only once throughout any execution (i.e., line~\ref{line:broadcast_qc} is executed at most once).
    Given that each messages contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{decision} messages while being in epoch $e$.
    
    \item \textsc{epoch-over} messages (sent at line~\ref{line:broadcast_epoch_over}):
    These messages are sent by $P_i$ only once while $P_i$ is in $e$ since the next \texttt{start\_round} event is triggered at line~\ref{line:start_round_2}, which implies that the new epoch has started (line~\ref{line:start_epoch}).
    Given that each \textsc{epoch-over} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over} messages while being in $e$.
    
    \item \textsc{epoch-over-complete} messages (sent at line~\ref{line:broadcast_epoch_over_complete}):
    These messages are sent by $P_i$ only once\footnote{Formally speaking, these messages can be sent twice while $P_i$ is in $e$: the first time when it starts $e$ (recall that local computation takes zero time) and the second time when it starts some other epoch. However, it is important that these messages are sent \emph{constant} number of times in $e$.} while $P_i$ is in $e$ because upon the expiration of the $\mathit{sync\_timer}$ (at line~\ref{line:sync_timer_expires}) $P_i$ starts a new epoch (at line~\ref{line:start_epoch}).
    Given that each \textsc{epoch-over-complete} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over-complete} messages while being in $e$.
    
    \item Messages of \Cref{algorithm:round_1}:
    While in $e$, $P_i$ executes at most $f + 1$ rounds\footnote{Again, it can happen that the process executes $f + 2$ rounds while in $e$: $f + 1$ rounds of the epoch $e$ and the first round of the new epoch. However, at most $O(n)$ words are sent by $P_i$ within these $f + 2$ rounds.}.
    If $P_i$ is the leader of a round, it sends (at most) $O(n)$ words; otherwise, it sends $O(1)$ words.
    Given that, while in $e$, $P_i$ is the leader of (at most) one round and $f = O(n)$, it sends (at most) $O(n)$ words via the messages of a round (i.e., of \Cref{algorithm:round_1}).
\end{compactitem}
While in $e$, $P_i$ sends at most $O(n)$ words via the messages of each type, which concludes the lemma.
\end{proof}

Next, we show that, within any period of $\delta$ time after $\mathit{GST}$, a correct process can be in (at most) two epochs.

\begin{lemma} \label{lemma:within_delta}
Let $\mathcal{P} = [t_1, t_2]$ denote a time period such that $t_1 \geq \mathit{GST}$ and $t_2 - t_1 \leq \delta$.
Consider any correct process $P_i$.
Then, $P_i$ can be in at most two epochs within $\mathcal{P}$.
\end{lemma}
\begin{proof}
Let $P_i$ start an epoch $e$ at some time $t_e \geq \mathit{GST}$.
Assume that $P_i$ starts another epoch $e'$ at some time $t_{e'} > t_e$.
Due to the fact that (1) $e'$ is started at line~\ref{line:start_epoch}, and (2) $\mathit{sync\_timer}$ measures $\delta$ time, $t_{e'} - t_e \geq \delta$.
The lemma holds.
\end{proof}

Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$ (as in the proof of \Cref{theorem:termination}).
Moreover, let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.
Note that $t_{\mathit{final}}$ is not defined if no correct process ever starts epoch $e_{\mathit{max}} + 1$.
The next lemma shows that every correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ (if $t_{\mathit{final}}$ is defined).

\begin{lemma} \label{lemma:all_decide_by_t_final_epoch}
Let $t_{\mathit{final}}$ be defined (i.e., let there exist a correct process that starts epoch $e_{\mathit{max}} + 1$).
Then, all correct processes decide by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
\end{lemma}
\begin{proof}
The proof of this lemma follows the same argument as the proof of \Cref{theorem:termination}.
If a correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$, every process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ and the lemma holds.

Otherwise, the leader of the last round of epoch $e_{\mathit{max}} + 1$ is correct (if that was not the case, a correct process would decide in a round preceding this one, which means that a correct process would decide by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$).
Moreover, the leader has sent the \textsc{decide} message (at line~\ref{line:broadcast_decide_message} of \Cref{algorithm:round_1}) by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$.
Once a correct process receives this message, which happens by time $t_{\mathit{final}} + \mathit{epoch\_duration}$, it decides.
The lemma holds.
\end{proof}

The next lemma shows that no correct process ever starts any epoch greater than $e_{\mathit{max}} + 1$.
This lemma is the consequence of \Cref{lemma:all_decide_by_t_final_epoch}.

\begin{lemma} \label{lemma:no_process_starts_emax_1}
No correct process starts an epoch $e > e_{\mathit{max}} + 1$.
\end{lemma}
\begin{proof}
By contradiction, suppose that a correct process starts an epoch $e > e_{\mathit{max}} + 1$.
Therefore, a correct process has sent an \textsc{epoch-over} message for $e_{\mathit{max}} + 1$.
However, this is impossible due to \Cref{lemma:all_decide_by_t_final_epoch} (recall that the rule at line~\ref{line:upon_round_timer} of \Cref{algorithm:round_2} activates only after all ``round-specific'' messages; see line~\ref{line:rule} of \Cref{algorithm:round_2}).
The lemma holds.
\end{proof}

Finally, we are ready to prove the communication complexity of \name.

\begin{theorem} [Communication complexity]
\name has $O(n^2)$ communication complexity.
\end{theorem}
\begin{proof}
By time $\mathit{GST} + \delta$, each process receives an \textsc{epoch-over-complete} message for epoch $e_{\mathit{max}} - 1$.
Hence, before time $\mathit{GST} + 3\delta$ each correct process starts either epoch $e_{\mathit{max}}$ or $e_{\mathit{max}} + 1$.
Let us explain: a correct process $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}} - 1$ at time $\mathit{GST} + \delta$, sets its $\mathit{epoch}$ variable to $e_{\mathit{max}}$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; just before time $\mathit{GST} + 2\delta$, $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}}$, sets its $\mathit{epoch}$ variable to $e_{\mathit{max}} + 1$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; therefore, before time $\mathit{GST} + 3\delta$, $P_i$ starts $e_{\mathit{max}} + 1$.


Let us fix a correct process $P_i$.
By time $\mathit{GST} + 3\delta$, $P_i$ starts either epoch $e_{\mathit{max}}$ or epoch $e_{\mathit{max}} + 1$ (because of the argument given above).
By \Cref{lemma:no_process_starts_emax_1}, $P_i$ never starts an epoch greater than $e_{\mathit{max}} + 1$.
During $3\delta$ time period, $P_i$ can be in (at most) $6$ epochs (by \Cref{lemma:within_delta}); afterwards, $P_i$ can be in two epochs ($e_{\mathit{max}}$ and $e_{\mathit{max}} + 1$).
Since it sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}), $P_i$ sends at most $O(n)$ words after $\mathit{GST}$.
Therefore, the communication complexity of \name is indeed $O(n^2)$.
\end{proof}

% Observe the difference between entering and starting an epoch.
% A process enters an epoch by updating its $\mathit{epoch}$ variable, and only then starts it (if it does not enter another epoch in the meantime).

% The next lemma shows that, if a correct process starts an epoch $e$, then it has previously entered it.

% \begin{lemma} \label{lemma:enter_before_start}
% Let a correct process $P_i$ start an epoch $e > 1$ at time $t$.
% Then, $P_i$ has entered $e$ at time $t' < t$.
% \end{lemma}
% \begin{proof}
% Since $P_i$ starts $e > 1$ at time $t$, $P_i$ executes line~\ref{line:start_epoch} at time $t$.
% Given that the value of the $\mathit{epoch}$ variable at $P_i$ is $e$, $P_i$ has entered $e$.
% Moreover, $P_i$ has entered $e$ at some time $t' < t$ since (1) $\mathit{sync\_timer}$ has expired (line~\ref{line:sync_timer_expires}), and (2) we assume that $\mathit{sync\_timer}$ expires after some non-zero real time when measuring $\delta$ (even before $\mathit{GST}$).
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% rewriting the section in modular fashion %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{\name (BIS)}

This section presents \name.



First, we give the utility functions (\Cref{algorithm:utilities}) and variables and constants (\Cref{algorithm:variable_constants}) of processes.
The \name protocol is divided into two parts:
\begin{compactenum}
    \item View Executor protocol (\cref{algorithm:view_1,algorithm:view_2}): An execution of \name unfolds in views (like many other ``PBFT-like'' protocols).
    This part of the \name protocol presents the pseudocode of a view.
    
    \item View Synchronizer protocol (\Cref{algorithm:synchronizer}): This part of \name implements the view synchronizer defined in subsection \ref{subsection:view_synchronization}, i. e. ensures eventual synchronization time property.  
\end{compactenum}
In the rest of the paper, we refer to \cref{algorithm:round_1,algorithm:round_2} as the ``executor protocol'', whereas we refer to \Cref{algorithm:synchronizer} as the ``synchronizer protocol''.

\begin{algorithm}
\caption{Utilities (for process $P_i$)}
\label{algorithm:utilities}
\begin{algorithmic} [1]
\State \textbf{function} \texttt{msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em $m.\mathit{type} \gets \mathit{type}$; $m.\mathit{value} \gets \mathit{value}$; $m.\mathit{qc} \gets \mathit{qc}$; $m.\mathit{epoch} \gets \mathit{epoch}$; $m.\mathit{view} \gets \mathit{view}$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{vote\_msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em $m \gets \texttt{msg(}\mathit{type}, \mathit{value}, \mathit{qc}, \mathit{epoch}, \mathit{view}\texttt{)}$
\State \hskip2em $m.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m.\mathit{type}, m.\mathit{value}, m.\mathit{epoch}, m.\mathit{view}])$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{qc(Set(Vote\_Message)} $M$\texttt{)}: \Comment{All the messages from $M$ have the same type, value, epoch and view}
\State \hskip2em $\mathit{qc}.\mathit{type} \gets m.\mathit{type}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{value} \gets m.\mathit{value}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{epoch} \gets m.\mathit{epoch}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{view} \gets m.\mathit{view}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{sig} \gets \mathit{Combine}(\{\mathit{partial\_sig} \,|\, \exists m \in M: m.\mathit{partial\_sig} = \mathit{partial\_sig}\})$
\State \hskip2em \textbf{return} $\mathit{qc}$

\medskip
\State \textbf{function} \texttt{matching\_msg(Message} $m$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em \textbf{return} $m.\mathit{type} = \mathit{type}$ and $m.\mathit{epoch} = \mathit{epoch}$ and $m.\mathit{view} = \mathit{view}$

\medskip
\State \textbf{function} \texttt{matching\_qc(Quorum\_Certificate} $\mathit{qc}$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em \textbf{return} $\mathit{qc}.\mathit{type} = \mathit{type}$ and $\mathit{qc}.\mathit{epoch} = \mathit{epoch}$ and $\mathit{qc}.\mathit{view} = \mathit{view}$

\medskip
\State \textbf{function} \texttt{global\_view(Quorum\_Certificate} $\mathit{qc}$\texttt{)}:
\State \hskip2em \textbf{return} $(\mathit{qc}.\mathit{epoch} - 1) \cdot (f + 1) + \mathit{qc}.\mathit{view}$
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}
\caption{Variables and constants of View Synchronizer (for process $P_i$)}
\label{algorithm:variable_constants}
\begin{algorithmic} [1]

%\State \blue{\textbf{Variables of Executor:}}
%\State \texttt{Integer} $Exec.\mathit{epoch} \gets 1$ 
%\State \texttt{Integer} $Exec.\mathit{view} \gets 1$ 
%\State \texttt{Quorum\_Certificate} $\mathit{prepareQC} \gets \bot$
%\State \texttt{Quorum\_Certificate} $\mathit{lockedQC} \gets \bot$
\State \textbf{Variables:}
\State \texttt{Integer} $sync\_\mathit{epoch} \gets 1$ 
\State \texttt{Integer} $sync\_\mathit{view} \gets 1$ 
\State \texttt{Timer} $\mathit{view\_timer}$
\State \texttt{Timer} $\mathit{sync\_timer}$
\State \texttt{Signature} $\mathit{epoch\_over\_sig} \gets \bot$

\medskip
\State \textbf{Constants:}
\State \texttt{Time} $\mathit{view\_duration} = 10\delta$
\end{algorithmic}
\end{algorithm} 

\begin{algorithm} 
\caption{\name (View Executor): Pseudocode for process $P_i$}
\label{algorithm:view_1}
\begin{algorithmic} [1]
\State \st{\textbf{upon} \texttt{start\_round}:} 
\State \blue{\textbf{upon} \texttt{start\_view}$(e,v)$:}

\State \hskip2em \blue{$Exec.epoch \gets e$, $Exec.view \gets v$} 

\State \hskip2em stop reacting to events of the previous view protocol
\State \hskip2em start reacting to events of the view protocol

\State \hskip2em
\blue{\st{$\mathit{round\_timer}$\texttt{.measure($\mathit{round\_duration}$)}} \label{line:round_timer_measure}
\Comment{Timeout is handled by synchronizer now}}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{View-Change phase}
\State \hskip2em \texttt{send} \texttt{msg(}\textsc{view-change}, $\bot$, $\mathit{prepareQC}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Prepare phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ \textsc{view-change} messages: $M \gets \{m \,|\, \texttt{matching\_msg(}m, \textsc{view-change}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{highQC} \gets \mathit{qc}$ with the highest $\texttt{global\_view(}\mathit{qc}\texttt{)}$ in $M$
\State \hskip4em \texttt{Integer} $\mathit{proposal} \gets \mathit{highQC}.\mathit{value}$
\State \hskip4em \textbf{if} $\mathit{proposal} = \bot$:
\State \hskip6em $\mathit{proposal} \gets \mathit{proposal}_i$ \Comment{$\mathit{proposal}_i$ denotes the proposal of $P_i$}
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{prepare}, $\mathit{proposal}$, $\mathit{highQC}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_msg(}$m$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em \textbf{if} $m.\mathit{qc}.\mathit{value} = m.\mathit{value}$ and ($\mathit{lockedQC}.\mathit{value} = m.\mathit{value}$ or $\texttt{global\_view(}\mathit{qc}\texttt{)} > \mathit{lockedQC}.\mathit{view}$):
\State \hskip6em \texttt{send} \texttt{vote\_msg(}\textsc{prepare}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Precommit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{prepare}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{precommit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em $\mathit{prepareQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{precommit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Commit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{precommit}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{commit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{precommit}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em $\mathit{lockedQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{commit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Decide phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{commit}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{decide}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} \label{line:broadcast_decide_message}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{commit}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
% \State \hskip4em $\mathit{round\_timer}$\texttt{.cancel()} \Comment{timer's expiration event is canceled}
\State \hskip4em \texttt{finalize\_decision(}$m.\mathit{qc}$\texttt{)}
\algstore{alg:example}
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}
\caption{\name (View Executor): Pseudocode for process $P_i$}
\label{algorithm:view_2}
\begin{algorithmic} [1]
\algrestore{alg:example}
\State \st{\textbf{upon} \texttt{terminate\_view}:}
\State \hskip2em \st{$\mathit{view\_timer}$\texttt{.cancel()}} \Comment{\st{timer's expiration event is canceled}}
\State \hskip2em \st{stop reacting to events of the view protocol}

\medskip
\LineComment{\st{This rule is activated only after all received messages of the view protocol have been processed}} \label{line:rule}
\State \st{\textbf{upon} $\mathit{view\_timer}$ \textbf{expires}: }\label{line:upon_view_timer}
\State \hskip2em \st{ \textbf{trigger} \texttt{view\_expired} }
\State \hskip2em \st{stop reacting to events of the view protocol} 

\medskip

\State \textbf{function} \texttt{finalize\_decision(Quorum\_Certificate} $\mathit{qc}$\texttt{)}: \label{line:finalize_decision_function}
\State \hskip2em \texttt{broadcast} $\langle \textsc{decision}, \mathit{qc} \rangle$ \Comment{disseminate the quorum certificate} \label{line:broadcast_qc}
\State \hskip2em \textbf{trigger} \texttt{decide(}$\mathit{qc}.\mathit{value}$\texttt{)} \Comment{decision is made} \label{line:decide}
\State \hskip2em stop reacting to all events \label{line:stop_all_events} \Comment{``end'' of the algorithm}

\medskip
\State \textbf{upon} reception of $\langle \textsc{decision}, \texttt{Quorum\_Certificate} \text{ } \mathit{qc} \rangle$:
\State \hskip2em \texttt{finalize\_decision(}$\mathit{qc}$\texttt{)} \label{line:invoke_finalize_decision}
\end{algorithmic}
\end{algorithm} 


\begin{algorithm}
\caption{\name (View Synchronizer): Pseudocode for process $P_i$}
\label{algorithm:synchronizer}
\begin{algorithmic} [1]

\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm} \label{line:start_algorithm}
%\State \hskip2em start epoch $1$ \Comment{enter epoch $1$} \label{line:start_epoch_1}
%\State \hskip2em \textbf{trigger} \texttt{start\_view} \label{line:start_view_1} \Comment{start the first view of the first epoch}

%\State \hskip2em \blue{start $\mathit{epoch} 1$ \label{line:start_epoch_1}} \blue{\Comment{What is the meaning of this line ? Is it just to define what does mean "starting epoch 1" by refering to the line ?}}

\State \hskip2em
\blue{$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)} } \blue{\Comment{Handled by View Synchronizer now}}


\State \hskip2em \textbf{trigger} \blue{\texttt{advance}($sync\_epoch=1, sync\_view=1$})) \label{line:start_view_1} \Comment{start the first view of the first epoch}

\medskip
\State \st{ \textbf{upon} \texttt{view\_expired}:}
\State \blue{\textbf{upon} $view\_timer$ \textbf{expires}:}
\label{line:rule_view_expired}
\State \hskip2em \textbf{if} $\mathit{sync\_view} \neq f + 1$:
\State \hskip4em $\mathit{sync\_view} \gets \mathit{sync\_view} + 1$

%%
\State \hskip4em
\blue{$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)} } \blue{\Comment{Handled by View Synchronizer now}}

\State \hskip4em \textbf{trigger} \blue{\texttt{advance}($sync\_epoch, sync\_view$}))  \Comment{start the next view of the current epoch}
%%

%\State \hskip4em \textbf{trigger} \texttt{start\_view} \Comment{start the next view of the current epoch}
\State \hskip2em \textbf{else:}
\State \hskip4em \texttt{broadcast} $\langle \textsc{epoch-over}, \mathit{sync\_epoch}, \mathit{ShareSign}_i(\mathit{sync\_epoch}) \rangle$ \label{line:broadcast_epoch_over}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ from $2f + 1$ processes such that $e \geq \mathit{sync\_epoch}$: \label{line:receive_epoch_over}
\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{Combine}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in an } \textsc{epoch-over} \text{ message}\})$
\State \hskip2em $\mathit{sync\_epoch} \gets e + 1$ \Comment{enter $\mathit{epoch}$} \label{line:update_epoch_1}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over-complete}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ such that $e \geq \mathit{sync\_epoch}$: \label{line:receive_epoch_over_complete}
\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{sig}$
\State \hskip2em $\mathit{sync\_epoch} \gets e + 1$ \Comment{enter $\mathit{epoch}$} \label{line:update_epoch_2}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()} 
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)}

\medskip
\State \textbf{upon} $\mathit{sync\_timer}$ \textbf{expires}: \label{line:sync_timer_expires}
\State \hskip2em \texttt{broadcast} $\langle \textsc{epoch-over-complete}, \mathit{sync\_epoch} - 1, \mathit{epoch\_over\_sig} \rangle$ \label{line:broadcast_epoch_over_complete}
\State \hskip2em $\mathit{sync\_view} \gets 1$
%\State \hskip2em \blue{start $\mathit{epoch}$ \label{line:start_epoch}} \blue{\Comment{What is the meaning of this line ? Is it just to define what does mean "starting an epoch" by refering to the line ?}}

\State \hskip2em
\blue{$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)} \label{line:view_timer_measure}} \blue{\Comment{Handled by View Synchronizer now}}

\State \hskip2em \textbf{trigger} \blue{\texttt{advance}($sync\_epoch, sync\_view=1$})) \label{line:start_view_2} \Comment{start the first view of the next epoch}



\end{algorithmic}
\end{algorithm}

\subsection{Proof of Correctness}
We now prove the correctness of \name.
In order to do so, we need to prove that the view synchronizer ensures eventual eventual synchronization time.
%\name (\cref{algorithm:view_1,algorithm:view_2,algorithm:synchronizer}) satisfies validity, termination and agreement.
Whenever we reference lines of the pseudocode in the rest of the subsection, we refer to the lines of \Cref{algorithm:synchronizer} (if not explicitly stated otherwise).
We say that process $P_i$ enters in epoch $e$ (resp. in view $v$ of epoch $e$) at time $t$ if it triggers $\texttt{advance}(e,1)$ (resp. $\texttt{advance}(e,v)$) at time $t$.

\paragraph{Termination}
First, we prove that all correct processes decide if a correct process decides.

\pierre{This following lemma concerns the view executor, which is a problem for modularity. In fact, as currently stated, the View Synchronization does not precisely ensure eventual synchronization time but ensures 1) either termination or 2) eventual synchronization time that then lead to termination. The point is that it is possible for the Byzantine processes to make correct processes agree before reaching a synchronization time. Typically with a Byzantine leader that behaves to ensures termination before synchronization time. }

\green{This lemma has to be removed for modularity}
\begin{lemma} \label{lemma:one_decides_all_decide}
Let a correct process decide a value.
Then, every correct process eventually decides a value.
\end{lemma}
\begin{proof}
Let $P_i$ be the correct process that decides.
Before deciding (line~\ref{line:decide} of \Cref{algorithm:view_2}), $P_i$ disseminates the obtained quorum certificate (line~\ref{line:broadcast_qc} of \Cref{algorithm:view_2}).
Eventually, every correct process receives the broadcast \textsc{decision} message, enters the \texttt{finalize\_decision} function (line~\ref{line:invoke_finalize_decision} \Cref{algorithm:view_2}) and decides (line~\ref{line:decide} \Cref{algorithm:view_2}).
\end{proof}

A correct process $P_i$ \emph{starts} an epoch $e$ (at time $t$) if and only if $P_i$ executes (1) line~\ref{line:start_epoch_1} (at time $t$) in the case of $e = 1$, or (2) line~\ref{line:start_epoch} with $\mathit{sync\_epoch} = e$ (at time $t$) in the case of $e > 1$.
The next lemma shows that, if a correct process sends an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}), then the process has previously started $e$.

\begin{lemma} \label{lemma:epoch_over_previously_started}
Let a correct process $P_i$ broadcast an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}) at some time $t$.
Then, $P_i$ has started $e$ at some time $t' < t$.
\end{lemma}



\begin{proof}
At the moment of broadcasting the message, the following holds: (1) $\mathit{sync\_epoch} = e$ at $P_i$, and (2) $\mathit{sync\_view} = f + 1$ at $P_i$.
Therefore, all $f + 1$ views of the epoch $e$ have expired (otherwise, $P_i$ would have decided at line~\ref{line:decide} and stopped executing the protocol at line~\ref{line:stop_all_events}). %
%Hence, the first (out of the aforementioned $f + 1$) view of the epoch $e$ expired. If $e=1$, the result is immediate since process $P_i$ triggers $\texttt{advance}(1,1)$ at its starting time $t^s_i$.
%
\pierre{TO SIMPLIFY}
When the first (out of the aforementioned $f + 1$) view started (at line~\ref{line:start_view_1} or at line~\ref{line:start_view_2}), the epoch $e$ has started at the same time  (by same line~\ref{line:start_view_1} or line~\ref{line:start_view_2}).
Moreover, the epoch $e$ has started before the broadcasting of the message since, for each view of the epoch, $\mathit{view\_timer}$ measures $\mathit{view\_duration}$ time (line~\ref{line:view_timer_measure} \pierre{handled by View Synchronizer now}) and we assume that the timer expires after some non-zero real time when measuring $\mathit{view\_duration}$ (even before $\mathit{GST}$).
% Therefore, the lemma holds.
\end{proof}

Next, we prove that, if an epoch $e > 1$ is started by a correct process at some time $t$, then epoch $e - 1$ is started by a (potentially different) correct process at some time $t' < t$. 

\begin{lemma} \label{lemma:epoch_previously_started}
Let a correct process start an epoch $e > 1$ at time $t$.
Then, epoch $e - 1$ is started by a correct process at some time $t' < t$. 
\end{lemma}
\begin{proof}
Let a correct process $P_i$ start an epoch $e > 1$ at time $t$.
That means that $P_i$ executes line~\ref{line:start_epoch} at time $t$.
Hence, either the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} has been previously activated at process $P_i$.
Therefore, (at least) $f + 1$ correct processes have sent an $\textsc{epoch-over}$ message for $e - 1$ before time $t$.
By \Cref{lemma:epoch_over_previously_started}, these correct processes have started epoch $e - 1$ before sending the \textsc{epoch-over} messages, which concludes the proof.
\end{proof}

The next lemma shows that, if no correct process ever decides, all epochs are eventually started. 
In other words, correct processes keep transiting to new epochs forever.

\begin{lemma} \label{lemma:no_decision_constantly_next_epoch}
\st{Let no correct process ever decide.
Then,} every epoch $e \in \mathbb{N}$ is eventually started by a correct process. 
\end{lemma}
\begin{proof}
Epoch $1$ is started by a correct process since every correct process initially starts the epoch (at line~\ref{line:start_epoch_1}, upon executing the \texttt{start} rule).
Therefore, it is left to prove that all epochs greater than $1$ are started by a correct process.

By contradiction, let $e + 1 \in \mathbb{N}$ be the smallest epoch that is never started by a correct process, where $e \geq 1$.

\Cref{lemma:epoch_previously_started} shows that no epoch $e' > e + 1$ is ever started by a correct process.

Since epochs greater than $e$ are never started, no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$ (by \Cref{lemma:epoch_over_previously_started}).
Hence, the $\mathit{sync\_epoch}$ variable at a correct process cannot contain a value greater than $e + 1$ (see the rules at lines~\ref{line:receive_epoch_over} and~\ref{line:receive_epoch_over_complete}).
Moreover, if the $\mathit{sync\_epoch}$ variable at a correct process becomes $e + 1$ (at line~\ref{line:update_epoch_1} or at line~\ref{line:update_epoch_2}), the epoch $e + 1$ is started at that process because (1) \textsc{epoch-over} messages are not sent for epochs greater than $e$, and (2) $\mathit{sync\_timer}$ eventually expires (and the rule at line~\ref{line:sync_timer_expires} activates).
Given that epoch $e + 1$ is never started, no correct process sets its $\mathit{sync\_epoch}$ variable to $e + 1$.

Since epoch $e$ is started by a correct process, every correct process eventually sets its $\mathit{sync\_epoch}$ variable to $e$: (1) if $e = 1$, that happens as soon as the process starts executing the protocol, or (2) otherwise, every correct process receives an \textsc{epoch-over-complete} message for $e - 1$ and, since the $\mathit{sync\_epoch}$ variable cannot have a value greater than $e$, starts $e$ eventually.
Given that (1) no correct process ever decides, and (2) no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$, \st{every correct process receives the \texttt{view\_expired} event} \blue{$view\_timer$ expires for every correct process} for each view of the epoch $e$ (line~\ref{line:rule_view_expired}).
Once that happens, a correct process broadcasts an \textsc{epoch-over} message for the epoch $e$ (line~\ref{line:broadcast_epoch_over}).
Therefore, once a correct process receives the \textsc{epoch-over} messages from all correct processes (and the rule at line~\ref{line:receive_epoch_over} activates), the process updates its $\mathit{sync\_epoch}$ variable to $e + 1$ (at line~\ref{line:update_epoch_1}).
Hence, we reach contradiction and the lemma holds.
\end{proof}

The following lemma proves that, if the first correct process to start an epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ before time $t + \mathit{epoch\_duration}$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{view\_duration}$.

\begin{lemma} \label{lemma:no_epoch_over_for_epoch_duration}
Let $t$ be time such that (1) $t \geq \mathit{GST}$, (2) a correct process starts an epoch $e$ at time $t$, and (3) no correct process has started $e$ before time $t$.
Then, no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) before time $t + \mathit{epoch\_duration}$.
\end{lemma}
\begin{proof}
First, no correct process sends an \textsc{epoch-over} message for epoch $e$ before time $t + \mathit{epoch\_duration}$ since the first process to start $e$ does so at time $t \geq \mathit{GST}$.
Therefore, epoch $e + 1$ cannot be started by a correct process by time $t + \mathit{epoch\_duration}$.

By contradiction, suppose that a correct process sends an \textsc{epoch-over} message for an epoch $e' > e$ before time $t + \mathit{epoch\_duration}$.
By \cref{lemma:epoch_over_previously_started,lemma:epoch_previously_started}, epoch $e + 1$ has started before time $t + \mathit{epoch\_duration}$, which is a contradiction with the fact that epoch $e + 1$ does not start by time $t + \mathit{epoch\_duration}$.
Therefore, the lemma stands.
\end{proof}

\Cref{lemma:no_epoch_over_for_epoch_duration} has the following consequence: if the first correct process that starts a new epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process ``leaves'' epoch $e$ by time $t + \mathit{epoch\_duration}$.

\paragraph*{Notation}

Let us fix an execution of the View Synchronizer.
We note:
\begin{compactitem}
\item  $e_{\mathit{max}}$: the highest epoch started by a correct process by time $\mathit{GST}$.
\item $t_{\mathit{final}}$: the first time such that a correct process starts epoch $e_{\mathit{max}} + 1$, i. e. a time such that: 
\begin{compactenum}
\item  a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and 
\item no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.
    
\end{compactenum}

\end{compactitem}

Note that $t_{\mathit{final}}$ exists (by \Cref{lemma:no_decision_constantly_next_epoch}) and $t_{\mathit{final}} > \mathit{GST}$.


Finally, we prove the termination property.

\begin{theorem} [Termination] \label{theorem:termination}
\blue{\Cref{algorithm:synchronizer} ensures eventual synchronization time which is reached by time $t_{\mathit{final}} + \mathit{epoch\_duration}$} (which means
\name satisfies termination).
\end{theorem}
\begin{proof}
\st{We prove the theorem by contradiction.}
\st{Let there exist a correct process $P_i$ that never decides.}
\st{By lemma 18, if a correct process decides, all correct processes (including $P_i$) decide.
Therefore, no correct process decides.}



\st{Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$.
Let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.}
\st{Note that $t_{\mathit{final}}$ exists (by lemma 21) and $t_{\mathit{final}} > \mathit{GST}$.}
Furthermore, \Cref{lemma:no_epoch_over_for_epoch_duration} guarantees that no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e_{\mathit{max}} + 1$ before time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
    
Next, the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} is activated at each correct process by time $t_{\mathit{final}} + \delta$ (recall that $t_{\mathit{final}} > \mathit{GST}$).
Hence, every correct process starts the epoch $e_{\mathit{max}} + 1$ by time $t_{\mathit{final}} + 2\delta$ (due to the $\mathit{sync\_timer}$).
    
Finally, in each view of the epoch $e_{\mathit{max}} + 1$, all correct processes overlap for (at least) $8\delta$ time (given that $\mathit{view\_duration} = 10\delta$ and the biggest ``delay'' between epoch starts is $2\delta$; recall that hardware clocks of processes do not drift after $\mathit{GST}$).
Given that (1) at least one view of the epoch $e_{\mathit{max}} + 1$ has a correct leader (since there are $f + 1$ views in $e_{\mathit{max}} + 1$), \st{(2) $8\delta$ time is sufficient for a decision in each view of the epoch $e_{\mathit{max}} + 1$ after the last correct process has started the view (if the view has a correct leader)}, and (3) the last correct process starts the $(f + 1)$-st view of the epoch by time $t_{\mathit{final}} + f\cdot\mathit{view\_duration} + 2\delta$, \st{every correct process decides} \blue{synchronization time is reached} by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
\pierre{The following sentence can be removed: Recall that the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} is activated only after all received messages of the view protocol have been processed, which implies that, in a view of the epoch with a correct leader, the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} is not activated at a correct process before the process decides\footnote{Observe that, in the case the correct process decides, the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} will never get activated because of line~\ref{line:stop_all_events} of \Cref{algorithm:synchronizer}.}.}
Therefore, we reach a contradiction with the fact that no correct process decides, which implies that termination is satisfied by \name.
% \end{compactenum}
% Termination is satisfied by \name.
\end{proof}

\paragraph{Communication complexity.}
First, we show that each process sends at most $O(n)$ words within any epoch.
Formally, we say that a correct process $P_i$ is \emph{in epoch $e$} between the time $t$ when it starts $e$ and the time $t'$ when it starts some other epoch.
If it does not start some other epoch, $P_i$ remains in $e$ forever.

\begin{lemma} \label{lemma:linear_in_an_epoch}
For any epoch $e$ and any correct process $P_i$, process $P_i$ sends at most $O(n)$ words while being in $e$.
\end{lemma}
\begin{proof}
Let us consider all messages that $P_i$ can send while being in epoch $e$:
\begin{compactitem}
    \item \textsc{decision} messages (sent at line~\ref{line:broadcast_qc}):
    These messages are sent by $P_i$ only once throughout any execution (i.e., line~\ref{line:broadcast_qc} is executed at most once).
    Given that each messages contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{decision} messages while being in epoch $e$.
    
    \item \textsc{epoch-over} messages (sent at line~\ref{line:broadcast_epoch_over}):
    These messages are sent by $P_i$ only once while $P_i$ is in $e$ \pierre{TO CORRECT} since the next \texttt{start\_view} event is triggered at line~\ref{line:start_view_2}, which implies that the new epoch has started (line~\ref{line:start_epoch}).
    Given that each \textsc{epoch-over} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over} messages while being in $e$.
    
    \item \textsc{epoch-over-complete} messages (sent at line~\ref{line:broadcast_epoch_over_complete}):
    These messages are sent by $P_i$ only once\footnote{Formally speaking, these messages can be sent twice while $P_i$ is in $e$: the first time when it starts $e$ (recall that local computation takes zero time) and the second time when it starts some other epoch. However, it is important that these messages are sent \emph{constant} number of times in $e$.} while $P_i$ is in $e$ because upon the expiration of the $\mathit{sync\_timer}$ (at line~\ref{line:sync_timer_expires}) $P_i$ starts a new epoch (at line~\ref{line:start_view_2}).
    Given that each \textsc{epoch-over-complete} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over-complete} messages while being in $e$.
    
    \item Messages of \Cref{algorithm:view_1}:
    While in $e$, $P_i$ executes at most $f + 1$ views\footnote{Again, it can happen that the process executes $f + 2$ views while in $e$: $f + 1$ views of the epoch $e$ and the first view of the new epoch. However, at most $O(n)$ words are sent by $P_i$ within these $f + 2$ views.}.
    If $P_i$ is the leader of a view, it sends (at most) $O(n)$ words; otherwise, it sends $O(1)$ words.
    Given that, while in $e$, $P_i$ is the leader of (at most) one view and $f = O(n)$, it sends (at most) $O(n)$ words via the messages of a view (i.e., of \Cref{algorithm:view_1}).
\end{compactitem}
While in $e$, $P_i$ sends at most $O(n)$ words via the messages of each type, which concludes the lemma.
\end{proof}

Next, we show that, within any period of $\delta$ time after $\mathit{GST}$, a correct process can be in (at most) two epochs.

\begin{lemma} \label{lemma:within_delta}
Let $\mathcal{P} = [t_1, t_2]$ denote a time period such that $t_1 \geq \mathit{GST}$ and $t_2 - t_1 \leq \delta$.
Consider any correct process $P_i$.
Then, $P_i$ can be in at most two epochs within $\mathcal{P}$.
\end{lemma}
\begin{proof}
Let $P_i$ start an epoch $e$ at some time $t_e \geq \mathit{GST}$.
Assume that $P_i$ starts another epoch $e'$ at some time $t_{e'} > t_e$.
Due to the fact that (1) $e'$ is started at line~\ref{line:start_epoch}, and (2) $\mathit{sync\_timer}$ measures $\delta$ time, $t_{e'} - t_e \geq \delta$.
The lemma holds.
\end{proof}

Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$ (as in the proof of \Cref{theorem:termination}).
Moreover, let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.
Note that $t_{\mathit{final}}$ is not defined if no correct process ever starts epoch $e_{\mathit{max}} + 1$.
The next lemma shows that every correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ (if $t_{\mathit{final}}$ is defined).

\begin{lemma} \label{lemma:all_decide_by_t_final_epoch}
Let $t_{\mathit{final}}$ be defined (i.e., let there exist a correct process that starts epoch $e_{\mathit{max}} + 1$).
Then, \st{all correct processes decide} \blue{synchronization time is reached} by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
\end{lemma}
\begin{proof}
The proof of this lemma follows the same argument as the proof of \Cref{theorem:termination}.
\st{If a correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$, every process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ and the lemma holds.}

\st{Otherwise,} there is a view $v$ of epoch $e_{\mathit{max}} + 1$ s. t. the leader of this view is correct.
\st{the last view of epoch $e_{\mathit{max}} + 1$ is correct (if that was not the case, a correct process would decide in a view preceding this one, which means that a correct process would decide by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$).}
Moreover, the leader has sent the \textsc{decide} message (at line~\ref{line:broadcast_decide_message} of \Cref{algorithm:view_1}) by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$.
Once a correct process receives this message, which happens by time $t_{\mathit{final}} + \mathit{epoch\_duration}$, it decides.
The lemma holds.
\end{proof}

The next lemma shows that no correct process ever starts any epoch greater than $e_{\mathit{max}} + 1$.
This lemma is the consequence of \Cref{lemma:all_decide_by_t_final_epoch}.

\begin{lemma} \label{lemma:no_process_starts_emax_1}
No correct process starts an epoch $e > e_{\mathit{max}} + 1$ \blue{before synchronization time}. 
\end{lemma}
\begin{proof}
By contradiction, suppose that a correct process starts an epoch $e > e_{\mathit{max}} + 1$ before synchronization time.
Therefore, a correct process has sent an \textsc{epoch-over} message for $e_{\mathit{max}} + 1$ before synchronization time.
However, this is impossible due to \Cref{lemma:all_decide_by_t_final_epoch} \pierre{TO REMOVE OR TO ADAPT (recall that the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} activates only after all ``view-specific'' messages; see line~\ref{line:rule} of \Cref{algorithm:view_2}).}
The lemma holds.
\end{proof}

Finally, we are ready to prove the communication complexity of \name.

\begin{theorem} [Communication complexity]
\name has $O(n^2)$ communication complexity.
\end{theorem}
\begin{proof}
By time $\mathit{GST} + \delta$, each process receives an \textsc{epoch-over-complete} message for epoch $e_{\mathit{max}} - 1$ .
Hence, before time $\mathit{GST} + 3\delta$ each correct process starts either epoch $e_{\mathit{max}}$ or $e_{\mathit{max}} + 1$.
Let us explain: a correct process $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}} - 1$ at time $\mathit{GST} + \delta$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}}$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; just before time $\mathit{GST} + 2\delta$, $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}}$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}} + 1$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; therefore, before time $\mathit{GST} + 3\delta$, $P_i$ starts $e_{\mathit{max}} + 1$.


Let us fix a correct process $P_i$.
By time $\mathit{GST} + 3\delta$, $P_i$ starts either epoch $e_{\mathit{max}}$ or epoch $e_{\mathit{max}} + 1$ (because of the argument given above).
By \Cref{lemma:no_process_starts_emax_1}, $P_i$ never starts an epoch greater than $e_{\mathit{max}} + 1$.
During $3\delta$ time period, $P_i$ can be in (at most) $6$ epochs (by \Cref{lemma:within_delta}); afterwards, $P_i$ can be in two epochs ($e_{\mathit{max}}$ and $e_{\mathit{max}} + 1$).
Since it sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}), $P_i$ sends at most $O(n)$ words after $\mathit{GST}$.
Therefore, the communication complexity of \name is indeed $O(n^2)$.
\end{proof}





==> depricated/round_sync.tex <==
\section{\rare: View Synchronizer with $O(n^2)$ Communication and \phantom{aa} $O(f)$ Latency}

This section is devoted to \rare (\Cref{algorithm:synchronizer}), a view synchronizer that achieves $O(n^2)$ worst-case communication complexity.
First, we formally define the problem of view synchronization (\Cref{subsection:view_synchronization_problem_definition}).
Then, we present \rare and prove its correctness and complexity (\Cref{subsection:rare}).

\subsection{View Synchronization: Problem Definition} \label{subsection:view_synchronization_problem_definition}

The following definition of the view synchronization problem follows previously introduced definitions~\cite{BravoCG20,naor2020expected,NBMS20}.
Let $\mathsf{View} = \{1, 2, ...\}$ denote the set of views.
For each view $v \in \mathsf{View}$, we define $\mathsf{leader}(v)$ to be a process that is the \emph{leader} of view $v$.
The view synchronization problem is associated with a predefined constant $c_s \in \mathbb{N}$ and it provides the following interface:
\begin{compactitem}
    \item \textbf{indication} $\mathsf{advance}(v \in \mathsf{View})$: The process advances to a view $v$.
\end{compactitem}
We say that a correct process \emph{is in view} $v \in \mathsf{View}$ between the time $t$ at which the process receives the $\mathsf{advance}(v)$ indication and the time at which the process receives the $\mathsf{advance}(v' \neq v)$ indication after time $t$.
If the process never receives $\mathsf{advance}(v' \neq v)$, then the process remains in the view $v$ from time $t$ onward.

Next, we define a synchronization time as a time at which all correct processes are in the same view with a correct leader for sufficiently long.

\begin{definition} [Synchronization Time]
Time $t_s$ is a \emph{synchronization time} if (1) all correct processes are in the same view $v$ from time $t_s$ to (at least) time $t_s + c_s\cdot\delta$, and (2) $\mathsf{leader}(v)$ is correct.
\end{definition}

View synchronization ensures the \emph{eventual synchronization} property which states that there exists a synchronization time after $\mathit{GST}$.

\medskip
\noindent \textbf{Complexity of view synchronization.}
Let $\mathsf{Synchronizer}$ be a view synchronizer and let $\mathcal{E}(\mathsf{Synchronizer})$ denote the set of all possible executions of $\mathsf{Synchronizer}$.
Let $\alpha \in \mathcal{E}(\mathsf{Synchronizer})$ be an execution and let $t_s(\alpha)$ denote the first synchronization time after $\mathit{GST}$ in $\alpha$ (i.e., $t_s(\alpha) \geq \mathit{GST}$).
We define the communication complexity of $\alpha$ as the number of words sent in messages in $\alpha$ by all correct processes in the time period $[\mathit{GST}, t_s(\alpha)]$.
The latency complexity of $\alpha$ is $t_s(\alpha) - \mathit{GST}$.

The \emph{communication complexity} of $\mathsf{Synchronizer}$ is defined as
\begin{equation*}
\max_{\alpha \in \mathcal{E}(\mathsf{Synchronizer})}\bigg\{\text{communication complexity of } \alpha\bigg\}.
\end{equation*}

Similarly, the \emph{latency complexity} of $\mathsf{Synchronizer}$ is defined as 
\begin{equation*}
\max_{\alpha \in \mathcal{E}(\mathsf{Synchronizer})}\bigg\{\text{latency complexity of } \alpha\bigg\}.
\end{equation*}

\iffalse
\subsection{Naive Implementation}

We rewrite the analysis of naive view doubling synchronizer (already presented in \cite{NBMS20}) that enables quadratic communication complexity but with costly latency complexity exponential with the number of faulty processes.

In this approach, each view has a timer, and if no progress is made the node moves to the next view and increases the timer time for the next view, where we note $\beta$ the arbitrary duration of the first view. The view duration has to increase indefinitely to enable late processes, (e.g. last ones that started the protocol or the ones with the slowest clocks), to catch up the most in advance ones, without communication.
To do this, the duration of a view $v$ has to be greater than the duration of the sum of all previous views up to view $v-1$, which lead us to an exponential pattern. Typically the duration of view $v$ is $\beta \cdot 2^{v-1}$ (The constant $2$ can be replaced by any value strictly greater than $1$).


\begin{algorithm} 
\caption{View doubling synchronizer: Pseudocode for process $P_i$}
\label{algorithm:view-doubling-synchronizer}
\begin{algorithmic} [1]


\State \textbf{initialize} : 
\State \hskip2em $current\_view \gets 1$
\State \hskip2em $view\_duration \gets \beta$ \Comment{$\beta$ is predefined value for the duration of the first view}

\State \textbf{upon} timer expiration: 
\State \hskip2em $view\_duration \gets 2\cdot view\_duration$ 
\State \hskip2em $start(current\_view +1)$

\end{algorithmic}
\end{algorithm}

This synchronizer possesses the advantage of a free communication, but suffer from an unbounded latency complexity. Indeed, even without clock drift, if the most in advance correct process start the protocol at time $0$, while the most late correct process start the protocol at time $GST$.



%it is possible for a correct process to enter in first view, while another 
Indeed, at GST, a correct process can enter in the first view, while
there is no bound on the view $v_{max}$ of the most in advance process. Hence, the synchronization time will not be met before time $\beta\cdot 2^{v_{max}}$ which is unbounded.
\fi

\subsection{\rare} \label{subsection:rare}

This subsection presents \rare, a view synchronizer with $O(n^2)$ communication complexity and $O(f)$ latency complexity.
In short, \rare achieves such complexity by exploiting the ``all-to-all'' communication only once per $f + 1$ views.

\medskip 
\noindent \textbf{Intuition.}
We group views into \emph{epochs}, where each epoch contains $f + 1$ sequential views.
Processes move through an epoch solely by means of local timeouts (without any communication).
However, at the end of each epoch, processes engage in an ``all-to-all'' communication step to obtain permission to move onto the next epoch: (1) Once a correct process has completed an epoch, it reliably broadcasts a message informing other processes of its completion; (2) Upon receiving $2f + 1$ of such messages, a correct process enters the future epoch. Note that (2) applies to \emph{all} processes, including those in arbitrarily ``old'' epochs.
Overall, this communication step is the \emph{only} communication processes perform within a single epoch, implying that per-process communication complexity in each epoch is $O(n)$.
\Cref{fig:raresync} illustrates the main idea behind \rare.


\begin{figure}[h]
    \centering
    \includegraphics[scale=0.22]{figures/raresync.png}
    \caption{Intuition behind \rare: Processes communicate only in the last view of an epoch; before the last view, they rely solely on local timeouts.}
    \label{fig:raresync}
\end{figure}

Roughly speaking, after $\mathit{GST}$, all correct processes will simultaneously enter the same epoch within $O(f)$ time.
After entering the same epoch, processes are guaranteed to synchronize in that epoch, which takes (at most) another $O(f)$ time.
Thus, the latency complexity of \rare is $O(f)$.
The communication complexity of \rare is $O(n^2)$ because every correct process executes at most a constant number of epochs, each with $O(n)$ per-process communication, after $\mathit{GST}$.


\medskip
\noindent \textbf{Protocol description.}


In that section, we will present \rare (\Cref{algorithm:synchronizer}), a protocol implementing the view synchronization abstraction with quadratic worst case communication complexity and linear worst case latency complexity.

The protocol increments a counter variable $global\_view$ and repeatedly triggers $\texttt{advance}(global\_view)$ (line~\ref{line:start_view_1}, \ref{line:start_view_without_msg_exchange}, \ref{line:start_view_2}) to enforce the core protocol to advance in the view $global\_view$.
The views are partitioned into epochs, that are set of $f+1$ consecutive views. Epoch 1 is the set of views $1, 2, ..., f+1$, epoch 2 is the set of views $f+2, f+3, ..., f+2$, etc. We say that process $P_i$ enters in view $v$ of epoch $e$ at time $t$ if it triggers $\texttt{advance}(global\_view)$ at time $t$ for variables $global\_view = (e-1) \cdot (f+1) + v$. If $v=1$, we say that $P_i$ enters in epoch $e$ (line~\ref{line:start_view_1}, \ref{line:start_view_2}). 
Every time a correct process enters in a view $v$, it sets its timer $view\_timer$ to $view\_duration$ (line~\ref{line:view_timer_measure_first_view}, \ref{line:view_timer_measure_without_msg_exchange}, \ref{line:view_timer_measure}). Then, by default (if it does not receive special messages), it waits for  $view\_timer$ expiration (line~\ref{line:rule_view_expired}), enter in next view (line \ref{line:start_view_without_msg_exchange}) and repeat that procedure again until it reach a new epoch. 
When the timer of correct process $P_i$ expires for last view of epoch $e$, $P_i$ informs the other processes that it terminated the epoch $e$ by broadcasting an $\textsc{epoch-over}$ message  for epoch $e$ with its share-signature (line~\ref{line:broadcast_epoch_over}). At this moment, process $P_i$ does not want to make progress alone. This is why, before starting next epoch, he waits for some special messages (line~\ref{line:receive_epoch_over}, \ref{line:receive_epoch_over_complete}) that cannot be computed if less than $f+1$  correct processes did not visit the epoch $e$. In fact, the reception of these special messages is a necessary and sufficient condition to start a new epoch $e'>e$, even if the current epoch $e$ is not over for $P_i$ but over for $2f+1$ processes, and so at least for $f+1$ correct processes.

Upon the reception of $2f+1$ share-signed $\textsc{epoch-over}$ messages for epoch $e$ with valid share-signatures (line~\ref{line:receive_epoch_over}), correct process $P_i$ combines the share-signatures to obtain a threshold signature (line \ref{line:combine-signatures}), wait $\delta$ time (line~\ref{line:sync_timer_measure} and \ref{line:sync_timer_expires}) to check if it does not receive some special messages for an higher epoch,  broadcasts an $\textsc{epoch-over-complete}$ message for epoch $e$ with the attached threshold signature (line~\ref{line:broadcast_epoch_over_complete}) and then advances to the epoch $e+1$ (line~\ref{line:start_view_2}). 
In the same way, upon the reception of a  $\textsc{epoch-over-message}$ message for epoch $e$ with valid threshold-signature (line~\ref{line:receive_epoch_over_complete}), correct process $P_i$ wait $\delta$ time (line~\ref{line:sync_timer_measure_2} and \ref{line:sync_timer_expires}) to check if it does not receive some special messages for an higher epoch, re-broadcast the same $\textsc{epoch-over-complete}$ message for epoch $e$ with the same attached threshold signature  (line~\ref{line:broadcast_epoch_over_complete}) and then advances to the epoch $e+1$ (line~\ref{line:start_view_2}). 
Waiting $\delta$ time (line~\ref{line:sync_timer_measure} or \ref{line:sync_timer_measure_2} and \ref{line:sync_timer_expires}) allows to bound the communication-complexity after GST, to not send an unbounded number of $\textsc{epoch-over}$ and $\textsc{epoch-over-complete}$ messages.

\begin{algorithm}
\caption{\rare: Variables and constants \rare (for process $P_i$)}
\label{algorithm:variable_constants}
\begin{algorithmic} [1]

%\State \blue{\textbf{Variables of Executor:}}
%\State \texttt{Integer} $Exec.\mathit{epoch} \gets 1$ 
%\State \texttt{Integer} $Exec.\mathit{view} \gets 1$ 
%\State \texttt{Quorum\_Certificate} $\mathit{prepareQC} \gets \bot$
%\State \texttt{Quorum\_Certificate} $\mathit{lockedQC} \gets \bot$
\State \textbf{Variables:}
\State \hskip2em $\mathsf{Epoch}$ $\mathit{epoch} \gets 1$ 
\State \hskip2em $\mathsf{View}$ $\mathit{view} \gets 1$ 
\State \hskip2em $\mathsf{Timer}$ $\mathit{view\_timer}$
\State \hskip2em $\mathsf{Timer}$ $\mathit{disseminate\_timer}$
\State \hskip2em $\mathsf{Signature}$ $\mathit{epoch\_completed}$

\smallskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Time}$ $\mathit{view\_duration} = (c_s + 2) \cdot \delta$
\end{algorithmic}
\end{algorithm} 

%% old presentation
\iffalse
First, we give the utility functions (\Cref{algorithm:utilities}) and variables and constants (\Cref{algorithm:variable_constants}) of processes.
The \name protocol is divided into two parts:
\begin{compactenum}
    \item View Executor protocol (\cref{algorithm:view_1,algorithm:view_2}): An execution of \name unfolds in views (like many other ``PBFT-like'' protocols).
    This part of the \name protocol presents the pseudocode of a view.
    
    \item View Synchronizer protocol (\Cref{algorithm:synchronizer}): This part of \name implements the view synchronizer defined in subsection \ref{subsection:view_synchronization}, i. e. ensures eventual synchronization time property.  
\end{compactenum}
In the rest of the paper, we refer to \cref{algorithm:round_1,algorithm:round_2} as the ``executor protocol'', whereas we refer to \Cref{algorithm:synchronizer} as the ``synchronizer protocol''.
\fi
%% old presentation
\begin{algorithm}
\caption{\rare (View Synchronizer): Pseudocode for process $P_i$}
\label{algorithm:synchronizer}
\begin{algorithmic} [1]

\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm} \label{line:start_algorithm}
%\State \hskip2em start epoch $1$ \Comment{enter epoch $1$} \label{line:start_epoch_1}
%\State \hskip2em \textbf{trigger} \texttt{start\_view} \label{line:start_view_1} \Comment{start the first view of the first epoch}

%\State \hskip2em \blue{start $\mathit{epoch} 1$ \label{line:start_epoch_1}} \blue{\Comment{What is the meaning of this line ? Is it just to define what does mean "starting epoch 1" by refering to the line ?}}

\State \hskip2em
$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)}  \label{line:view_timer_measure_first_view} 

\State \hskip2em \textbf{trigger} \texttt{advance}($\mathit{global\_view}$) \label{line:start_view_1} \Comment{start the first view of the first epoch}

\medskip
%\State \st{ \textbf{upon} \texttt{view\_expired}:}
\State \textbf{upon} $view\_timer$ \textbf{expires}:
\label{line:rule_view_expired}
\State \hskip2em \textbf{if} $\mathit{sync\_view} \neq f + 1$:
\State \hskip4em $\mathit{sync\_view} \gets \mathit{sync\_view} + 1$
\State \hskip4em $\mathit{global\_view} \gets (\mathit{sync\_epoch}-1) \cdot (f+1) + \mathit{sync\_view}$

%%
\State \hskip4em
$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)}  \label{line:view_timer_measure_without_msg_exchange} 

\State \hskip4em \textbf{trigger} \texttt{advance}($\mathit{global\_view}$) \label{line:start_view_without_msg_exchange} \Comment{start the next view of the current epoch}
%%

%\State \hskip4em \textbf{trigger} \texttt{start\_view} \Comment{start the next view of the current epoch}
\State \hskip2em \textbf{else:}
\State \hskip4em \texttt{broadcast} $\langle \textsc{epoch-over}, \mathit{sync\_epoch}, \mathit{ShareSign}_i(\mathit{sync\_epoch}) \rangle$ \label{line:broadcast_epoch_over}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ from $2f + 1$ processes such that $e \geq \mathit{sync\_epoch}$: \label{line:receive_epoch_over}
%\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{Combine}(\{\mathit{sig} \,|\, \mathit{sig} \text{ is received in an } \textsc{epoch-over} \text{ message}\})$ \label{line:combine-signatures}
\State \hskip2em $\mathit{sync\_epoch} \gets e + 1$  \label{line:update_epoch_1} %\Comment{enter $\mathit{epoch}$}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)} \label{line:sync_timer_measure}

\medskip
\State \textbf{upon} reception of $\langle \textsc{epoch-over-complete}, \texttt{Integer} \text{ } e, \texttt{Signature} \text{ } \mathit{sig} \rangle$ such that $e \geq \mathit{sync\_epoch}$: \label{line:receive_epoch_over_complete}
%\State \hskip2em \st{\textbf{trigger} \texttt{terminate\_view}} 
\State \hskip2em $\mathit{epoch\_over\_sig} \gets \mathit{sig}$
\State \hskip2em $\mathit{sync\_epoch} \gets e + 1$  \label{line:update_epoch_2} %\Comment{enter $\mathit{epoch}$}
\State \hskip2em $\mathit{sync\_timer}$\texttt{.cancel()} 
\State \hskip2em $\mathit{sync\_timer}$\texttt{.measure(}$\delta$\texttt{)} \label{line:sync_timer_measure_2}

\medskip
\State \textbf{upon} $\mathit{sync\_timer}$ \textbf{expires}: \label{line:sync_timer_expires}
\State \hskip2em \texttt{broadcast} $\langle \textsc{epoch-over-complete}, \mathit{sync\_epoch} - 1, \mathit{epoch\_over\_sig} \rangle$ \label{line:broadcast_epoch_over_complete}
\State \hskip2em $\mathit{sync\_view} \gets 1$
\State \hskip2em $\mathit{global\_view} \gets (\mathit{sync\_epoch}-1) \cdot (f+1) + \mathit{sync\_view}$
%\State \hskip2em \blue{start $\mathit{epoch}$ \label{line:start_epoch}} \blue{\Comment{What is the meaning of this line ? Is it just to define what does mean "starting an epoch" by refering to the line ?}}

\State \hskip2em
$\mathit{view\_timer}$\texttt{.measure($\mathit{view\_duration}$)} \label{line:view_timer_measure} 

\State \hskip2em \textbf{trigger} \texttt{advance}($\mathit{global\_view}$) \label{line:start_view_2} \Comment{start the first view of the next epoch}



\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Utilities (for process $P_i$)}
\label{algorithm:utilities}
\begin{algorithmic} [1]
\State \textbf{function} \texttt{msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em $m.\mathit{type} \gets \mathit{type}$; $m.\mathit{value} \gets \mathit{value}$; $m.\mathit{qc} \gets \mathit{qc}$; $m.\mathit{epoch} \gets \mathit{epoch}$; $m.\mathit{view} \gets \mathit{view}$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{vote\_msg(String} $\mathit{type}$, \texttt{Integer} $\mathit{value}$, \texttt{Quorum\_Certificate} $\mathit{qc}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em $m \gets \texttt{msg(}\mathit{type}, \mathit{value}, \mathit{qc}, \mathit{epoch}, \mathit{view}\texttt{)}$
\State \hskip2em $m.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m.\mathit{type}, m.\mathit{value}, m.\mathit{epoch}, m.\mathit{view}])$
\State \hskip2em \textbf{return} $m$

\medskip
\State \textbf{function} \texttt{qc(Set(Vote\_Message)} $M$\texttt{)}: \Comment{All the messages from $M$ have the same type, value, epoch and view}
\State \hskip2em $\mathit{qc}.\mathit{type} \gets m.\mathit{type}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{value} \gets m.\mathit{value}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{epoch} \gets m.\mathit{epoch}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{view} \gets m.\mathit{view}$, where $m \in M$
\State \hskip2em $\mathit{qc}.\mathit{sig} \gets \mathit{Combine}(\{\mathit{partial\_sig} \,|\, \exists m \in M: m.\mathit{partial\_sig} = \mathit{partial\_sig}\})$
\State \hskip2em \textbf{return} $\mathit{qc}$

\medskip
\State \textbf{function} \texttt{matching\_msg(Message} $m$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em \textbf{return} $m.\mathit{type} = \mathit{type}$ and $m.\mathit{epoch} = \mathit{epoch}$ and $m.\mathit{view} = \mathit{view}$

\medskip
\State \textbf{function} \texttt{matching\_qc(Quorum\_Certificate} $\mathit{qc}$, \texttt{String} $\mathit{type}$, \texttt{Integer} $\mathit{epoch}$, \texttt{Integer} $\mathit{view}$\texttt{)}:
\State \hskip2em \textbf{return} $\mathit{qc}.\mathit{type} = \mathit{type}$ and $\mathit{qc}.\mathit{epoch} = \mathit{epoch}$ and $\mathit{qc}.\mathit{view} = \mathit{view}$

\medskip
\State \textbf{function} \texttt{global\_view(Quorum\_Certificate} $\mathit{qc}$\texttt{)}:
\State \hskip2em \textbf{return} $(\mathit{qc}.\mathit{epoch} - 1) \cdot (f + 1) + \mathit{qc}.\mathit{view}$
\end{algorithmic}
\end{algorithm} 



\begin{algorithm} 
\caption{\name (View Executor): Pseudocode for process $P_i$}
\label{algorithm:view_1}
\begin{algorithmic} [1]
%\State \st{\textbf{upon} \texttt{start\_round}:} 
\State \textbf{upon} \texttt{start\_view}$(\mathit{global\_view})$:

\State \hskip2em $Exec.epoch \gets (\mathit{global\_view} //(f+1)) +1$, \Comment{// stands for quotient of Euclidian division}
\State \hskip2em $Exec.view \gets \mathit{global\_view} \%(f+1)$ \Comment{\% stands for rest of Euclidian division}

\State \hskip2em stop reacting to events of the previous view protocol
\State \hskip2em start reacting to events of the view protocol

%\State \hskip2em \blue{\st{$\mathit{round\_timer}$\texttt{.measure($\mathit{round\_duration}$)}} \label{line:round_timer_measure} \Comment{Timeout is handled by synchronizer now}}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{View-Change phase}
\State \hskip2em \texttt{send} \texttt{msg(}\textsc{view-change}, $\bot$, $\mathit{prepareQC}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Prepare phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ \textsc{view-change} messages: $M \gets \{m \,|\, \texttt{matching\_msg(}m, \textsc{view-change}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{highQC} \gets \mathit{qc}$ with the highest $\texttt{global\_view(}\mathit{qc}\texttt{)}$ in $M$
\State \hskip4em \texttt{Integer} $\mathit{proposal} \gets \mathit{highQC}.\mathit{value}$
\State \hskip4em \textbf{if} $\mathit{proposal} = \bot$:
\State \hskip6em $\mathit{proposal} \gets \mathit{proposal}_i$ \Comment{$\mathit{proposal}_i$ denotes the proposal of $P_i$}
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{prepare}, $\mathit{proposal}$, $\mathit{highQC}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_msg(}$m$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em \textbf{if} $m.\mathit{qc}.\mathit{value} = m.\mathit{value}$ and ($\mathit{lockedQC}.\mathit{value} = m.\mathit{value}$ or $\texttt{global\_view(}\mathit{qc}\texttt{)} > \mathit{lockedQC}.\mathit{view}$):
\State \hskip6em \texttt{send} \texttt{vote\_msg(}\textsc{prepare}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Precommit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{prepare}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{precommit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{prepare}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em $\mathit{prepareQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{precommit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Commit phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{precommit}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{commit}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{precommit}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
\State \hskip4em $\mathit{lockedQC} \gets m.\mathit{qc}$
\State \hskip4em \texttt{send} \texttt{vote\_msg(}\textsc{commit}, $m.\mathit{value}$, $\bot$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} to \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}

\smallskip
\State \hskip2em \(\triangleright\) \textcolor{red}{Decide phase}
\State \hskip2em \textbf{as} \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}:
\State \hskip4em \textbf{wait for} $2f + 1$ votes: $V \gets \{\mathit{vote} \,|\, \texttt{matching\_msg(}\mathit{vote}, \textsc{commit}, \mathit{epoch}, \mathit{view}\texttt{)}\}$
\State \hskip4em \texttt{Quorum\_Certificate} $\mathit{qc} \gets \texttt{qc(}V\texttt{)}$
\State \hskip4em \texttt{broadcast} \texttt{msg(}\textsc{decide}, $\bot$, $\mathit{qc}$, $\mathit{epoch}$, $\mathit{view}$\texttt{)} \label{line:broadcast_decide_message}

\smallskip
\State \hskip2em \textbf{as} a process: \Comment{``always'' execute this part of the pseudocode}
\State \hskip4em \textbf{wait for} message $m$: \texttt{matching\_qc(}$m.\mathit{qc}$, \textsc{commit}, $\mathit{epoch}$, $\mathit{view}$\texttt{)} from \texttt{leader(}$\mathit{epoch}, \mathit{view}$\texttt{)}
% \State \hskip4em $\mathit{round\_timer}$\texttt{.cancel()} \Comment{timer's expiration event is canceled}
\State \hskip4em \texttt{finalize\_decision(}$m.\mathit{qc}$\texttt{)}
\algstore{alg:example}
\end{algorithmic}
\end{algorithm} 

\begin{algorithm}
\caption{\name (View Executor): Pseudocode for process $P_i$}
\label{algorithm:view_2}
\begin{algorithmic} [1]
\algrestore{alg:example}
%\State \st{\textbf{upon} \texttt{terminate\_view}:}
%\State \hskip2em \st{$\mathit{view\_timer}$\texttt{.cancel()}} \Comment{\st{timer's expiration event is canceled}}
%\State \hskip2em \st{stop reacting to events of the view protocol}

%\medskip
%\LineComment{\st{This rule is activated only after all received messages of the view protocol have been processed}} \label{line:rule}
%\State \st{\textbf{upon} $\mathit{view\_timer}$ \textbf{expires}: }\label{line:upon_view_timer}
%\State \hskip2em \st{ \textbf{trigger} \texttt{view\_expired} }
%\State \hskip2em \st{stop reacting to events of the view protocol} 

%\medskip

\State \textbf{function} \texttt{finalize\_decision(Quorum\_Certificate} $\mathit{qc}$\texttt{)}: \label{line:finalize_decision_function}
\State \hskip2em \texttt{broadcast} $\langle \textsc{decision}, \mathit{qc} \rangle$ \Comment{disseminate the quorum certificate} \label{line:broadcast_qc}
\State \hskip2em \textbf{trigger} \texttt{decide(}$\mathit{qc}.\mathit{value}$\texttt{)} \Comment{decision is made} \label{line:decide}
\State \hskip2em stop reacting to all events \label{line:stop_all_events} \Comment{``end'' of the algorithm}

\medskip
\State \textbf{upon} reception of $\langle \textsc{decision}, \texttt{Quorum\_Certificate} \text{ } \mathit{qc} \rangle$:
\State \hskip2em \texttt{finalize\_decision(}$\mathit{qc}$\texttt{)} \label{line:invoke_finalize_decision}
\end{algorithmic}
\end{algorithm} 




\subsection{Proof of Correctness}
We now prove the correctness of \rare.
In order to do so, we need to prove that the view synchronizer ensures eventual synchronization time.
%\name (\cref{algorithm:view_1,algorithm:view_2,algorithm:synchronizer}) satisfies validity, termination and agreement.
Whenever we reference lines of the pseudocode in the rest of the subsection, we refer to the lines of \Cref{algorithm:synchronizer} (if not explicitly stated otherwise).
We say that process $P_i$ enters in view $v$ of epoch $e$ at time $t$ if it triggers $\texttt{advance}(global\_view)$ at time $t$ for variables $global\_view = (e-1) \cdot (f+1) + v$. If $v=1$, we say that $P_i$ enters in epoch $e$ (line~\ref{line:start_view_1}, \ref{line:start_view_2}). 
%We say that process $P_i$ enters in epoch $e$ (resp. in view $v$ of epoch $e$) at time $t$ if it triggers $\texttt{advance}(sync\_epoch, sync\_view)$ for variables $sync\_epoch = e $ and $sync\_view = 1$ (resp. $sync\_view = v$) at time $t$.

%\subsubsection{Eventual Synchronization Time}

%% old presentation with decision
\iffalse
First, we prove that all correct processes decide if a correct process decides.

\pierre{This following lemma concerns the view executor, which is a problem for modularity. In fact, as currently stated, the View Synchronization does not precisely ensure eventual synchronization time but ensures 1) either termination or 2) eventual synchronization time that then lead to termination. The point is that it is possible for the Byzantine processes to make correct processes agree before reaching a synchronization time. Typically with a Byzantine leader that behaves to ensures termination before synchronization time. }

\green{This lemma has to be removed for modularity}
\begin{lemma} \label{lemma:one_decides_all_decide}
Let a correct process decide a value.
Then, every correct process eventually decides a value.
\end{lemma}
\begin{proof}
Let $P_i$ be the correct process that decides.
Before deciding (line~\ref{line:decide} of \Cref{algorithm:view_2}), $P_i$ disseminates the obtained quorum certificate (line~\ref{line:broadcast_qc} of \Cref{algorithm:view_2}).
Eventually, every correct process receives the broadcast \textsc{decision} message, enters the \texttt{finalize\_decision} function (line~\ref{line:invoke_finalize_decision} \Cref{algorithm:view_2}) and decides (line~\ref{line:decide} \Cref{algorithm:view_2}).
\end{proof}

A correct process $P_i$ \emph{starts} an epoch $e$ (at time $t$) if and only if $P_i$ executes (1) line~\ref{line:start_epoch_1} (at time $t$) in the case of $e = 1$, or (2) line~\ref{line:start_epoch} with $\mathit{sync\_epoch} = e$ (at time $t$) in the case of $e > 1$. 
%% old presentation with termination
\fi

%%% useless lemma
\iffalse
First we prove some basic implications about the execution of some steps of \rare.

\begin{lemma} \label{lemma:basic_implications}
Let a correct process $P_j$ that start an epoch $e>1$ (line~\ref{line:start_view_2}) at time $t$, then 
\begin{compactenum}


\item $P_j$ has broadcast a \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over_complete}) at time $t$. \label{item:basic_1}

\item $P_j$ has received either (i) $2f+1$ \textsc{epoch-over} messages for epoch $e-1$ (line~\ref{line:receive_epoch_over}) or (ii) an \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:receive_epoch_over_complete}) \label{item:basic_2}

\item $f+1$ correct processes have broadcast a \textsc{epoch-over} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over}) \label{item:basic_3} 
\end{compactenum}
\end{lemma}

\begin{proof}
The start of epoch $e$, means 
the execution of line~\ref{line:start_view_2} with $sync\_epoch = e$ which implies the expiration of $sync\_timer$ with variable $sync\_epoch = e$ (\ref{line:sync_timer_expires}) (*). We immediately obtain that $P_j$ has broadcast a \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over_complete}) at time $t$. So item \ref{item:basic_1} holds.
Then (*) implies that either (i) line~\ref{line:sync_timer_measure_2} or (ii) line~\ref{line:sync_timer_measure} has been executed with variable $sync\_epoch = e$. Since this variable $sync\_epoch$ is updated at (i) line~\ref{line:update_epoch_1} and (ii) line~\ref{line:update_epoch_2} to $e'+1$ where $e'$ is the epoch attached to messages received at (i) line \ref{line:receive_epoch_over} or (ii)  line~\ref{line:receive_epoch_over_complete} , then $P_j$ received either (i) 
 $2f+1$ \textsc{epoch-over} messages at line~\ref{line:receive_epoch_over} or (ii) an \textsc{epoch-over-complete} message at line~\ref{line:receive_epoch_over_complete} for epoch $e' = e-1$. 
 Hence item \ref{item:basic_2} holds.

Finally, if item \ref{item:basic_2} (i) holds. Then $P_j$ has received $f+1$ \textsc{epoch-over} message for epoch $e-1$ from $f+1$ correct processes. If item \ref{item:basic_2} (ii) holds, then the received \textsc{epoch-over-complete} contains a threshold signature for $(2f+1)$ \textsc{epoch-over} messages for epoch $e-1$. Here again, $f+1$ \textsc{epoch-over-complete} messages for epoch $e-1$ have been sent by $f+1$ correct processes. In both cases, these messages have been necessarily sent by the execution of line~\ref{line:broadcast_epoch_over} and so $f+1$ correct processes have broadcast an \textsc{epoch-over} message for epoch $e-1$. Thus item \ref{item:basic_3} holds.
This ends the proof.
\end{proof}
%useless lemma
\fi

First, we prove that, if a correct process sends an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}), then the process has previously started $e$.

\begin{lemma} \label{lemma:epoch_over_previously_started}
Let a correct process $P_i$ broadcast an \textsc{epoch-over} message for an epoch $e$ (at line~\ref{line:broadcast_epoch_over}) at some time $t$.
Then, $P_i$ has started $e$ at some time $t' < t$ and the timer $view\_timer$ of $P_i$ expired $f+1$ times between $t'$ and $t$.
\end{lemma}



\begin{proof}
At the moment of broadcasting the message, the following holds: (1) $\mathit{sync\_epoch} = e$ at $P_i$, and (2) $\mathit{sync\_view} = f + 1$ at $P_i$.
Therefore, all $f + 1$ views of the epoch $e$ have expired. %(otherwise, $P_i$ would have decided at line~\ref{line:decide} and stopped executing the protocol at line~\ref{line:stop_all_events}). %
%Hence, the first (out of the aforementioned $f + 1$) view of the epoch $e$ expired. If $e=1$, the result is immediate since process $P_i$ triggers $\texttt{advance}(1,1)$ at its starting time $t^s_i$.
%
When the first (out of the aforementioned $f + 1$) view started at time $t'$ (at line~\ref{line:start_view_1} or at line~\ref{line:start_view_2}), the epoch $e$ has started at the same time $t'$  (by same line~\ref{line:start_view_1} or line~\ref{line:start_view_2}).
Moreover, the epoch $e$ has started before the broadcasting of the message since, for each view of the epoch, $\mathit{view\_timer}$ measures $\mathit{view\_duration}$ time (line~\ref{line:view_timer_measure_without_msg_exchange} for views from index $2$  to index $f+1$ and line \ref{line:view_timer_measure} or \ref{line:view_timer_measure_first_view} for first view of the epoch) and we assume that the timer expires after some non-zero real time when measuring $\mathit{view\_duration}$ (even before $\mathit{GST}$).
% Therefore, the lemma holds.
\end{proof}


%%% useless lemma
\iffalse
Next, we prove that, if an epoch $e > 1$ is started by a correct process at some time $t$, then epoch $e - 1$ is started by a (potentially different) correct process at some time $t' < t$. 

\begin{lemma} \label{lemma:epoch_previously_started}
Let a correct process start an epoch $e > 1$ at time $t$.
Then, epoch $e - 1$ is started by a correct process at some time $t' < t$. 
\end{lemma}
\begin{proof}
Let a correct process $P_i$ start an epoch $e > 1$ at time $t$.
That means that $P_i$ executes line~\ref{line:start_view_2} at time $t$.
Hence, either the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} has been previously activated at process $P_i$.
Therefore, (at least) $f + 1$ correct processes have sent an $\textsc{epoch-over}$ message for $e - 1$ before time $t$.
By \Cref{lemma:epoch_over_previously_started}, these correct processes have started epoch $e - 1$ before sending the \textsc{epoch-over} messages, which concludes the proof.
\end{proof}
\fi
%% useless lemma

The next lemma shows that, all epochs are eventually started. 
In other words, correct processes keep transiting to new epochs forever.

\begin{lemma} \label{lemma:no_decision_constantly_next_epoch}
Every epoch $e \in \mathbb{N}$ is eventually started by a correct process. 
\end{lemma}

\begin{proof}
Epoch $1$ is started by a correct process since every correct process initially starts the epoch (at line~\ref{line:start_view_1}, upon executing the \texttt{start} rule).
Therefore, it is left to prove that all epochs greater than $1$ are started by a correct process.
By contradiction, let $e_h \in \mathbb{N}$ be the highest epoch that is ever started by a correct process, where $e_h \geq 1$.

Since, no epoch $e'>e_h$ is never started by a correct process, (**) no correct process ever received neither (i) $2f+1$ \textsc{epoch-over} messages nor (ii) an \textsc{epoch-over-complete} message, for epoch $e''\geq e_h$ . Indeed, the contrary would mean that a correct process either (1) enters in epoch $e_h+1$ after $sync\_timer$ expiration or (2) receives either (i) $2f+1$ \textsc{epoch-over} messages nor (ii) an \textsc{epoch-over-complete} message, for epoch $e' > e_h$. Case (1) is excluded by assumption. The case (2) would mean that a correct process would have sent an \textsc{epoch-over} message for epoch $e'>e_h$ and by 
\Cref{lemma:epoch_over_previously_started}, would have started an epoch $e'>e_h$. Hence case (2) is also excluded, which lead us to (**).

We can deduce that all the correct processes will eventually enter in epoch $e_h$. Let us explain: if $e_h = 1$, this is immediate since every correct process eventually start the protocol. If $e_h>1$,
the start of epoch $e_h$, means 
the execution of line~\ref{line:start_view_2} with $sync\_epoch = e_h$ which implies that $P_j$ has broadcast a \textsc{epoch-over-complete} message for epoch $e_h-1$ (line~\ref{line:broadcast_epoch_over_complete}) just before
 This message will be eventually received and so all the correct processes will eventually enter in epoch $e_h$, either by line~\ref{line:receive_epoch_over} or line~\ref{line:receive_epoch_over_complete}, while (**) ensures theses lines \ref{line:receive_epoch_over} and \ref{line:receive_epoch_over_complete} are not executed for a greater epoch $e'-1>e_h-1$. 
Thereafter, by assumption, all the correct processes will stay in $e_h$ forever.
Finally, the $view\_timer$ will expire $f+1$ times in epoch $e_h$ for every correct process with variable $sync\_view$ reaching $f+1$. Indeed, (**) prevents $sync\_view$ to be reset to 1. This lead to the broadcast of $2f+1$ \textsc{epoch-over} messages by as many correct processes at line~\ref{line:broadcast_epoch_over}. These messages will be eventually received by correct processes, which is in contradiction with (**). 
This concludes the proof.


\end{proof}

%%old proof
\iffalse
\begin{proof}
Epoch $1$ is started by a correct process since every correct process initially starts the epoch (at line~\ref{line:start_view_1}, upon executing the \texttt{start} rule).
Therefore, it is left to prove that all epochs greater than $1$ are started by a correct process.

By contradiction, let $e + 1 \in \mathbb{N}$ be the smallest epoch that is never started by a correct process, where $e \geq 1$.

\Cref{lemma:epoch_previously_started} shows that no epoch $e' > e + 1$ is ever started by a correct process \pierre{(1) Why do we need lemma 2 for this claim ? By assumption, $e+1$ is the smallest epoch never started by a correct process. (2) If indeed lemma 2 is useless, then it can be removed since it is never reused again. }.

Since epochs greater than $e$ are never started, no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$ (by \Cref{lemma:epoch_over_previously_started}).
\pierre{\Cref{lemma:epoch_over_previously_started} claims that the sent of \textsc{epoch-over} message for an epoch $e' > e$ means the start of $e'$ by a correct process. So no start of $e'$, implies no \textsc{epoch-over} message for an epoch $e' > e$ but does not implie this result for $e$ (at least not immediately)}
\pierre{I guess we can just show that if $e$ is started and no greater epoch $e'$ is never started, then eventually the \textsc{epoch-over} message is bcast by all correct processes and we reach a contradiction. Thus we do not use neither lemma 1 or lemma 2}

Hence, the $\mathit{sync\_epoch}$ variable at a correct process cannot contain a value greater than $e + 1$ (see the rules at lines~\ref{line:receive_epoch_over} and~\ref{line:receive_epoch_over_complete}).
Moreover, if the $\mathit{sync\_epoch}$ variable at a correct process becomes $e + 1$ (at line~\ref{line:update_epoch_1} or at line~\ref{line:update_epoch_2}), the epoch $e + 1$ is started at that process because (1) \textsc{epoch-over} messages are not sent for epochs greater than $e$, and (2) $\mathit{sync\_timer}$ eventually expires (and the rule at line~\ref{line:sync_timer_expires} activates).
Given that epoch $e + 1$ is never started, no correct process sets its $\mathit{sync\_epoch}$ variable to $e + 1$.

Since epoch $e$ is started by a correct process, every correct process eventually sets its $\mathit{sync\_epoch}$ variable to $e$: (1) if $e = 1$, that happens as soon as the process starts executing the protocol, or (2) otherwise, every correct process receives an \textsc{epoch-over-complete} message for $e - 1$ and, since the $\mathit{sync\_epoch}$ variable cannot have a value greater than $e$, starts $e$ eventually.
Given that no correct process ever sends an \textsc{epoch-over} message for an epoch $e' > e$,  $view\_timer$ expires for every correct process for each view of the epoch $e$ (line~\ref{line:rule_view_expired}).
Once that happens, a correct process broadcasts an \textsc{epoch-over} message for the epoch $e$ (line~\ref{line:broadcast_epoch_over}).
Therefore, once a correct process receives the \textsc{epoch-over} messages from all correct processes (and the rule at line~\ref{line:receive_epoch_over} activates), the process updates its $\mathit{sync\_epoch}$ variable to $e + 1$ (at line~\ref{line:update_epoch_1}).
Hence, we reach contradiction and the lemma holds.
\end{proof}
%%old proof
\fi

The following lemma proves that, if the first correct process to start an epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ before time $t + \mathit{epoch\_duration}$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{view\_duration}$.


\begin{lemma} \label{lemma:no_epoch_over_for_epoch_duration}
Let $t$ be time such that (1) $t \geq \mathit{GST}$ and (2) no correct process has started $e$ before time $t$.
Then, no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) before time $t + \mathit{epoch\_duration}$.
\end{lemma}

\begin{proof}
Let $t_e$ be the first time a correct process, noted $P_j$, sends an \textsc{epoch-over} message for an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) (if $t_e$ does not exists, the lemma holds immediately).
By \Cref{lemma:epoch_over_previously_started}, $P_j$ started epoch $e'$ at time $t'<t_e$ and the timer $view\_timer$ of $P_i$ expired $f+1$ times between $t'$ and $t_e$. By precondition of the  \Cref{lemma:no_epoch_over_for_epoch_duration}, $GST \leq t \leq t'$. Since there is no clock drift after GST and $t'\geq GST$,  $(f+1)\cdot view\_duration$ elapses between $t'$ and $t_e$. Hence no  correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ before time $t + \mathit{epoch\_duration}$, where $\mathit{epoch\_duration} = (f + 1) \cdot \mathit{view\_duration}$. The lemma holds.
\end{proof}


%old proof 
\iffalse
\begin{proof}
First, no correct process sends an \textsc{epoch-over} message for epoch $e$ before time $t + \mathit{epoch\_duration}$ since the first process to start $e$ does so at time $t \geq \mathit{GST}$.
Therefore, epoch $e + 1$ cannot be started by a correct process by time $t + \mathit{epoch\_duration}$.

By contradiction, suppose that a correct process sends an \textsc{epoch-over} message for an epoch $e' > e$ before time $t + \mathit{epoch\_duration}$.
By \cref{lemma:epoch_over_previously_started,lemma:epoch_previously_started}, epoch $e + 1$ has started before time $t + \mathit{epoch\_duration}$, which is a contradiction with the fact that epoch $e + 1$ does not start by time $t + \mathit{epoch\_duration}$.
Therefore, the lemma stands.
\end{proof}
\fi
%old proof

\Cref{lemma:no_epoch_over_for_epoch_duration} has the following consequence: if the first correct process that starts a new epoch $e$ does so at time $t \geq \mathit{GST}$, then no correct process ``leaves'' epoch $e$ by time $t + \mathit{epoch\_duration}$.

\paragraph*{Notation}

Let us fix an execution of the View Synchronizer \rare.
We note:
\begin{compactitem}
\item  $e_{\mathit{max}}$: the highest epoch started by a correct process by time $\mathit{GST}$.
\item $t_{\mathit{final}}$: the first time such that a correct process starts epoch $e_{\mathit{max}} + 1$, i. e. a time such that: 
\begin{compactenum}
\item  a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and 
\item no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.
    
\end{compactenum}

\end{compactitem}

Note that $t_{\mathit{final}}$ exists (by \Cref{lemma:no_decision_constantly_next_epoch}) and $t_{\mathit{final}} > \mathit{GST}$.


Finally, we prove that \rare ensures the eventual synchronization time property.

\begin{theorem} [Eventual Synchronization Time] \label{theorem:termination}
\rare (\Cref{algorithm:synchronizer}) ensures eventual synchronization time which is reached by time $t_{\mathit{final}} + \mathit{epoch\_duration}$, i.e. by time $GST + 2 \cdot \mathit{epoch\_duration}$ %(which means \name satisfies termination).
\end{theorem}
\begin{proof}
%\st{We prove the theorem by contradiction.} \st{Let there exist a correct process $P_i$ that never decides.} \st{By lemma 18, if a correct process decides, all correct processes (including $P_i$) decide. Therefore, no correct process decides.}

%\st{Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$. Let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$.}
%\st{Note that $t_{\mathit{final}}$ exists (by lemma 21) and $t_{\mathit{final}} > \mathit{GST}$.}
The \Cref{lemma:no_epoch_over_for_epoch_duration} guarantees that no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e_{\mathit{max}} + 1$ before time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
    
Next, the rule at line~\ref{line:receive_epoch_over} or the rule at line~\ref{line:receive_epoch_over_complete} is activated at each correct process by time $t_{\mathit{final}} + \delta$ (recall that $t_{\mathit{final}} > \mathit{GST}$).
Hence, every correct process starts the epoch $e_{\mathit{max}} + 1$ by time $t_{\mathit{final}} + 2\delta$ (due to the $\mathit{sync\_timer}$).
    
Finally, in each view of the epoch $e_{\mathit{max}} + 1$, all correct processes overlap for (at least) $8\delta$ time (given that $\mathit{view\_duration} = 10\delta$ and the biggest ``delay'' between epoch starts is $2\delta$ (recall that hardware clocks of processes do not drift after $\mathit{GST}$).
Given that (1) at least one view of the epoch $e_{\mathit{max}} + 1$ has a correct leader (since there are $f + 1$ views in $e_{\mathit{max}} + 1$), %\st{(2) $8\delta$ time is sufficient for a decision in each view of the epoch $e_{\mathit{max}} + 1$ after the last correct process has started the view (if the view has a correct leader)}, 
and (2) the last correct process starts the $(f + 1)$-st view of the epoch by time $t_{\mathit{final}} + f\cdot\mathit{view\_duration} + 2\delta$, %\st{every correct process decides}
synchronization time is reached by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
%\pierre{The following sentence can be removed: Recall that the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} is activated only after all received messages of the view protocol have been processed, which implies that, in a view of the epoch with a correct leader, the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} is not activated at a correct process before the process decides\footnote{Observe that, in the case the correct process decides, the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} will never get activated because of line~\ref{line:stop_all_events} of \Cref{algorithm:synchronizer}.}.}
%Therefore, we reach a contradiction with the fact that no correct process decides, which implies that termination is satisfied by \name.
% \end{compactenum}
% Termination is satisfied by \name.
\end{proof}

\subsection{Communication complexity.}
First, we show that each process sends at most $O(n)$ words within any epoch.
Formally, we say that a correct process $P_i$ is \emph{in epoch $e$} between the time $t$ when it starts $e$ and the time $t'$ when it starts some other epoch.
If it does not start some other epoch, $P_i$ remains in $e$ forever.

\begin{lemma} \label{lemma:linear_in_an_epoch}
For any epoch $e$ and any correct process $P_i$, process $P_i$ sends at most $O(n)$ words while being in $e$.
\end{lemma}
\begin{proof}
Let us consider all messages that $P_i$ can send while being in epoch $e$:
\begin{compactitem}
    \item \textsc{decision} messages (sent at line~\ref{line:broadcast_qc}):
    These messages are sent by $P_i$ only once throughout any execution (i.e., line~\ref{line:broadcast_qc} is executed at most once).
    Given that each messages contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{decision} messages while being in epoch $e$.
    
    \item \textsc{epoch-over} messages (sent at line~\ref{line:broadcast_epoch_over}):
    These messages are sent by $P_i$ only once while $P_i$ is in $e$, since it requires a $view\_timer$ expiration that can append only after the execution of line \ref{line:view_timer_measure} that immediately precedes the execution of line \ref{line:start_view_2} which triggers the start of a new epoch.
    
    %\pierre{TO CORRECT} since the next \texttt{start\_view} event is triggered at line~\ref{line:start_view_2}, which implies that the new epoch has started (line~\ref{line:start_epoch}).
    Given that each \textsc{epoch-over} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over} messages while being in $e$.
    
    \item \textsc{epoch-over-complete} messages (sent at line~\ref{line:broadcast_epoch_over_complete}):
    These messages are sent by $P_i$ only once\footnote{Formally speaking, these messages can be sent twice while $P_i$ is in $e$: the first time when it starts $e$ (recall that local computation takes zero time) and the second time when it starts some other epoch. However, it is important that these messages are sent \emph{constant} number of times in $e$.} while $P_i$ is in $e$ because upon the expiration of the $\mathit{sync\_timer}$ (at line~\ref{line:sync_timer_expires}) $P_i$ starts a new epoch (at line~\ref{line:start_view_2}).
    Given that each \textsc{epoch-over-complete} message contains a single word, $P_i$ sends (at most) $O(n)$ words via the \textsc{epoch-over-complete} messages while being in $e$.
    
    \item Messages of \Cref{algorithm:view_1}:
    While in $e$, $P_i$ executes at most $f + 1$ views\footnote{Again, it can happen that the process executes $f + 2$ views while in $e$: $f + 1$ views of the epoch $e$ and the first view of the new epoch. However, at most $O(n)$ words are sent by $P_i$ within these $f + 2$ views.}.
    If $P_i$ is the leader of a view, it sends (at most) $O(n)$ words; otherwise, it sends $O(1)$ words.
    Given that, while in $e$, $P_i$ is the leader of (at most) one view and $f = O(n)$, it sends (at most) $O(n)$ words via the messages of a view (i.e., of \Cref{algorithm:view_1}).
\end{compactitem}
While in $e$, $P_i$ sends at most $O(n)$ words via the messages of each type, which concludes the lemma.
\end{proof}

Next, we show that, within any period of $\delta$ time after $\mathit{GST}$, a correct process can be in (at most) two epochs.

\begin{lemma} \label{lemma:within_delta}
Let $\mathcal{P} = [t_1, t_2]$ denote a time period such that $t_1 \geq \mathit{GST}$ and $t_2 - t_1 \leq \delta$.
Consider any correct process $P_i$.
Then, $P_i$ can be in at most two epochs within $\mathcal{P}$.
\end{lemma}
\begin{proof}
Let $P_i$ start an epoch $e$ at some time $t_e \geq \mathit{GST}$.
Assume that $P_i$ starts another epoch $e'$ at some time $t_{e'} > t_e$.
Due to the fact that (1) $e'$ is started at line~\ref{line:start_view_2}, and (2) $\mathit{sync\_timer}$ measures $\delta$ time (it is recalled that there is no clock drift after GST), then $t_{e'} - t_e \geq \delta$.
The lemma holds.
\end{proof}

%Let $e_{\mathit{max}}$ denote the highest epoch started by a correct process by time $\mathit{GST}$ (as in the proof of \Cref{theorem:termination}). Moreover, let $t_{\mathit{final}}$ denote the time such that (1) a correct process starts epoch $e_{\mathit{max}} + 1$ at time $t_{\mathit{final}}$, and (2) no correct process has started $e_{\mathit{max}} + 1$ before time $t_{\mathit{final}}$. Note that $t_{\mathit{final}}$ is not defined if no correct process ever starts epoch $e_{\mathit{max}} + 1$. The next lemma shows that every correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ (if $t_{\mathit{final}}$ is defined).

%\begin{lemma} \label{lemma:all_decide_by_t_final_epoch}
%Let $t_{\mathit{final}}$ be defined (i.e., let there exist a correct process that starts epoch $e_{\mathit{max}} + 1$).Then, \st{all correct processes decide} \blue{synchronization time is reached} by time $t_{\mathit{final}} + \mathit{epoch\_duration}$.
%\end{lemma}
%\begin{proof}
%The proof of this lemma follows the same argument as the proof of \Cref{theorem:termination}.\st{If a correct process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$, every process decides by time $t_{\mathit{final}} + \mathit{epoch\_duration}$ and the lemma holds.} \st{Otherwise,} there is a view $v$ of epoch $e_{\mathit{max}} + 1$ s. t. the leader of this view is correct. \st{the last view of epoch $e_{\mathit{max}} + 1$ is correct (if that was not the case, a correct process would decide in a view preceding this one, which means that a correct process would decide by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$).} Moreover, the leader has sent the \textsc{decide} message (at line~\ref{line:broadcast_decide_message} of \Cref{algorithm:view_1}) by time $t_{\mathit{final}} + \mathit{epoch\_duration} - \delta$. Once a correct process receives this message, which happens by time $t_{\mathit{final}} + \mathit{epoch\_duration}$, it decides.The lemma holds.
%\end{proof}

The next lemma shows that no correct process ever starts any epoch greater than $e_{\mathit{max}} + 1$ before synchronization time.
This lemma is the consequence of \Cref{lemma:no_epoch_over_for_epoch_duration} and \Cref{theorem:termination}.

\begin{lemma} \label{lemma:no_process_starts_emax_1}
No correct process starts an epoch $e > e_{\mathit{max}} + 1$ before synchronization time. 
\end{lemma}
\begin{proof}
By \Cref{lemma:no_epoch_over_for_epoch_duration}, no correct process sends an \textsc{epoch-over} message for an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) before time $t + \mathit{epoch\_duration}$. Hence,
no correct process start an epoch $e' \geq e$ (at line~\ref{line:broadcast_epoch_over}) before time $t + \mathit{epoch\_duration}$.
Moreover, by \Cref{theorem:termination}, synchronization time is reached by time $t + \mathit{epoch\_duration}$. 
%By contradiction, suppose that a correct process starts an epoch $e > e_{\mathit{max}} + 1$ before synchronization time. Therefore, a correct process has sent an \textsc{epoch-over} message for $e_{\mathit{max}} + 1$ before synchronization time. However, this is impossible due to \Cref{lemma:all_decide_by_t_final_epoch} 
%\pierre{TO REMOVE OR TO ADAPT (recall that the rule at line~\ref{line:upon_view_timer} of \Cref{algorithm:view_2} activates only after all ``view-specific'' messages; see line~\ref{line:rule} of \Cref{algorithm:view_2}).}
The lemma holds.
\end{proof}

Finally we are able to bound the number of views visited between $GST$ and synchronization time.

\begin{lemma} \label{lemma:constant-number-of-epochs-after-GST}
No correct process visit more than $O(1)$ epochs between GST and synchronization time.
\end{lemma}

\begin{proof}
By time $\mathit{GST} + \delta$, each process receives an \textsc{epoch-over-complete} message for epoch $e_{\mathit{max}} - 1$ .
Hence, before time $\mathit{GST} + 3\delta$ each correct process starts either epoch $e_{\mathit{max}}$ or $e_{\mathit{max}} + 1$.
Let us explain: a correct process $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}} - 1$ at time $\mathit{GST} + \delta$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}}$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; just before time $\mathit{GST} + 2\delta$, $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}}$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}} + 1$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; therefore, before time $\mathit{GST} + 3\delta$, $P_i$ starts $e_{\mathit{max}} + 1$.


Let us fix a correct process $P_i$.
By time $\mathit{GST} + 3\delta$, $P_i$ starts either epoch $e_{\mathit{max}}$ or epoch $e_{\mathit{max}} + 1$ (because of the argument given above).
By \Cref{lemma:no_process_starts_emax_1}, $P_i$ never starts an epoch greater than $e_{\mathit{max}} + 1$ before synchronization time.
During $3\delta$ time period, $P_i$ can be in (at most) $6$ epochs (by \Cref{lemma:within_delta}); afterwards, $P_i$ can be in two epochs ($e_{\mathit{max}}$ and $e_{\mathit{max}} + 1$).
Hence process $P_i$ does not visit more than $O(1)$ epochs and the lemma holds. (In fact, we could have shown that, between $GST$ an synchronization time, $P_i$ cannot visit more than 2 epochs and 2 views, but this refinement is not necessary for the lemma).
\end{proof}

As a corollary, we directly obtain the communication complexity of \name.

\begin{theorem} [Communication complexity]
\name has $O(n^2)$ communication complexity.
\end{theorem}
\begin{proof}
%By time $\mathit{GST} + \delta$, each process receives an \textsc{epoch-over-complete} message for epoch $e_{\mathit{max}} - 1$ . Hence, before time $\mathit{GST} + 3\delta$ each correct process starts either epoch $e_{\mathit{max}}$ or $e_{\mathit{max}} + 1$. Let us explain: a correct process $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}} - 1$ at time $\mathit{GST} + \delta$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}}$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; just before time $\mathit{GST} + 2\delta$, $P_i$ receives an \textsc{epoch-over-complete} message for $e_{\mathit{max}}$, sets its $\mathit{sync\_epoch}$ variable to $e_{\mathit{max}} + 1$ and sets $\mathit{sync\_timer}$ to measure $\delta$ time; therefore, before time $\mathit{GST} + 3\delta$, $P_i$ starts $e_{\mathit{max}} + 1$. Let us fix a correct process $P_i$. By time $\mathit{GST} + 3\delta$, $P_i$ starts either epoch $e_{\mathit{max}}$ or epoch $e_{\mathit{max}} + 1$ (because of the argument given above). By \Cref{lemma:no_process_starts_emax_1}, $P_i$ never starts an epoch greater than $e_{\mathit{max}} + 1$ before synchronization time. During $3\delta$ time period, $P_i$ can be in (at most) $6$ epochs (by \Cref{lemma:within_delta}); afterwards, $P_i$ can be in two epochs ($e_{\mathit{max}}$ and $e_{\mathit{max}} + 1$).
Since it sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}), and that $P_i$ visit at most $O(1)$ epochs between $\mathit{GST}$ and synchronization time (by \Cref{lemma:constant-number-of-epochs-after-GST}), $P_i$ sends at most $O(n)$ words between $\mathit{GST}$ and synchronization time.
Therefore, the communication complexity of \name is indeed $O(n^2)$.
\end{proof}

\subsection{\name}

\medskip
\noindent \textbf{Composition.}
Finally, \Cref{algorithm:composition} shows how the view core and the view synchronizer components collaborate in order to solve Byzantine consensus.

\begin{algorithm}
\caption{Core + Synchronizer = Byzantine Consensus}
\label{algorithm:composition}
\begin{multicols}{2}
\begin{algorithmic} [1]
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\texttt{Core.}\mathsf{init(}\mathit{proposal}\mathsf{)}$

\medskip
\State \textbf{upon} $\texttt{Synchronizer.}\mathsf{advance(}v\mathsf{)}$:
\State \hskip2em $\texttt{Core.}\mathsf{start(}v\mathsf{)}$

\columnbreak
\medskip
\State \textbf{upon} $\texttt{Core.}\mathsf{decide(}v\mathsf{)}$:
\State \hskip2em \textbf{trigger} $\mathsf{decide(}v\mathsf{)}$
\end{algorithmic}
\end{multicols}
\end{algorithm} 

We prove the correctness and the complexity of \Cref{algorithm:composition}.

\begin{theorem} \label{theorem:quad-solves-consensus} \name
(\Cref{algorithm:composition}) solves the Byzantine consensus problem with $O(n^2)$ worst-case communication complexity and $O(f\cdot \delta)$ worst-case latency complexity.
\end{theorem}
\begin{proof}
The safety properties of Byzantine consensus follows directly from the safety properties of the core module. The termination comes from the eventual view synchronization property of the view synchronizer component.
By lemma \ref{lemma:constant-number-of-epochs-after-GST}, no correct process visit more than $O(1)$ epochs.

Since a correct process sends at most $O(n)$ words within every epoch (by \Cref{lemma:linear_in_an_epoch}) of the synchronizer module, and at most $O(n)$ words within every epoch of the core module, by using Hotstuff core protocol, the worst-case communication complexity of \name is $O(n^2)$.

Moreover, the duration of an epoch is $(f+1)\cdot (c_s+2) \cdot \delta$, which means the worst-case latency complexity is $O(f \cdot \delta)$. 
The theorem holds.

For sake of completeness, the pseudo-code of HotStuff can be found in the appendix.

\end{proof}

%% merged into one unique theorem
\iffalse
Finally, we prove the complexity of \Cref{algorithm:composition}.

\begin{theorem}
The communication complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{com\_per\_view} + \mathit{sync\_com}$.The latency complexity of \Cref{algorithm:composition} is $\mathit{num\_views} \cdot \mathit{latency\_per\_view} + \mathit{sync\_latency}$.
\end{theorem}

\fi
%merge into one unique theorem

\subsection{Adding strong validity to \name}

The actual \name protocol only ensures weak validity (if all processes are correct and a process decides value $w$, then value $w$ is proposed by a correct process) but does not ensure \emph{strong validity}: If all correct processes propose the same value $w$, then $w$ is decided. In this subsection, we add a groundwork step before \name to obtain \namebis that solves consensus with strong validity, quadratic worst-case communication complexity and linear worst-case latency complexity.

\subsubsection{Implementation of \namebis}

We assume another $(k', n)$-threshold signature scheme~\cite{LJY16}, where $k' = f + 1$ (and not $2f+1$). In the remaining, \name is used in a black-box fashion, so we use the same names $ShareSign$, $ShareVerify$, $Combine$, $Verify$ for the $(k', n)$-threshold signature without fearing any ambiguity with the $(2f+1, n)$-threshold signature used in \name.

 The basic idea is to propose and accept only values that are \emph{legitimate}, in the sense that deciding one of them cannot violate strong validity. Hence a groundwork is added to know what are the legitimate values. At first round of the groundwork, every correct process send its (signed) proposal. If a process $p$ does not receive $f+1$ times the same proposal, it knows that any value $w$ could be decided safely. A naive solution could consist in broadcasting $2f+1$ signed proposals, s. t. eventually, every correct process knows that any value $w$ could be decided safely. But it would induce a $O(n^3)$ communication complexity. We adapt this idea with some optimization to reach a $O(n^2)$ communication complexity. The groundwork pseudo-code is presented in \ref{algorithm:groundwork} and counts 3 rounds that are presented here.
 \begin{enumerate}
     \item PROPOSAL: every process $i$ send its partially-signed proposal $[PROPOSAL, proposal_i]_{\sigma_i}$ (line \ref{line-gw:bcast-proposal}).
     
     \item ECHO: Upon the reception of $2f+1$ proposals (line \ref{line-gw:proposal-reception}), a process deals with two possible situations:
     \begin{enumerate}
         \item It did not receive more than $f$ times the same proposal (line \ref{line-gw:not-same-proposals}). It knows that any value can be safely decided. To inform other processes, it broadcasts a message $[ECHO, \bot]_{\sigma_i}$ (line \ref{line-gw:claim-not-same-proposals} and \ref{line-gw:bcast-echo}).
         
         \item It received $f+1$ times the same proposal $w$ (line \ref{line-gw:same-proposals}). Potentially, it could be the only legitimate  value to decide. To inform the other processes, it broadcast a message $[ECHO, \sigma]$ where $\sigma$ is the $(f+1)$-threshold signature of message $[PROPOSAL, w]$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). 
          \end{enumerate}
     
     \item JUSTIFICATION: Upon the reception of $2f+1$ echo messages, a process deals with two possible situations:
     \begin{enumerate}
     \item It receives $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$ (line \ref{line-gw:uniform-claim-not-same-proposals}).
     The process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts a message $[JUSTIFICATION, \sigma]$ where $\sigma$
 is the $(f+1)$-threshold signature of message $[ECHO, \bot]$ (line \ref{line-gw:certify-uniform-claim-not-same-proposals} and \ref{line-gw:bcast-justification}). 
 
 \item It does not receive $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$. Here again, two possibilities: 
 \begin{enumerate}
     \item it receives $m_x = [ECHO, \sigma_x]$ and $m_y = [ECHO, \sigma_y]$ that justifies two different values $x$ and $y$ (line \ref{line-gw:at-least-two-different proposals}). Since at least two different correct processes proposed two different values, the process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts $[JUSTIFICATION, (m_x, m_y)]$ (line \ref{line-gw:certify-at-least-two-different-proposals} and \ref{line-gw:bcast-justification-2}).
     \item it receives only message of the form $m_w = [ECHO, \sigma_w]$ that justifies $w$ (line \ref{line-gw:all-processes-consider-value-legitimate}) (with $Verify([PROPOSAL,w], \sigma_w)==true$) . In that case, all the correct processes also receive $[ECHO, \sigma_w]$ and thus knows that $w$ can be decided safely. Moreover, it updates its proposal to $w$ before starting \name (line \ref{line-gw:update-proposal-upon-same-proposals}). 
 \end{enumerate}
     \end{enumerate}
     
     \item Later, a message $m$ legitimates a value $w$ iff it is a well-formed JUSTIFICATION message or if $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$. %either (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
 %(2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
 %(3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$. 
 Upon the reception of the first JUSTIFICATION message, it is broadcast in order to ensure uniformity, i. e. if a value is considered legitimate by a correct process, it is considered legitimate by all correct processes by time $GST + \delta$.
     It is worthy to note that if no justification message is sent by a correct process, it means it is in case 3) b) ii) which means that every correct process receives a message $[ECHO, \sigma_w]$  s.t. $Verify([PROPOSAL, w], \sigma_w)$.
 \end{enumerate}
 
 The pseudo-code of \namebis is presented in algorithms \ref{algorithm:groundwork} and \ref{algorithm:wrapper-for-strong-validity}.

\begin{algorithm} 
\caption{GroundWork: Pseudocode for process $P_i$}
\label{algorithm:groundwork}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm}

\State \hskip2em $certified \gets \emptyset$

\medskip

\State \hskip2em $m^p.\mathit{type} \gets PROPOSAL$
\State \hskip2em $m^p.\mathit{proposal} \gets proposal_i$
\State \hskip2em $m^p.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m^p.\mathit{type}, m^p.\mathit{proposal}])$
\State \hskip2em \texttt{broadcast} $m^p$ \label{line-gw:bcast-proposal}

\medskip

%%%Rcving Phase proposal
\State \hskip2em \textbf{wait for } $2f + 1$ proposals: $M \gets \{m'|m'.type = PROPOSAL\}$.  \label{line-gw:proposal-reception}
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m', m'' \in M', m'.\mathit{proposal} = m''.proposal$: \label{line-gw:same-proposals}

\State \hskip4em $m^e.\mathit{cert} \gets Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-same-proposals}
%\State \hskip4em $proposal_i \gets w$ where $Verify([Proposal, w], m^e.\mathit{cert})$ \label{line-gw:update-proposal-upon-same-proposals}
\State \hskip2em \textbf{else } \label{line-gw:not-same-proposals} 
\State \hskip4em $m^e.\mathit{cert} \gets \bot$ \label{line-gw:claim-not-same-proposals}

\State \hskip2em $m^e.\mathit{type} \gets ECHO$
\State \hskip2em $m^e.\mathit{partial\_sig} \gets ShareSign_i([m^e.\mathit{type}, m^e.\mathit{cert}])$

\State \hskip2em \texttt{broadcast} $m^e$ \label{line-gw:bcast-echo}

\medskip
%%%
\State \hskip2em \textbf{wait for } $2f + 1$ echo messages: $M \gets \{m'|m'.type = ECHO\}$.
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m' \in M', m'.\mathit{cert} = \bot$: \label{line-gw:uniform-claim-not-same-proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-uniform-claim-not-same-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification}

\State \hskip2em \textbf{else if}: $\exists m_x, m_y \in M$ s. t. $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ with $x \neq y$ \label{line-gw:at-least-two-different proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $\{m_x, m_y\}$ \label{line-gw:certify-at-least-two-different-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification-2}


\State \hskip2em \textbf{else}: \label{line-gw:all-processes-consider-value-legitimate}

\State \hskip4em $proposal_i \gets w$ where  $Verify([PROPOSAL, w], m'.cert)$ for some $m' \in M$ \label{line-gw:update-proposal-upon-same-proposals}

\State \hskip2em \textbf{trigger} \texttt{terminate\_GroundWork}

\medskip

%%%Uniformity Phase
\State \textbf{upon} first reception of a message $m$ with $m.type = JUSTIFICATION$
\State \hskip2em \texttt{broadcast} $m$ if it is not already done \label{line-gw:forward-justification}

%\medskip

%\State \textbf{upon} reception of a message $m$ with $m.type = ECHO$ and $Verify([ECHO, x], m.cert)$
%\State \hskip2em $certified \gets certified \cup \{x\}$
%\State \hskip2em \textbf{if} $|certified| \leq 2$:
%\State \hskip4em \texttt{broadcast} $m$

\medskip
%Utility

\State \textbf{function} \texttt{legitimate}(\texttt{Message} $m$, \texttt{Integer} $w$):
\State \hskip2em \textbf{if} either
\State \hskip4em (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
\State \hskip4em (2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
\State \hskip4em (3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$:
\State \hskip6em \textbf{return} true

\State \hskip2em \textbf{else}
\State \hskip4em \textbf{return} false



\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{\namebis: Pseudocode for process $P_i$}
\label{algorithm:wrapper-for-strong-validity}
\begin{algorithmic} [1]
\State \texttt{start} GroundWork
\State \textbf{upon} \texttt{terminate\_GroundWork}: \State \hskip2em \texttt{start} \name where a proposal $w$ is ignored in the PREPARE phase of any view iff no message $m$ s. t. $\texttt{legitimate}(m, w)$ has been delivered 
\end{algorithmic}
\end{algorithm}

\subsubsection{Proof of correctness of \namebis}

Here we prove the correctness of the algorithm \namebis.

\begin{lemma}[Validity]\label{lemma:sv-validity}
If all correct processes proposes the same value $w$, then
\begin{enumerate}
    \item every correct process receives (immediately from itself) a message $m = [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$
    \item No correct process delivers $M$ s. t. $\texttt{legitimate}(M, x)$ with $x \neq w$
\end{enumerate}
 
\end{lemma}

\begin{proof}
They are at least $2f+1$ broadcast of  messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:bcast-proposal}). Hence, every correct process receives $f+1$ messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:same-proposals}) and hence sends  $ [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). This implies the item (1) of the lemma.
Moreover, the $f$ remaining processes cannot neither compute $ [ECHO, \sigma']$ with $Verify([PROPOSAL, x], \sigma')$ with $x \neq w$ nor compute $[JUSTIFICATION, \sigma_{\bot}]$ with $Verify([ECHO, \bot], \sigma_{\bot})$, since the threshold-scheme requires at least $f+1$ different share-signatures. 



\end{proof}

\begin{lemma}[Uniformity]\label{lemma:sv-uniformity}
If a correct process delivers $m$ by time $t$ s. t. $\texttt{legitimate}(m, w)$, then every correct process eventually receives $m'$ s. t. $\texttt{legitimate}(m', w)$ by time $max(GST, t) + \delta$.
\end{lemma}

\begin{proof}
Let $p$ be a correct process that terminates the GroundWork.
Necessarily, $p$ enter either in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or in line \ref{line-gw:all-processes-consider-value-legitimate}. In first case, $p$ broadcast a JUSTIFICATION message (lines \ref{line-gw:certify-uniform-claim-not-same-proposals}and  \ref{line-gw:bcast-justification} or lines \ref{line-gw:certify-at-least-two-different-proposals} and  \ref{line-gw:bcast-justification-2} ) that legitimates all possible values. 
By justification's forwarding  (line \ref{line-gw:forward-justification}), if a justification message is received by a correct process by time $t$, then a justification message is received by each correct process by time $max(GST, t) + \delta$.
The only way to avoid that every correct process obtain a justification message before $GST + \delta$ is if all correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate}. But it is impossible that two correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate} for two different values. Hence they enter in line \ref{line-gw:all-processes-consider-value-legitimate} for one unique value $w$, which means they all received a message $m = [ECHO, \sigma_w]$ with $Verify([PROPOSAL, w], \sigma_w)$, which ends the proof.
\end{proof}



\begin{lemma}[Obligation]\label{lemma:sv-obligation}
After GST, for every correct leader $p$, its proposal is not ignored.  
\end{lemma}

\begin{proof}
Case 1: the proposal is its own proposal in \name.

This proposal has been chosen according to received messages in the groundWork algorithm.
$p$ entered either (i) in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or (ii) in line \ref{line-gw:all-processes-consider-value-legitimate}.
In case (i), a JUSTIFICATION message will be received by every correct process by time $GST + \delta$.
In case (ii), the proposal has been updated to the relevant value so that every correct process receives $(ECHO, \sigma_w)$ with $Verify([PROPOSAL, w], \sigma_w)$.

Case 2: its proposal comes from the delivered $2f+1$ VIEW-CHANGE messages.

A VIEW-CHANGE message, encapsulates necessarily a value considered legitimate by at least $f+1$ correct processes by the quorum certificate.  The lemma holds by lemma \ref{lemma:sv-uniformity}.  
\end{proof}

\begin{lemma}[$O(n^2)$ complexity]\label{lemma:sv-complexity}
The communication complexity of the GroundWork algorithm is $O(n^2)$
\end{lemma}

\begin{proof}
Every correct process broadcast only one PROPOSAL message, one ECHO message and at most one JUSTIFICATION message where each message contains no more than ine threshold-signature and no more than share-signature.
\end{proof}

\begin{theorem}[Strong Validity]
 \namebis solves Byzantine consensus with strong validity, $O(n^2)$ communication complexity and $O(f\cdot\delta)$ latency complexity. 
\end{theorem}

\begin{proof}
 The strong validity is ensured by lemma \ref{lemma:sv-validity}. The liveness of the algorithm is preserved by lemma \ref{lemma:sv-obligation}. The quadratic communication complexity is ensured by lemma \ref{lemma:sv-complexity} and theorem \ref{theorem:quad-solves-consensus}.
 The latency complexity is ensured by theorem \ref{theorem:quad-solves-consensus}, since the groundwork only add 3 additional asynchronous rounds.
\end{proof}


%\subsubsection{Eventual Synchronization Time}

%% old presentation with decision
\iffalse
First, we prove that all correct processes decide if a correct process decides.

\pierre{This following lemma concerns the view executor, which is a problem for modularity. In fact, as currently stated, the View Synchronization does not precisely ensure eventual synchronization time but ensures 1) either termination or 2) eventual synchronization time that then lead to termination. The point is that it is possible for the Byzantine processes to make correct processes agree before reaching a synchronization time. Typically with a Byzantine leader that behaves to ensures termination before synchronization time. }

\green{This lemma has to be removed for modularity}
\begin{lemma} \label{lemma:one_decides_all_decide}
Let a correct process decide a value.
Then, every correct process eventually decides a value.
\end{lemma}
\begin{proof}
Let $P_i$ be the correct process that decides.
Before deciding (line~\ref{line:decide} of \Cref{algorithm:view_2}), $P_i$ disseminates the obtained quorum certificate (line~\ref{line:broadcast_qc} of \Cref{algorithm:view_2}).
Eventually, every correct process receives the broadcast \textsc{decision} message, enters the \texttt{finalize\_decision} function (line~\ref{line:invoke_finalize_decision} \Cref{algorithm:view_2}) and decides (line~\ref{line:decide} \Cref{algorithm:view_2}).
\end{proof}

A correct process $P_i$ \emph{starts} an epoch $e$ (at time $t$) if and only if $P_i$ executes (1) line~\ref{line:start_epoch_1} (at time $t$) in the case of $e = 1$, or (2) line~\ref{line:start_epoch} with $\mathit{sync\_epoch} = e$ (at time $t$) in the case of $e > 1$. 
%% old presentation with termination
\fi

%%% useless lemma
\iffalse
First we prove some basic implications about the execution of some steps of \rare.

\begin{lemma} \label{lemma:basic_implications}
Let a correct process $P_j$ that start an epoch $e>1$ (line~\ref{line:start_view_2}) at time $t$, then 
\begin{compactenum}


\item $P_j$ has broadcast a \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over_complete}) at time $t$. \label{item:basic_1}

\item $P_j$ has received either (i) $2f+1$ \textsc{epoch-over} messages for epoch $e-1$ (line~\ref{line:receive_epoch_over}) or (ii) an \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:receive_epoch_over_complete}) \label{item:basic_2}

\item $f+1$ correct processes have broadcast a \textsc{epoch-over} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over}) \label{item:basic_3} 
\end{compactenum}
\end{lemma}

\begin{proof}
The start of epoch $e$, means 
the execution of line~\ref{line:start_view_2} with $sync\_epoch = e$ which implies the expiration of $sync\_timer$ with variable $sync\_epoch = e$ (\ref{line:sync_timer_expires}) (*). We immediately obtain that $P_j$ has broadcast a \textsc{epoch-over-complete} message for epoch $e-1$ (line~\ref{line:broadcast_epoch_over_complete}) at time $t$. So item \ref{item:basic_1} holds.
Then (*) implies that either (i) line~\ref{line:sync_timer_measure_2} or (ii) line~\ref{line:sync_timer_measure} has been executed with variable $sync\_epoch = e$. Since this variable $sync\_epoch$ is updated at (i) line~\ref{line:update_epoch_1} and (ii) line~\ref{line:update_epoch_2} to $e'+1$ where $e'$ is the epoch attached to messages received at (i) line \ref{line:receive_epoch_over} or (ii)  line~\ref{line:receive_epoch_over_complete} , then $P_j$ received either (i) 
 $2f+1$ \textsc{epoch-over} messages at line~\ref{line:receive_epoch_over} or (ii) an \textsc{epoch-over-complete} message at line~\ref{line:receive_epoch_over_complete} for epoch $e' = e-1$. 
 Hence item \ref{item:basic_2} holds.

Finally, if item \ref{item:basic_2} (i) holds. Then $P_j$ has received $f+1$ \textsc{epoch-over} message for epoch $e-1$ from $f+1$ correct processes. If item \ref{item:basic_2} (ii) holds, then the received \textsc{epoch-over-complete} contains a threshold signature for $(2f+1)$ \textsc{epoch-over} messages for epoch $e-1$. Here again, $f+1$ \textsc{epoch-over-complete} messages for epoch $e-1$ have been sent by $f+1$ correct processes. In both cases, these messages have been necessarily sent by the execution of line~\ref{line:broadcast_epoch_over} and so $f+1$ correct processes have broadcast an \textsc{epoch-over} message for epoch $e-1$. Thus item \ref{item:basic_3} holds.
This ends the proof.
\end{proof}
%useless lemma
\fi

==> deterministic.tex <==

\section{Deterministic Solution to the Grid Coloring Game}

\emph{Note: this is just a sketch to capture my current thoughts. Everything here needs to be explained better, along with added correctness.}

Recall the grid coloring problem is as follows:
\begin{itemize}
    \item There exists a 2-dimensional grid that has $n$ columns and $n$ rows.
    \item The problem is to assign a color from the set $\colors \triangleq \{1, \ldots n\}$ to each cell in the grid. 
    \item For a given coloring $c$ and a given subset $B \subseteq \colors$, the value of column $j$ is $V_c(B, j)$ is the $y$-index of the first cell in column $j$ that is not assigned a color in $B$.
    \item For a given coloring $c$ and a given subset $B \subseteq \colors$, the value of the coloring $V_c(B)$ is the sum of the values of the columns.
    \item The score of a coloring $\mathit{score}(f)$ is the maximum value of the coloring for any set $B \subseteq \colors$ where $|B| \leq f$.
\end{itemize}

Our overall goal is to show the following theorem: 
\begin{theorem}
We give a solution to the grid coloring problem where for every value of $f$ (simultaneously) the score of the grid coloring game is $O(f \log{n}\log(f)^{\log\log{f}}$. 
\end{theorem}

\subsection{Extractors and Dispersers}

In this section, we review the definitions of extractors and their connection to bipartite graphs. 

\begin{definition}
For a random variable $X$, define the \emph{min-entropy} of $X$ to be the maximum value $k$ such that for all $x$ in the support of $X$, $\Pr{[X = x]} \leq 1/2^k$.
\end{definition}

\iffalse
Example: 5 outcomes with probability: $1/4, 1/6, 1/6, 1/6, 1/4$

min-entropy = 2

Flat random variable:

n outcomes: $\{1, 2, 3, 4, ..., 2^k, 2^k+1, 2^k+2, ..., n\}$

Choose items ${1, ..., 2^k}$ with probability $1/2^k$.  Ignore everything bigger than item $2^k$.  (Actually, fix any $2^k$ items to choose uniformly, while everything else is 0.)

Flat random variable has min-entropy $k$.  

Arbitrary min-entropy $k$ variable $X$ can be represented as a sum of flat random variables:  $X = \sum{X_i}$ where each $X_i is \{1, ..., 2^k\}$ flat.
\fi

For the remainder of this subsection, fix integer values $L$, $R$, and $D$, and let $\ell = \log{(L)}$, $r = \log{(R)}$, and $d = \log{(D)}$.   Fix an error parameter $\epsilon < 1$.

A randomness extractor is a function that takes as input an $\ell$-bit value that is \emph{somewhat random} (i.e., has a given min-entropy), along with a $d$ bit input that is uniformly random.  It outputs an $r$-bit value that is close to uniformly random.  More formally:
\begin{definition}
A $(k, \epsilon)$ extractor is a function $E(x,y) : 2^{\ell} \times 2^{d} \to 2^{r}$ that satisfies the following property: if $x$ is chosen from a distribution with min-entropy $k$ and $y$ is chosen uniformly at random, then $|E(x,y) - U_r| \leq \epsilon$, where $U_r$ is the uniform distribution on $r$ bits and the distance measure is the total variation distance.
\end{definition}

\iffalse
E(x,y)

x: random variable with min-entropy k, n bits  (ideal: would be min-entropy log(n) ==> uniform distribution)
y: uniform random d bits 

output: (1-epsilon) distance from uniform, m bits

(Ideal: m = n?  m = k+d: k bits of min-entropy, added d bits, so k+d-o(1) out seems optimal.)


\fi

An extractor can also be used to define a bipartite graph: assume graph $G$ has $L$ left nodes and $R$ right nodes, and each left node in $L$ has degree $D$.  Then for a left node $u \in L$, for $j \in [1, \ldots D]$, we add an edges $(u, E(u, j)]$ connecting $u$ to the right node determined by the extractor.

For a set of left nodes $U \subseteq L$, we define the right neighbors of $U$ to be $N(U) = \{v~:~u \in U,~(u,v) \in G_E\}$.  The bipartite graph associated with a $(k, \epsilon)$ extractor has a very strong ``expansion'' property:
\begin{lemma}
Let $E(x,y)$ be a $(k, \epsilon)$ extractor, and let $G_E$ be the bipartite graph associated with $E$.  Then graph $G_E$ has the following property: for every subset of left nodes $U \subseteq L$ where $|U| = 2^k$, the right neighbors of $U$ consist of at least $R(1-\epsilon)$ nodes, i.e., $|N(U)| \geq (1-\epsilon)R$.
\end{lemma}

\pierre{Has this lemma a name ?}


\iffalse
E: n bit input, d-bit input

Define bipartite (multi)graph:

$2^n$ left nodes: each input is associated with one left node 
degree $2^d$ for each left node

$2^m$ right nodes: one right node for each output

left node $x$ is connected right node $E(x, j)$ for $j = 1 \ldots 2^d$

Adversary chooses a set of $k$ (left) nodes.  (Flat min-entropy $k$ random variable.)
Choose a left node uniformly at random from the subset of size $k$.
Choose an outgoing edge at random.  (uniform random variable)
==> (bad translation of the statistical distance property) (need right definition) each of the right nodes is reached with probability $(1-\epsilon)(1/2^m)$
(The exactly probability here depends on our definition of statistical distance.)

==> Each set of $k$ left nodes has at least $(1-\epsilon)2^m$ right nodes as neighbors.

Disperser:

A $(k, \epsilon)$ disperer is a function $D(x,y) : 2^{\ell} \times 2^{d} \to 2^{r}$ that satisfies the following property: if $x$ is chosen from a distribution with min-entropy $k$ and $y$ is chosen uniformly at random, then $D(x,y)$ has at least $(1-\epsilon)2^r$ distinct outputs.

==> this is good enough to get our bipartite graph property

\fi


\iffalse

See the disperser construction in this paper:
\texttt{https://yuanz.web.illinois.edu/papers/dispersers.pdf}

I think dispersers have the same useful property as extractors in this case, i.e., that they imply graphs with good expansion.  (Why is this?  You can think of a source with $k$ min-entropy as consisting of a set $S$ of $k$ items of which one is chosen uniformly at random.  That is, a $k$ min-entropy source is equivalent, in some sense, to choose a set of $k$ left nodes and choosing one at random.  The disperser then randomly selects one of the neighbors of the chosen node, and says that the support of the distribution is large.  But if the support of the distribution is large, that means there must be many possible right nodes that can be hit!)

Theorem from the paper above:
For all $\ell$, $k$, and constant $\epsilon$, there exists an explicit $(k,\epsilon)$-strong disperser $D : 2^{\ell} \times 2^d \to 2^r$  with $d = O(\log n)$ and $r = k - 3\log{\ell}+O(1)$.

(One way to think about this: $2^k$ is the number of grid squares chosen by adversary and $2^r$ number of colors.)

In this case, we can set $\ell = 2\log{n}$, $r = \log{f} + 1$, and $k = \log{f} + 3\log\log{n} + O(1)$.  This yields a graph with $d = O(\log\log{n})$, and hence degree $O(\log{n})$.  The left set size of interest is $2^k = Cf\log^3{n}$, so any set of size $Cf\log^3{n}$ should have at least $(1-\epsilon)2f$ right neighbors.

\fi


\subsection{Constructing a Good Bipartite Graph}

\iffalse

The above works for only one value of $f$.  But we can combine $\log(t)$ graphs with:

$f = 1, 2, 4, 8, 16, 32, \ldots, n/3$

To get a graph that works for all values.  At worst, that increases the degree by $\log(n)$.

(The goal is to say that a left set of size $x$ has at least $x/2$ right neighbors.  So combining graphs doesn't hurt.  Adding an edge never removes a right neighbor.

What if we have 6 failures?  Treat 6 failures as 4.  More generally, treat $f$ failures as hyperfloor(f)
Why is this ok?  
If there are 6 failures, then certainly there 4 failures, which means that we have 2 right neighbors.
If there are f failures, then there must be hyperfloor(f) failures, and so we have hyperfloor(f/2) right neighbors ==> good enough.



\fi

In this section, we construct a bipartite graph with $n^2$ left nodes (which will later correspond to grid cells), $n$ right nodes (that will later correspond to colors), and a strong expansion property that we can use to bound the cost of the coloring game.

We first recall an existing extractor construction.  For every $\ell, k$, for every $\epsilon < 1$, there exist explicit extractors with the following parameters:
\begin{itemize}
    \item $d = \log{n} + \log^2{k}$ \pierre{it is $D = \log{n} + \log^2{k}$ right ?}
    \item $r = k + d - 2\log(1/\epsilon) - O(1)$
\end{itemize}

We use this existing construction to build a family of bipartite graphs.  For $f \leq n/3$, we define the bipartite graph $G(n, f)$ to be the graph associated with the following extractor:
\begin{itemize}
    \item $L = n^2$, $\ell = 2\log{n}$.
    \item $k = \log(f) + 1$, $2^k = 2f \leq 2n/3$.
    \item $\epsilon = 1/3$.
    \item $R = 2f$, $r = \log(f) + \log^2\log{n} - O(1) \leq n$. Note that $2^r \geq 2f$ (for sufficiently large $n$).
    \item $d = \log\log{n} + \log^2\log(2f) + C$ for some constant $C$.
\end{itemize}

(Note: we have to be careful to get these parameters right.)

That is, this produces a graph with $n^2$ left nodes, at least $2f$ right nodes (at most $n$ right nodes), and degree $O(\log{n}\log(2f)^{\log\log{f}})$.  This graph has the property that every set of at least $2f$ left nodes has at least $f+1$ right neighbors.

Finally, we combine $\log{n}$ versions of this graph to build our final bipartite graph $G$ as follows:
\begin{itemize}
    \item There are $n^2$ left nodes $\{1, \ldots, n^2\}$.
    \item There are $n$ right nodes $\{1, \ldots, n\}$.
    \item Add an edges $(u,v)$ if for some $i \leq \log{n}-1$, graph $G(n, 2^i)$ contains edge $(u, v)$.  (Notice that graph $G(n, 2^i)$ may have fewer right nodes, but we can map the right nodes of $G(n, 2^i)$ to the first $2^i$ right nodes of $G$.)
\end{itemize}

This final graph $G$ has degree $\log^2{n}\log(2f)^{\log\log{f}}$, and it has the property that for every value of $f < n/3$, every set of at least $2f$ left nodes has at least $f+1$ right neighbors. (TODO: there is a problem with the parameters here: we lost a factor of 2 in constructing $G$.  Need to back and fix.)

\iffalse
    Some catch here: for expander graph from extractor to work, $l$, $r$, $d$, and $k$ have to be an integer. also, for the construction to work, we also need to ensure $|R| \leq n = 3f+1$ ($n=$ number of processes/colors). in other words, $r < \log{f} + c$ for some constant $c$.
    
    On the 2nd result from \url{https://people.seas.harvard.edu/~salil/research/PVcondenser-jacm.pdf}, $d = \log{l} + \log^2{k}$ and $r = k + d - O(1)$. If we use $k = \log{f}$ and $l = 2 \log{n}$, then $r = \log{f} + \log{\log{n}} + \log^2{\log{f}} - O(1)$. For large enough $n$, I think eventually $r$ will be larger than the threshold, and thus the number of processes or colors we need will be more that what we have.
    
    For the first result, $d = \log{l} + \log{k}$ and $r = (1-\alpha)k$ for arbitrary constant $\alpha \in (0, 1)$.  We can set $k = \log{f}+1$, $l = 2 \log{n}$, and $\alpha = 0.01$ (make it arbitrarily close to 1, so $2^r \approx 2f$). This might work? But not as good as the 2nd result. The degree still $polylog(f)$ though.
    
    this one also looks promising: Theorem 1.7 from \url{https://www.cs.utexas.edu/~diz/Sub Websites/Research/Lossless_condensers_unbalanced_expanders_and_extractors.pdf}. There is explicit $(K, (1-\epsilon)D)$ expander for $D = 2^{O(\log{\log{L}}^2)}$ and $R = 2^{O(k/\epsilon)}$. If we set $k = \log{f}+1, \epsilon=0.99$, then $R$ can be at most $3f+1 = n$? this is big O though, but the idea is that there should be a constant which works. note that this is expander, so the guarantee holds for all subset of size \textbf{at most} $K$.
\fi

\subsection{Coloring the grid.}

Let $D$ be the degree of the final bipartite graph created in the last subsection.  We can now color the grid as follows: divide each column into at most $n/D + 1$ chunks of size $D$.  (If it does not divide evenly, the last chunk may have $< D$ cells.) There are at most $n^2$ such chunks, so map each chunk to a left node in the final bipartite graph.  If a chunk maps to left node $u$, color cell $i$ the chunk according to the $i$th outgoing edge of $G$ \pierre{of $u$ ?}.

By construction, for any value $f$, if we take $2f$ chunks, they will have at least $f+1$ colors.  However there is one final step: dealing with grid selections that do not respect chunk boundaries.

For a fixed $f$, assume that we are given the first $c_1$ cells in column 1, $c_2$ cells in column 2, $c_3$ cells in column 3, etc., so that $\sum_j c_j = 4(f+1)D$.  For column $j$ there are two cases to consider: $c_j < D$ (and hence does not even include one complete chunk), and $c_j \geq D$ (and hence includes at least one chunk).

Since there can be at most $f+1$ views, we know there are at most $f+1$ columns, and hence at most $f+1$ columns of type 1.  This will add a cost of at most $(f+1)D$.  The remaining columns of type 2 contain at least $3(f+1)D$ cells.  For each such column, remove the last incomplete chunk.  This yields a total remaining area of at least $2(f+1)D$, all of which is contained in complete chunks.  By the property of the construction, these cells will contain at least $(f+1)$ colors.

Thus we conclude that any given column area that contains at most $f$ colors has area $O(fD)$, i.e., $O(f \log(n) \log(f)^{\log\log(f)})$.

\iffalse
    if we only care about exact $f$: for each column, take the first $n*D$ cells, and divide them into $n$ chunks of size $D$. take any non-taken node from left set of the expander graph, then color the cells by using the edges of the node (i.e color the $i$-th node in the chunk with the color connected by the $i$-th edge of that node). So now we have $(f+1)n$ chunks.
    
    The maximum cells that can be taken without having $K$ full chunks are $(K-1)D + (f+1)(D-1)$. So, the minimum cells that guaranteed to have $K$ full chunks are $KD + f(D-1)$. as we can set $K$ to be $O(f)$, the number of cells will be $O(fD) = O(f \cdot polylog(f))$
\fi

\pierre{Did I understand ? Let $c$ be a coloring, $B \subset \colors$, $|B| \leq f$ and $D \in \mathbb{N}$. The area  covered by the adversary is $\mathrm{Area} = \sum_{j \in [1:n]}V_{c}(B,j)$. For each $j \in [1,n]$, we can note $V_{c}(B,j) = x_j\cdot D + y_j$ with $y_j \in [0,D-1]$. Thus, $\mathrm{Area} =  \sum_{j \in [1:n]}y_j + D\cdot (\sum_{j \in [1:n]}x_j)$, that is $\mathrm{Area} \leq  n(D-1) + D\cdot X$ where the number of complete chunks chosen by the adversary is $X = (\sum_{j \in [1:n]}x_j)$. It seems it is possible to have $D$ quite small (e.g. $D = \tilde{O}(1)$). So, if we neglect this factor, we can focus on $X$. 

The adversary can choose only $|B|=f$ different colors. So the trick is to use an extractor with a good expansion property s.t. for any selection of $X=K$ chunks, it boils down to the selection of $A \cdot K$ colors where $A$ is the factor attached to the expansion. Finally, we have to fine-tune the parameters $A$ and $D$ to minimize the final $\mathrm{Area}$. 

1st problem: $A = (1-\epsilon)\frac{|\colors|}{K}$ depends on the exact number $K$ of chunks selected by the adversary. Since the coloring has to be chosen in advance, then the extractor has to be chosen in advance, so $K$ has to be chosen in advance. The solution will not be perfectly adaptive. A more adaptive solution would require a $(\leq K, A)$ vertex expander graph that probably does not exists with the good parameters. We can alleviate this issue with this technique of merging the family of $log(n)$ bipartite graphs. This induces a "non-adaptive" factor of $log(n)$ but the remaining factors are "adaptive" (depending on $f$ only).
}

\subsection{Notes}

\begin{itemize}
    \item Dispersers may yield a better bound than extractors.  We might be able to get rid of the exponential term (but we would still have a polylog term).
    \item Need to fix the parameters and the constants to make things work.  The parameters here aren't quite right (see https://www.cs.cmu.edu/~venkatg/pubs/papers/PV-condenser.pdf, page 5), and the constants aren't quite right to get the $f+1$ claim.
    \item There is an issue with my claim that a column assignment can't have more than $f+1$ columns.  There is no reason as given that this should be true.  It may be that we want to color the bottom row in the grid with horizontal chunks of size $D$, so that any set of columns that includes at least $2f$ columns will necessarily include at least $f+1$ colors.
\end{itemize}



==> probabilistic.tex <==


\section{Adaptive View Synchronizer}

\iffalse
Things we need to do:
(1) Relate the view synchronization to grid coloring game
(2) Write a better version of the existential result
(3) If we can, write a constructive version (using one of the approaches we've talked about today)
(4) Implications
\fi

\subsection{View Synchronization}

"Leader-based" consensus protocols typically operate in views, where in each view, there is a designated leader whose job is to drive the system to reach a decision. If a process does not decide within a view, the process will try again in the next view, and so on. Eventually, when all processes are in the same view with a correct leader for a sufficiently long time, decision will be made. However, ensuring this overlap is not a trivial task, as process' view can be very far apart.

To this end, usually leader-based consensus protocols consist of two modules: \textit{view core} which job is pick the leader for each view and reach a decision within a view, and \textit{view synchronizer} which responsibility is to help processes to advance into the next view and make all processes overlap in the same view for sufficiently long time. We can summarize the communication complexity as  $\#V \cdot C_v + C_s$, where:

\begin{itemize}
    \item $\#V$ is the number of view the view core executes after GST.
    \item $C_v$ is the communication complexity of the view core within a view.
    \item $C_s$ is the communication complexity of the view synchronizer after GST.
\end{itemize}

In a similar manner, we can also summarize the latency complexity as $\#V \cdot L_v + L_s$, where $L_v$ denotes the latency complexity of the view core within a view and $L_s$ denotes the latency complexity of the view synchronizer after GST.

On the view core part, leader-based protocol such as HotStuff can achieve $\#V = O(f)$, $C_v = O(n)$, and $L_v = O(1)$. However, the complexities are dominated by the view synchronizer, as their protocol achieve $C_s = O(n^3)$ and $C_s = O(n^2)$. Now, the question is whether we can push down the complexity of the view synchronizer.

% ^ just in case we need the definition and motivation

In this section, we present the existence of an adaptive view synchronizer that at the worst case, has the communication complexity of $O(fn \log{f})$ and latency complexity of $O(f \log{f})$, where $f$ is the number of byzantine failures the algorithm can tolerate. Meanwhile, if the actual number of byzantine failures, $t$, is less than $f$, the communication complexity will be $O(tn \log{f})$ and the latency complexity will be $O(t \log{f})$.

First, we explain another view synchronizer which is highly based on the one described in \cite{Naor2020}. Then, we describe a related combinatorial game we refer to as the \textit{grid coloring game}. Finally, we show the existence of a "good" solution to the grid coloring game, which implies the existence of the adaptive view synchronizer.

\subsection{Relay-based View Synchronizer}

In this subsection we will describe the \textit{relay-based} view synchronizer which is largely based on the one described in \cite{Naor2020}. We will only describe the high-level idea, and we defer the technical detail and the correctness proof to the aforementioned paper. We emphasize here that the modification we made will not change the correctness, and they only affect the performance of the protocol. The modification is made to better suit our purposes which will be explained in later parts.

First, recall that the responsibility of a synchronizer is to help processes to advance into the next view and to ensure that after GST, there exists a view in which all correct processes stays in that view for a sufficiently long time. To do this, the synchronizer needs to provide these interfaces:

\begin{compactitem}
    \item \textbf{function} $\mathsf{advance}()$: Advance into the next view.
    \item \textbf{timer}: A timer interface that supports waiting for certain amount of time before triggering expiry signal. The timer can be interrupted at any time.
\end{compactitem}

% high level idea

In several consensus protocol such as HotStuff, the crux is that during the trigger of $\mathsf{advance}$, a broadcast is done in an attempt to make all processes to be at the same view. Thus, this yields an $O(n^2)$ communication complexity. To overcome this, relay-based view synchronizer uses one-to-all and all-to-one communication instead of all-to-all broadcast. Instead of broadcasting the intention to advance, a process will send the advance message to a \textit{relay} process. Once enough advance message has been received, the relay will aggregate the messages, and broadcast the aggregate to all processes. Finally, after receiving the message, a process can advance to a new view. On a normal case, this will yield $O(n)$ communication complexity. However, there are some issues that need to be addressed, specifically when the relay is a byzantine process.

We first define the relay interface which is available to all synchronizer:
\begin{compactitem}
    \item \textbf{function} $\mathsf{relay}(\mathsf{View} \text{ } v \text{, } \mathsf{Int} \text{ } k)$: returns the $k$-th relay on view $v$. The output of this interface will be identical on all correct processes. Lastly, $\mathsf{relay}(v, 1)$ corresponds to the leader of view $v$.
\end{compactitem}

We would like to denote a distinction from the original paper on the requirement of the relay interface. First, the original paper requires for each view, the first $f+1$ relays have to be distinct and all process have equal probability on becoming the relay. We  drop this requirement, and note that this will only affect the complexity, but not the correctness of the protocol. 
Apart from that, we would like to highlight the coupling between view core and synchronizer, in a way that the leader of view $v$ is also the first relay in that view. Here, we assume that the view leader is rotated, i.e the leader of the view $v$ is process $v \mod{n} + 1$ 
% this turns out to be necessary. otherwise, we either
% - set the duration of a round to be somewhat O(f * \delta)
% - set the duration to be constant, but we can only terminate when both the leader and the first relay is correct
% basic idea is: if we decouple, and the first relay is corrupt but the leader is correct, we still cannot achieve synchronization time. the relay can gate a subset of correct processes from entering the view in time

% 2nd high level idea

We then describe how the invocation of $\mathsf{advance}$ goes. Suppose a process wish to advance to view $v$. First, the synchronizer starts the $\mathsf{timer}$, and sends a message to $\mathsf{relay}(v, 1)$. If the relay replies, then the process can advance to the next view as indicated by the relay. Otherwise, at some point, the timer will expire and signal the synchronizer. As the network is reliable, this implies that this relay is byzantine. In this case, the synchronizer then starts the timer again, and sends the message to $\mathsf{relay}(v, 2)$. We repeat this until a relay $\mathsf{relay}(v, k)$ replies for some $k$, in which case the process can finally advance to the next view. 
% technical detail of sending the message

In order to ensure the complexity and correctness, relay cannot simply reply the next view of an individual process. The relay need to aggregate the messages from several processes, and then send messages to all other processes containing the largest possible next view at the moment. Thus, this part consists of several phases:

\begin{enumerate}
    \item \textbf{pre-commit phase}: In this phase, processes in view $v-1$ sends a pre-commit message to the relay. The message contains the intention to advance to the view $v$. After the relay collects $f+1$ such messages, it broadcasts the pre-commit reply message to all processes. % needs f+1 to ensure at least one of them is correct
    \item \textbf{commit phase}: After receiving the pre-commit reply message from the relay, all processes at view $v' < v$ sends a commit message to relay, with intention to advance to the view $v$. After the relay collects $2f+1$ such messages, it broadcasts the commit reply message to all processes. % needs 2f+1 to ensure at least f+1 correct process will enter the next view
    \item \textbf{finalize phase}: Upon receiving the commit reply message, a process at lower view advance to view $v$. However, it is not finished yet. The processes then send a finalize message to the relay. After the relay collects $2f+1$ such messages, it broadcasts the finalize reply message. After receiving the message, a process can safely stays at view $v$. % if we don't get the finalize reply, after timeout we try the next relay instead
\end{enumerate}

% how the execution goes
Then, we describe the overview of an execution of the synchronizer. Recall that the goal of the view synchronization problem is to reach synchronization time. That is, we want to find a view $v$ after GST such that the leader of view $v$ is correct. Whenever a process observe that the leader of the current view $v$ is byzantine, it tries to advance to the next view. It does so invoking $\mathsf{advance}$ on the view synchronization. Then, the synchronization will finish at the first view $v'$ in which the leader is correct. As the leader is rotated, a correct leader must be found among the first $f+1$ view after GST.


The next lemma describes the complexity of relay-based view synchronizer.

% todo(ayaz): check the original paper, if there is something similar there. probably the closest thing is when they describe the expected complexity
\begin{lemma}\label{relay-complexity}
    Let $C_B$ be the number of byzantine relays an execution see throughout the first $f+1$ view after GST. Then, the communication complexity of the relay-based synchronizer will be $O((C_B+f) \cdot n)$ and the latency complexity will be $O(C_B+f)$.
\end{lemma}
\begin{proof}
    Observe that $C_B+f$ is the maximum number of relays a process need to contact throughout the execution. As the communication complexity for one relay is $O(n)$, it follows that the communication complexity will be $O((C_B+f) \cdot n)$. Then, as the time duration before contacting the next relay is a constant, the latency complexity will be $O(C_B+f)$.
\end{proof}

Notice that $C_B$ depends on the $\mathsf{relay}$ function. This brings motivation to find a "good" $\mathsf{relay}$ function which yields a low $C_B$, that implies a low communication and latency complexity. We will show the existence of such good $\mathsf{relay}$ in the next subsections.

\subsection{Grid Coloring Game}

In this subsection, we will describe a combinatorial game we refer to as the \textit{grid coloring game}. Later we will also show how we can relate the relay-based view synchronizer with this game.

The grid coloring game, parameterized by the number of columns $m$, is as follows: The game is played by two players, where we play as the first player. There exists a 2-dimensional grid with $m+1$ columns and infinite rows. Initially, the grid is empty, except for the first row. The cell at the first row of the $j$-th column is already filled with color $j$. The first player then assign each empty cells with a color from the set $\{1, \ldots, 3m+1\}$. For a given coloring $c$, we denote the color of the cell at the $i$-th row and $j$-th column as $c_{ij}$. Then, the second player will pick a set $B \subseteq \{1, \ldots, 3m+1\}$ of size at most $m$. Now, we denote the covered region from a given coloring $c$ and the given set $B$ as the union of the longest prefix from each column, where all the cells' color is contained in $B$. Formally, for a fixed column $j$, the longest prefix is $i$, such that $c_{i'j} \in B$ holds for all $i' \leq i$. An example for the game is depicted in Figure~\ref{fig:grid-coloring-example}. The goal of the second player is to maximize the area of the covered region (the number of cells it contains). Meanwhile, our goal as the first player is to minimize it.

\begin{figure}
    \centering
    \begin{tikzpicture}
        \fill[gray] (0,0) rectangle (1,2);
        \draw (0.5,0.5) node{1};
        \draw (0.5,1.5) node{4};
        \draw (0.5,2.5) node{6};
        \fill[gray] (1,0) rectangle (2,1);
        \draw (1.5,0.5) node{2};
        \draw (1.5,1.5) node{5};
        \draw (1.5,2.5) node{3};
        \draw (2.5,0.5) node{3};
        \draw (2.5,1.5) node{3};
        \draw (2.5,2.5) node{2};
        \fill[gray] (3,0) rectangle (4,2);
        \draw (3.5,0.5) node{4};
        \draw (3.5,1.5) node{1};
        \draw (3.5,2.5) node{7};
        \draw[step=1cm,black,very thin] (0,0) grid (4,3);
        \foreach \i in {0,...,4} {
            \draw [step=1cm,black,very thin] (\i,3) -- (\i,3.8);
        }
        \draw[loosely dotted, thick] (0,4.5) -- (4,4.5);
    \end{tikzpicture}
    \caption{An example of the grid coloring game with $m=3$, and the second player choose $B = \{1, 2, 4\}$. The shaded cells denote the covered region for the given coloring $c$ and set $B$.}
    \label{fig:grid-coloring-example}
\end{figure}

% TODO: is this the best/clearest definition?
% Possible alternate definition:
% Adversary chooses prefix of each column.
% That defines a region of the plane.
% Cost of the game game(f) = maximal sized region so defined with at most f colors.

We demonstrate the relation between the grid coloring game and the view synchronization problem in the following lemma:

\begin{lemma}\label{grid-relay-relation}
    Suppose for a grid coloring game with $f+1$ columns, there exists a coloring with covered region area of $s$. Then, there exists a relay-based view synchronizer which solves the view synchronization problem with up to $f$ byzantine failures and $n=3f+1$ processes. Furthermore, the communication complexity of such synchronizer is $O((s+f) \cdot n)$, and the latency complexity is $O(s+f)$.
\end{lemma}
\begin{proof}
    Notice that the relay-based view synchronizer with $f$ byzantine faults and $n$ processes corresponds to the grid coloring game with $f+1$ columns and $3f+1$ colors. The coloring $c$ corresponds to the $\mathsf{relay}$ function, the set $B$ corresponds to the byzantine processes. Then, the covered region area corresponds to the number of byzantine relays on the first $f+1$ view after GST.  As the covered region area is $s$, by Lemma~\ref{relay-complexity}, the communication complexity will be $O((s+f) \cdot n)$, and the latency complexity will be $O(s+f)$.
\end{proof}

By Lemma~\ref{grid-relay-relation}, we can find a good $\mathsf{relay}$ function by finding a good coloring in the grid coloring game. The next step would be to find the upper bound of the covered region area of a good coloring.

\subsection{Existence of Coloring with $O(m \log{m})$ Area}

In this subsection, we will show the existence of a good coloring with $O(m \log{m})$ area for a grid coloring game with $m+1$ columns and $3m+1$ colors. To do this, we will assign each empty cell a color uniformly at random, i.e, the probability that $c_{ij} = l$ for a fixed color $l$ is $1/(3m+1)$.

We will show that for a fixed set $B$, the probability of a large area is exponentially small. For simplicity, we define $Area_c(B)$ as the covered region area of a given coloring $c$ and a set $B$, and $Area(c)$ as the maximum area of a given coloring $c$ from any set $B$.

\begin{lemma}
For a fixed set $B \subseteq \{1, \ldots, 3m+1\}$ where $|B| \leq m$: $\texttt{Pr}(Area_c(B) > km\log{3m}) \leq (3m+1)^{-m}$, for a fixed constant $k$.
\end{lemma}

A corollary of this lemma is that there exists a good coloring:

\begin{corollary}
    For all sets $B \subseteq \{1, \ldots, 3m+1\}$ where $|B| \leq m$: $\texttt{Pr}(Area_c(B) > km\log{m}) \leq 1/2$. That is, with probability $> 0$, the area is at most $km \log{m}$ for a fixed constant $k$.
\end{corollary}

To analyze the coloring, we associate it with a typical coin-flipping process. First, assume that we have fixed the subset $B$.

The process goes as follows. We start at cell $(2, 1)$ in the grid. When we visit a cell, we flip a coin to determine whether this cell is owned by the adversary or not. Here, "head" means the $c_{ij} \notin B$, and "tail" means otherwise. Another way to view this is that head means the current cell is not owned by the adversary, while tail means the opposite. As we color the cell uniformly at random, the probability that the coin flip will be head is at least $2/3$, while the probability that it will be tail is at most $1/3$. 

If the coin comes up head (the cell is not owned by the adversary), then we move to the $2$nd row of the next column. Otherwise, if the coin comes up tail (the cell is owned by the adversary), we move up one row.

The game ends when we flip exactly $m$ heads. At this point, we have advanced through all the $m$ columns. Here, the number of flips we need before we find $m$ heads is exactly the area of the covered region plus $m$.

Now, we can analyze the game via a typical coin flipping process.

\begin{lemma}\label{few-head-probability}
    Given a coin that outputs head with probability at least $2/3$ and tail with probability at most $1/3$.  Assume we flip the coin $12m \ln{(3m+1)}$ times.  The probability that we will see $\leq m$ heads is $\leq (3m+1)^{-m}$.
\end{lemma}
\begin{proof}
    Let $X_i$ be the indicator random variable for the outcome of the $i$-th flip, where $X_i = 1$ if the $i$-th flip is head, and $X_i = 0$ otherwise. Let $X = \sum(X_i)$. Then, $\texttt{E}[X] = 8m \ln{(3m+1)}$.  Each coin flip is independent. Thus, via Chernoff Bound: $\texttt{Pr}(X  \leq  4m\ln{(3m+1)})  \leq  e^{-8m\ln{(3m+1)}(1/2)^2/2}  \leq  e^{-m\ln{(3m+1)}} \leq (3m+1)^{-m}$.
    
    Thus, the probability that we see fewer than $m$ heads is exponentially small.
\end{proof}

\begin{corollary}\label{good-coloring-existence}
    For all sets $B \subseteq \{1, \ldots, 3m+1\}$ where $|B| \leq m$: $\texttt{Pr}(Area(c) > km\log{m}) < 1$. That is, with probability $> 0$, the area is at most $km\log{m}$, for a fixed constant $k$.
\end{corollary}
\begin{proof}
    For any given set $B$, we know that the probability its area is at least $12m \ln{(3m+1)}$ is at most $(3m+1)^{-m}$.
    There are at most ${3m+1 \choose m} \leq (3m+1)^m$ possible sets $B$ of
    size at most $m$. Thus, by a union bound over all the possible sets $B$, we know that the probability that there exists a failure set $B$ of size at most $m$ where the area is $> 12m \ln{k}$ is $ < (3m+1)^m / (3m+1)^m < 1$. In other words, the probability that the coloring has a area of $\leq 12m \ln{m}$ is $> 0$.
\end{proof}

Thus we have shown that by choosing the coloring at random, the area is $O(m \log{m})$ with probability $> 0$. So we can conclude that there exists a good coloring which area is $O(m \log{m})$.

\subsection{Implications for Byzantine Agreement and Replicated State Machines}

In this subsection, we will describe the implications from the existence of good $\mathsf{relay}$ function. 

We start with another corollary from Lemma~\ref{few-head-probability}, which will help in showing the adaptiveness of the relay-based view algorithm:

\begin{corollary}\label{adaptive-coloring}
    Let $t$ be an integer $\leq m$. For all sets $B \subseteq \{1, \ldots, 3m+1\}$ where $|B| = t$: $\texttt{Pr}(Area(c) > kt\log{m}) < 1$. That is, with probability $> 0$, the area is at most $kt\log{m}$, for a fixed constant $k$.
\end{corollary}
\begin{proof}
    We follow the same argument from Lemma~\ref{few-head-probability} and Corollary~\ref{good-coloring-existence}. However, we change the number of coin flips into $12t \ln{(3m+1)}$. Thus, the probability that we will see $\leq t$ heads will be at most $(3m+1)^{-t}$. Finally, by doing union bound over ${3m+1 \choose t} \leq (3m+1)^t$ different subsets $B$ of size $t$, the probability that the coloring has an area of $\leq 12t \ln{m}$ is $> 0$.
\end{proof}

Thus, we reach the following lemma:

\begin{lemma}\label{adaptive-synchronizer}
    There exists a view synchronizer which solves the view synchronization problem that tolerates up to $f$ byzantine failures. This synchronizer has communication complexity of $O(fn \log{f})$ and latency complexity of $O(f \log{f})$. Furthermore, this synchronizer is adaptive. If there are only $t \leq f$ byzantine failures, the communication complexity will be $O(tn \log{f})$ and the latency complexity will be $O(t \log{f})$.
\end{lemma}
\begin{proof}
    This directly follows by applying Corollary~\ref{good-coloring-existence} and Corollary~\ref{adaptive-coloring} to Lemma~\ref{grid-relay-relation}. As there exists a good coloring in which the area is $O(f \log{f})$ (or $O(t \log{f})$ if there are only $t \leq f$ byzantine failures), Lemma~\ref{grid-relay-relation} implies that there exists a relay-based view synchronizer that at the worst case, has the communication complexity of $O(fn \log{f})$ and latency complexity of $O(f \log{f})$. Meanwhile, if there are only $t \leq f$ byzantine failures, the communication complexity will be $O(tn \log{f})$ and latency complexity of $O(t \log{f})$.
\end{proof}

Finally, we reach the conclusion of this section:

\begin{theorem}
    There exists a protocol that solves the byzantine agreement problem which tolerates up to $f$ byzantine failures. At the worst case, the protocol has communication complexity of $O(fn \log{f})$ and latency complexity of $O(f \log{f})$. Furthermore, the protocol is adaptive. If there are only $t \leq f$ byzantine failures, the communication complexity will be $O(fn + tn \log{f})$, and the latency complexity will be $O(f + t \log{f})$.
\end{theorem}
\begin{proof}
    We use the view core module from HotStuff and view synchronizer from Lemma~\ref{adaptive-synchronizer}. Recall that the view core module from HotStuff have the communication complexity of $O(fn)$ and latency complexity of $O(f)$. It follows that in the worst case, the communication complexity will be $O(fn \log{f})$ and the latency complexity will be $O(f \log{f})$. Meanwhile, if there are only $t \leq f$ byzantine failures, the communication complexity will be $O(fn + tn \log{f})$, and the latency complexity will be $O(f + t \log{f})$.
\end{proof}


\iffalse
% Explain what is view synchronization (maybe copy from other part of the paper, maybe adapt from Naor/Keidar paper.
% Give a view synchronization algorithm (which depends on relays, probably similar to the one in Naor/Keidar).
% ==> try to do something (consensus?)
% ==> if not, try to move to the next view
% ==> if view change fails advance to next relay (which tries to change the view)
% ==> until we find a relax that advances to the new view
% ==> until we find a view where our main task succeeds
% Define the grid coloring game
% Show how solving the grid coloring problem yields an efficient view synchronization algorithm (because grid cells represent relays/leaders). 
% ==> Lemma: if we can solve the grid coloring game in XXX time, then something is true of view synchronization

Here we present a proof sketch to show that there exists an $O(n \log{n})$ solution to the grid coloring problem.  We give an argument via the probabilistic method, which demonstrates (non-constructively) that a good coloring exists.

% This is a brief and probably unclear version of the grid coloring game
% should be more clear, probably
Recall the grid coloring problem is as follows:
\begin{itemize}
    \item There exists a 2-dimensional grid that has $n$ columns (and infinite rows).
    \item The problem is to assign a color from the set $\{1, \ldots 3n\}$ to each cell in the grid. 
    \item For a given coloring $c$ and a given subset $B \subseteq \{1, \ldots, 3n\}$, the value of column $j$ is $V_c(B, j)$ is the $y$-index of the first cell in column $j$ that is not assigned a color in $B$.
    \item For a given coloring $c$ and a given subset $B \subseteq \{1, \ldots, 3n\}$, the value of the coloring $V_c(B)$ is the sum of the values of the columns.
    \item The score of a coloring is the maximum value of the coloring for any set $B \subseteq \{1, \ldots, 3n\}$ where $|B| \leq n$.
\end{itemize}


\subsection{Existential solution to grid coloring}

We will show that there exists a coloring with a score $O(n \log{n})$ via the probabilistic method.  To do this, we assign each cell a color uniformly at random, i.e.,  it is assigned each color with probability $1/3n$. The coloring $c$ is now considered as a random variable.

We will show that for a fixed set $B$, the probability of a large score is exponentially small.
\begin{lemma}
For a fixed set $B \subseteq \{1, \ldots, 3n\}$ where $|B| \leq n$: $\texttt{Pr}(V_c(B) > kn\log{n}) \leq 1/(3n)^n$, for a fixed constant $k$.
\end{lemma}

A corollary of this is that there exists a good coloring:
\begin{corollary}
For all sets $B \subseteq \{1, \ldots, 3n\}$ where $|B| \leq n$: $\texttt{Pr}(V_c(B) > kn\log{n}) \leq 1/2$. That is, with probability $> 0$, the score is $\leq kn\log{n}$, for a fixed constant $k$.  
\end{corollary}
This implies that a good coloring exists via the probabilistic method.  (If no good coloring existed, then the probability of finding one would necessarily be zero!)

To analyze the coloring, we associate it with a typical coin-flipping process.  (Formally, this is a stochastic dominance argument.)  First, assume we have fixed a coloring $B$.

Imagine starting at position $(1, 1)$ in the grid. We flip a coin that comes up ``heads'' with probability $2/3$ and ``tails'' with probability $1/3$.  In the grid, the probability that a cell's color is owned by the adversary is at most the probability the coin comes up tails.  The probability that a cell's color is not owned by the adversary is at least the probability the coin comes up heads.  

If the coin comes up heads (i.e., if the grid cell is not owned by the adversary), then we move to the next column.  If the coin comes up tails (i.e., if the grid cell is owned by the adversary), then we move up one row.

Notice that the game ends when we flip exactly $n$ heads.  At that point, we have advanced through all $n$ columns.  The score for this set $B$ is exactly the number of flips we need before we find $n$ heads.

And so now we can analyze this via a typical coin flipping process:
\begin{lemma}
    Given a coin that outputs heads with probability $2/3$ and tails with probability $1/3$.  Assume we flip the coin $12n \ln{(3n)}$ times.  The probability that we will see $\leq n$ heads is $\leq 1/(3n)^n$.
\end{lemma}
\begin{proof}
Let $X_i$ be the outcome of the $i$th flip, and let $X = \sum(X_i)$.  The expected number of heads flipped is $8n \ln{(3n)}$.  Each coin flip is independent. Thus, by a Chernoff Bound:$\texttt{Pr}(X  \leq  4n\ln{(3n)})  \leq  e^{-8n\ln{(3n)}(1/2)^2/2}  \leq  e^{-n\ln{(3n)}} \leq  1/(3n)^n$

%\begin{eqnarray*}
%$\texttt{Pr}(X & \leq & 4n\ln{(3n)}) & \leq & e^{-8n\ln{(3n)}(1/2)^2/2} \\
%& \leq & e^{-n\ln{(3n)}} \\
%& \leq & 1/(3n)^n$
%\end{eqnarray*}
Thus the probability that we see fewer than $n$ heads is exponentially small.
\end{proof}

\begin{corollary}
For all sets $B \subseteq \{1, \ldots, 3n\}$ where $|B| \leq n$: $\texttt{Pr}(score(c) > kn\log{n}) < 1$. That is, with probability $> 0$, the score is $\leq kn\log{n}$, for a fixed constant $k$.  
\end{corollary}
\begin{proof}
For any given set $B$, we know that the probability its score is $> 24n \ln n$ is at most $1/(3n)^n$.  There are at most $(3n \choose n) < (3n)^n$ possible sets $B$ of size at most $n$.  Thus, by a union bound over all the possible sets $B$, we know that the probability that there exists a failure set $B$ of size at most $n$ where the score is $> 24 n \ln n$ is $ < (3n)^n / (3n)^n < 1$, i.e., the probability that the coloring has a score of $\leq 24n \ln n$ is $> 0$.
\end{proof}

Thus we have shown that choosing the coloring at random, the score is $O(n \log n)$ with probability $> 0$, and so we conclude that there exists a good coloring.


\subsection{Implications for Byzantine Agreement and Replicated State Machines}

% Main theorems:
% We can solve byzantine agreement in this message complexity
% Adaptive BA: if there are f < t failures, then we get message complexity something something
% Replicated state machines / blockchains: ....
\fi

==> sections/discussion.tex <==
\section{Discussion}

\subsection{Obtaining Strong Validity with quadratic communication}

The actual \name protocol only ensures weak validity (if all processes are correct and a process decides $w$, then $w$ is proposed by a correct process) but does not ensure \emph{strong validity}: If all correct processes propose the same value $w$, then $w$ is decided. In this subsection, we add a groundwork step before \name to obtain \namebis that ensures strong validity.

We assume another $(k', n)$-threshold signature scheme~\cite{LJY16}, where $k' = f + 1$ (and not $2f+1$). In the remaining, \name is used in a black-box fashion, so we use the same names $ShareSign$, $ShareVerify$, $Combine$, $Verify$ for the $(k', n)$-threshold signature without fearing any ambiguity with the $(2f+1, n)$-threshold signature used in \name.

 The basic idea is to propose and accept only values that are \emph{legitimate}, in the sense that deciding one of them cannot violate strong validity. Hence a groundwork is added to know what are the legitimate values. At first round of the groundwork, every correct process send its (signed) proposal. If a process $p$ does not receive $f+1$ times the same proposal, it knows that any value $w$ could be decided safely. A naive solution could consist in broadcasting $2f+1$ signed proposals, s. t. eventually, every correct process knows that any value $w$ could be decided safely. But it would induce a $O(n^3)$ communication complexity. We adapt this idea with some optimization to reach a $O(n^2)$ communication complexity. The groundwork pseudo-code is presented in \ref{algorithm:groundwork} and counts 3 rounds that are presented here.
 \begin{enumerate}
     \item PROPOSAL: every process $i$ send its partially-signed proposal $[PROPOSAL, proposal_i]_{\sigma_i}$ (line \ref{line-gw:bcast-proposal}).
     
     \item ECHO: Upon the reception of $2f+1$ proposals (line \ref{line-gw:proposal-reception}), a process deals with two possible situations:
     \begin{enumerate}
         \item It did not receive more than $f$ times the same proposal (line \ref{line-gw:not-same-proposals}). It knows that any value can be safely decided. To inform other processes, it broadcasts a message $[ECHO, \bot]_{\sigma_i}$ (line \ref{line-gw:claim-not-same-proposals} and \ref{line-gw:bcast-echo}).
         
         \item It received $f+1$ times the same proposal $w$ (line \ref{line-gw:same-proposals}). Potentially, it could be the only legitimate  value to decide. To inform the other processes, it broadcast a message $[ECHO, \sigma]$ where $\sigma$ is the $(f+1)$-threshold signature of message $[PROPOSAL, w]$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). 
          \end{enumerate}
     
     \item JUSTIFICATION: Upon the reception of $2f+1$ echo messages, a process deals with two possible situations:
     \begin{enumerate}
     \item It receives $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$ (line \ref{line-gw:uniform-claim-not-same-proposals}).
     The process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts a message $[JUSTIFICATION, \sigma]$ where $\sigma$
 is the $(f+1)$-threshold signature of message $[ECHO, \bot]$ (line \ref{line-gw:certify-uniform-claim-not-same-proposals} and \ref{line-gw:bcast-justification}). 
 
 \item It does not receive $f+1$ messages of the form $[ECHO, \bot]_{\sigma_j}$. Here again, two possibilities: 
 \begin{enumerate}
     \item it receives $m_x = [ECHO, \sigma_x]$ and $m_y = [ECHO, \sigma_y]$ that justifies two different values $x$ and $y$ (line \ref{line-gw:at-least-two-different proposals}). Since at least two different correct processes proposed two different values, the process knows
     that any value can be safely decided, but now, it can prove it with a reasonable cost. To inform other processes, it broadcasts $[JUSTIFICATION, (m_x, m_y)]$ (line \ref{line-gw:certify-at-least-two-different-proposals} and \ref{line-gw:bcast-justification-2}).
     \item it receives only message of the form $m_w = [ECHO, \sigma_w]$ that justifies $w$ ($Verify([PROPOSAL,w], \sigma_w)$) (line \ref{line-gw:all-processes-consider-value-legitimate}). In that case, all the correct processes also receive $[ECHO, \sigma_w]$ and thus knows that $w$ can be decided safely. Moreover, it updates its proposal to $w$ before starting \name (line \ref{line-gw:update-proposal-upon-same-proposals}). 
 \end{enumerate}
     \end{enumerate}
     
     \item Later, a message $m$ legitimates a value $w$ iff it is a well-formed JUSTIFICATION message or if $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$. %either (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
 %(2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
 %(3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$. 
 Upon the reception of the first JUSTIFICATION message, it is broadcast in order to ensure uniformity, i. e. if a value is considered legitimate by a correct process, it is considered legitimate by all correct processes by time $GST + \delta$.
     It is worthy to note that if no justification message is sent by a correct process, it means it is in case 3) b) ii) which means that every correct process receives a message $[ECHO, \sigma_w]$  s.t. $Verify([PROPOSAL, w], \sigma_w)$.
 \end{enumerate}
 
 The pseudo-code of \namebis is presented in algorithms \ref{algorithm:groundwork} and \ref{algorithm:wrapper-for-strong-validity}.

\begin{algorithm} 
\caption{GroundWork: Pseudocode for process $P_i$}
\label{algorithm:groundwork}
\begin{algorithmic} [1]

%Sending Phase proposal
\State \textbf{upon} \texttt{start}: \Comment{start of the algorithm}

\State \hskip2em $certified \gets \emptyset$

\medskip

\State \hskip2em $m^p.\mathit{type} \gets PROPOSAL$
\State \hskip2em $m^p.\mathit{proposal} \gets proposal_i$
\State \hskip2em $m^p.\mathit{partial\_sig} \gets \mathit{ShareSign}_i([m^p.\mathit{type}, m^p.\mathit{proposal}])$
\State \hskip2em \texttt{broadcast} $m^p$ \label{line-gw:bcast-proposal}

\medskip

%%%Rcving Phase proposal
\State \hskip2em \textbf{wait for } $2f + 1$ proposals: $M \gets \{m'|m'.type = PROPOSAL\}$.  \label{line-gw:proposal-reception}
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m', m'' \in M', m'.\mathit{proposal} = m''.proposal$: \label{line-gw:same-proposals}

\State \hskip4em $m^e.\mathit{cert} \gets Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-same-proposals}
%\State \hskip4em $proposal_i \gets w$ where $Verify([Proposal, w], m^e.\mathit{cert})$ \label{line-gw:update-proposal-upon-same-proposals}
\State \hskip2em \textbf{else } \label{line-gw:not-same-proposals} 
\State \hskip4em $m^e.\mathit{cert} \gets \bot$ \label{line-gw:claim-not-same-proposals}

\State \hskip2em $m^e.\mathit{type} \gets ECHO$
\State \hskip2em $m^e.\mathit{partial\_sig} \gets ShareSign_i([m^e.\mathit{type}, m^e.\mathit{cert}])$

\State \hskip2em \texttt{broadcast} $m^e$ \label{line-gw:bcast-echo}

\medskip
%%%
\State \hskip2em \textbf{wait for } $2f + 1$ echo messages: $M \gets \{m'|m'.type = ECHO\}$.
\State \hskip2em \textbf{if } $\exists M' \subset M$, s. t. $\forall m' \in M', m'.\mathit{cert} = \bot$: \label{line-gw:uniform-claim-not-same-proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $Combine(\{m'.\mathit{partial\_sig}| m' \in M'\})$ \label{line-gw:certify-uniform-claim-not-same-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification}

\State \hskip2em \textbf{else if}: $\exists m_x, m_y \in M$ s. t. $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ with $x \neq y$ \label{line-gw:at-least-two-different proposals}

\State \hskip4em $m^j.\mathit{type} \gets$ $JUSTIFICATION$

\State \hskip4em $m^j.\mathit{justification} \gets$ $\{m_x, m_y\}$ \label{line-gw:certify-at-least-two-different-proposals}

\State \hskip4em \texttt{broadcast} $m^j$ \label{line-gw:bcast-justification-2}


\State \hskip2em \textbf{else}: \label{line-gw:all-processes-consider-value-legitimate}

\State \hskip4em $proposal_i \gets w$ where  $Verify([PROPOSAL, w], m'.cert)$ for some $m' \in M$ \label{line-gw:update-proposal-upon-same-proposals}

\State \hskip2em \textbf{trigger} \texttt{terminate\_GroundWork}

\medskip

%%%Uniformity Phase
\State \textbf{upon} first reception of a message $m$ with $m.type = JUSTIFICATION$
\State \hskip2em \texttt{broadcast} $m$ if it is not already done \label{line-gw:forward-justification}

%\medskip

%\State \textbf{upon} reception of a message $m$ with $m.type = ECHO$ and $Verify([ECHO, x], m.cert)$
%\State \hskip2em $certified \gets certified \cup \{x\}$
%\State \hskip2em \textbf{if} $|certified| \leq 2$:
%\State \hskip4em \texttt{broadcast} $m$

\medskip
%Utility

\State \textbf{function} \texttt{legitimate}(\texttt{Message} $m$, \texttt{Integer} $w$):
\State \hskip2em \textbf{if} either
\State \hskip4em (1)  $m = (JUSTIFICATION, \sigma)$ with $Verify([ECHO, \bot], \sigma)$ or 
\State \hskip4em (2)  $m = (ECHO, \sigma)$ with $Verify([PROPOSAL, w], \sigma)$ or
\State \hskip4em (3) $m = ( JUSTIFICATION, \{m_x, m_y\} )$ with $Verify([PROPOSAL, x], m_x.cert)$ and $Verify([PROPOSAL, y], m_y.cert)$ and $x \neq y$:
\State \hskip6em \textbf{return} true

\State \hskip2em \textbf{else}
\State \hskip4em \textbf{return} false



\end{algorithmic}
\end{algorithm}

\begin{algorithm} 
\caption{\namebis: Pseudocode for process $P_i$}
\label{algorithm:wrapper-for-strong-validity}
\begin{algorithmic} [1]
\State \texttt{start} GroundWork
\State \textbf{upon} \texttt{terminate\_GroundWork}: \State \hskip2em \texttt{start} \name where a proposal $w$ is ignored in the PREPARE phase of any view iff no message $m$ s. t. $\texttt{legitimate}(m, w)$ has been delivered 
\end{algorithmic}
\end{algorithm}

\subsubsection{Proof of correctness of \namebis}

Here we prove the correctness of the algorithm \namebis.

\begin{lemma}[Validity]\label{lemma:sv-validity}
If all correct processes proposes the same value $w$, then
\begin{enumerate}
    \item every correct process receives (immediately from itself) a message $m = [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$
    \item No correct process delivers $M$ s. t. $\texttt{legitimate}(M, x)$ with $x \neq w$
\end{enumerate}
 
\end{lemma}

\begin{proof}
They are at least $2f+1$ broadcast of  messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:bcast-proposal}). Hence, every correct process receives $f+1$ messages of the form $[PROPOSAL, w]_{\sigma_j}$ (line \ref{line-gw:same-proposals}) and hence sends  $ [ECHO, \sigma]$ with $Verify([PROPOSAL, w], \sigma)$ (line \ref{line-gw:certify-same-proposals} and \ref{line-gw:bcast-echo}). This implies the item (1) of the lemma.
Moreover, the $f$ remaining processes cannot neither compute $ [ECHO, \sigma']$ with $Verify([PROPOSAL, x], \sigma')$ with $x \neq w$ nor compute $[JUSTIFICATION, \sigma_{\bot}]$ with $Verify([ECHO, \bot], \sigma_{\bot})$, since the threshold-scheme requires at least $f+1$ different share-signatures. 



\end{proof}

\begin{lemma}[Uniformity]\label{lemma:sv-uniformity}
If a correct process delivers $m$ by time $t$ s. t. $\texttt{legitimate}(m, w)$, then every correct process eventually receives $m'$ s. t. $\texttt{legitimate}(m', w)$ by time $max(GST, t) + \delta$.
\end{lemma}

\begin{proof}
Let $p$ be a correct process that terminates the GroundWork.
Necessarily, $p$ enter either in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or in line \ref{line-gw:all-processes-consider-value-legitimate}. In first case, $p$ broadcast a JUSTIFICATION message (lines \ref{line-gw:certify-uniform-claim-not-same-proposals}and  \ref{line-gw:bcast-justification} or lines \ref{line-gw:certify-at-least-two-different-proposals} and  \ref{line-gw:bcast-justification-2} ) that legitimates all possible values. 
By justification's forwarding  (line \ref{line-gw:forward-justification}), if a justification message is received by a correct process by time $t$, then a justification message is received by each correct process by time $max(GST, t) + \delta$.
The only way to avoid that every correct process obtain a justification message before $GST + \delta$ is if all correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate}. But it is impossible that two correct processes enter in line \ref{line-gw:all-processes-consider-value-legitimate} for two different values. Hence they enter in line \ref{line-gw:all-processes-consider-value-legitimate} for one unique value $w$, which means they all received a message $m = [ECHO, \sigma_w]$ with $Verify([PROPOSAL, w], \sigma_w)$, which ends the proof.
\end{proof}



\begin{lemma}[Obligation]\label{lemma:sv-obligation}
After GST, for every correct leader $p$, its proposal is not ignored.  
\end{lemma}

\begin{proof}
Case 1: the proposal is its own proposal in \name.

This proposal has been chosen according to received messages in the groundWork algorithm.
$p$ entered either (i) in line \ref{line-gw:uniform-claim-not-same-proposals} or \ref{line-gw:at-least-two-different proposals} or (ii) in line \ref{line-gw:all-processes-consider-value-legitimate}.
In case (i), a JUSTIFICATION message will be received by every correct process by time $GST + \delta$.
In case (ii), the proposal has been updated to the relevant value so that every correct process receives $(ECHO, \sigma_w)$ with $Verify([PROPOSAL, w], \sigma_w)$.

Case 2: its proposal comes from the delivered $2f+1$ VIEW-CHANGE messages.

A VIEW-CHANGE message, encapsulates necessarily a value considered legitimate by at least $f+1$ correct processes by the quorum certificate.  The lemma holds by lemma \ref{lemma:sv-uniformity}.  
\end{proof}

\begin{lemma}[$O(n^2)$ complexity]\label{lemma:sv-complexity}
The communication complexity of the GroundWork algorithm is $O(n^2)$
\end{lemma}

\begin{proof}
Every correct process broadcast only one PROPOSAL message, one ECHO message and at most one JUSTIFICATION message where each message contains no more than ine threshold-signature and no more than share-signature.
\end{proof}

\begin{theorem}[Strong Validity]
 \namebis solves consensus with strong validity with $O(n^2)$ communication complexity. 
\end{theorem}

\begin{proof}
 The strong validity is ensured by lemma \ref{lemma:sv-validity}. The liveness of the algorithm is preserved by lemma \ref{lemma:sv-obligation}. The quadratic complexity is ensured by \ref{lemma:sv-complexity}
\end{proof}



\subsection{Drawbacks}

By synchronizing at each epoch only, the protocol suffers from some drawbacks that are discussed here.

\subsubsection{Clock Drift Tolerance}

Our model supposes that after GST, there is no clock drift, i.e. the real time is available to correct processes. It is legitimate to ask what happen if this assumption does not hold.
Let us investigate a less accomodating model where after GST, there exists a known bound $c > 1$ on clock drift. Without loss of generality, we assume that every correct process measures real time with a clock drift in $[1,c]$. Hence, if a correct process sets its timer to $c \cdot s$ seconds, when its timer expires, $s' \in [s, c \cdot s]$ real time seconds have elapsed.
The algorithm is slightly modified as follows: line 3 of algorithm 3 becomes $round\_timer$.measure$(k_{r} \cdot round\_duration$) where $k_{r}$ is an accurate coefficient, depending on round $r$ and clock drift bound $c$, to maintain the necessary and sufficient overlap of $8 \cdot \delta$ seconds at each round after first epoch synchronization after GST. In our case, setting $\forall r \in [1,f+1], k_{r} = c^{r}$ is necessary and sufficient to maintain the overlap (we fix $k_{0} = 0$). Indeed, for any $r \in [0,f+1]$, after $\tau_{r} = 2\delta + 10 \delta \cdot \sum_{i \in [1,r]} k_{i}$ real time seconds, the slowest process can enter in round $r+1$, while for any $r' \in [0,f]$, after $\tau'_{r'} = 10 \delta \cdot \sum_{i \in [1,r']} \frac{k_{i}}{c}$ real time seconds, the faster correct process can enter in round $r'+1$. To maintain the overlap, we want $\forall r \in [0,f]$, $\tau'_{r+1}- \tau_{r} \geq 8 \delta$. This lead us to $\forall r \in [0,f]$, $k_{r+1} \geq c +  (c-1) \cdot \sum_{i \in [1,r]} k_i $ and finally $\forall r \in [1,f+1]$, $k_{r} \geq c^{r}$ after an immediate induction. Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(10 \delta \cdot c^{f})$, while synchronizing at each round, like in \cite{NBMS19, NK20}, leads to a worst-case latency complexity of $O(10 \delta \cdot c)$.

\subsubsection{Adaptiveness a.k.a. early stopping}

It is valuable to obtain complexity which depends on the \emph{actual} number $t$ of Byzantine processes instead of a bound $f$ on this number $t$. This property called adaptiveness or early-stopping is not ensured by our protocol. Indeed, we can imagine a scenario $S$ where at GST, the correct processes are partitioned in 3 groups of $f$ processes that are respectively in round $1$, $2$ and $3$ of the same epoch $e_{max}$. Then they will perform $O(f)$ rounds of epoch $e_{max}$ before triggering the round synchronization of epoch $e_{max + 1}$ and eventually agree on a common value, leading to a worst-case latency complexity of $O(\delta \cdot f)$ (and a worst-case communication complexity of $O(f \cdot n)$) . In the same scenario $S$, a protocol that synchronize at each round, like in \cite{NBMS19, NK20}, will perform $O(t)$ rounds before agreeing on a common value , leading to a worst-case latency complexity of $O(\delta \cdot t)$ (and a worst-case communication complexity of $O(t^2 \cdot n)$) .

\subsubsection{expected complexity}

Our protocol is designed to optimize worst-case complexity only, but neglect expected complexity, where the adversary does not choose the Byzantine processes according to the order of leaders. Again, because of scenario $S$, the expected complexity is the same than the worst-case complexity, that is an expected latency complexity of $O(\delta \cdot f)$ and an expected communication complexity of $O(f \cdot n)$. In the same scenario, protocol from $\cite{NK20}$ synchronize a $O(1)$ expected number of times, with a $O(n)$ expected communication complexity per round synchronization, leading to a $O(\delta)$ expected latency complexity and a $O(n)$ expected communication complexity. 

\begin{table}[]
\begin{tabular}{|l|ll|ll|ll|}
\hline
Protocols  & \multicolumn{2}{l|}{Complexity with clock drift}                                                                                                                & \multicolumn{2}{l|}{Adaptative Complexity}                                                         & \multicolumn{2}{l|}{Expected Complexity}                                                           \\ \hline
           & \multicolumn{1}{l|}{Latency}                                                                                   & Communication                                  & \multicolumn{1}{l|}{Latency}                                         & Communication               & \multicolumn{1}{l|}{Latency}                                         & Communication               \\ \hline
This paper & \multicolumn{1}{l|}{$O(\delta \cdot f \cdot c^f)$} & $O(f \cdot n)$                    & \multicolumn{1}{l|}{$O(\delta \cdot f)$} & $O(f \cdot n)$ & \multicolumn{1}{l|}{$O(\delta \cdot f)$} & $O(f \cdot n)$ \\ \hline
\cite{NK20}       & \multicolumn{1}{l|}{$O(\delta \cdot f \cdot c)$}                    & $O(f^2 \cdot n)$ & \multicolumn{1}{l|}{$O(\delta \cdot t)$} & $O(t \cdot n)$ & \multicolumn{1}{l|}{$O(\delta)$}                        & $O(n)$                        \\ \hline
\end{tabular}
\caption{Comparison between our solution and state-of-art solution \cite{NK20}. The only improvement is for worst-case communication complexity where we reach the Dolev-Reischuk bound}. We also meet the optimal worst-case latency complexity when there is no clock drift after GST.
\end{table}

\subsection{The naive view increasing synchronizer}


For sake of completeness, we rewrite (in slightly more general manner)  the analysis of (naive) view doubling synchronizer \cite{NBMS19} that enables quadratic communication complexity but with costly latency complexity exponential with the number of faulty processes.

In this approach, each view has a timer, and if no progress is made the node moves to the next view and increases the timer time for the next view, where we note $\beta$ the arbitrary duration of the first view. The view duration has to increase indefinitely not only for being able to exceed the unknown $c \cdot \delta$ overlap time, but also for enable late processes, that were the last ones to start the protocol, to catch up the most in advance ones, without synchronization.

The duration of view $v$ is so $\beta 2^{v-1}$.


\begin{algorithm} 
\caption{View doubling synchronizer: Pseudocode for process $P_i$}
\label{algorithm:view-doubling-synchronizer}
\begin{algorithmic} [1]


\State \textbf{initialize} : 
\State \hskip2em $current\_view \gets 1$
\State \hskip2em $view\_duration \gets \beta$ \Comment{$\beta$ is predefined value for the duration of the first view}

\State \textbf{upon} timer expiration: 
\State \hskip2em $view\_duration \gets 2\cdot view\_duration$ 
\State \hskip2em $start(current\_view +1)$

\end{algorithmic}
\end{algorithm}

\paragraph{Latency complexity with known $\delta$ standing after unknown $GST$}

\paragraph{Latency complexity with unknown $\delta$, unknown $GST$}

Let $E_{max}$ be the the maximum epoch where a correct process is when the last correct process start the protocol. 
Let us compute the view $v_d$ of decision in worst case. This view appears $O(f)$ views after $v_o$ which is the first view where correct processes overlap for time $d = constant \cdot \delta$.







==> sections/drawbacks.tex <==
\section{Drawbacks}\label{section:drawbacks}

By synchronizing at each epoch only, the protocol suffers from some drawbacks that are discussed here.



\subsection{Adaptiveness a.k.a. early stopping} \label{subsection:adaptiveness}

It is valuable to obtain complexity which depends on the \emph{actual} number $b$ of Byzantine processes instead of a bound $f$ on this number $b$. This property called adaptiveness (or early-stopping for the latency) is not ensured by our protocol. Indeed, we can imagine a scenario $S$ where at GST, the correct processes are partitioned in 3 groups of $f$ processes that are respectively in view $1$, $2$ and $3$ of the same epoch $e_{max}$. Then they will perform $O(f)$ views of epoch $e_{max}$ before triggering the view synchronization of epoch $e_{max + 1}$ and eventually agree on a common value, leading to a worst-case latency complexity of $O( f)$ (and a worst-case communication complexity of $O(f \cdot n)$) . In the same scenario $S$, a protocol that synchronize at each view, like in \cite{ Naor2020}, will perform $O(b)$ views before agreeing on a common value , leading to a worst-case latency complexity of $O(
b)$ (and a worst-case communication complexity of $O(b^2 \cdot n)$) .

\subsubsection{expected complexity}\label{subsection:expected_complexity}

Our protocol is designed to optimize worst-case complexity only, but neglects expected complexity, where the adversary does not choose the Byzantine processes according to the order of leaders. Again, because of scenario $S$, the expected complexity is the same than the worst-case complexity, that is an expected latency complexity of $O(f)$ and an expected communication complexity of $O(f \cdot n)$. In the same scenario, protocol from $\cite{Naor2020}$ synchronize a $O(1)$ expected number of times, with a $O(n)$ expected communication complexity per view synchronization, leading to a $O(1)$ expected latency complexity and a $O(n)$ expected communication complexity. 

\subsection{Clock Drift Tolerance}\label{subsection:clock_drift_tolerance}

Our model supposes that after GST, there is no clock drift, i.e. the real time is available to correct processes. It is legitimate to ask what happen if this assumption does not hold. 
Let us investigate a less accomodating model where after GST, there exists a known bound $c > 1$ on clock drift. Without loss of generality, we assume that every correct process measures real time with a clock drift in $[1,c]$. Hence, if a correct process sets its timer to $c \cdot s$ seconds, when its timer expires, $s' \in [s, c \cdot s]$ real time seconds have elapsed.
The algorithm \ref{algorithm:synchronizer} is slightly modified as follows: line \ref{line:view_timer_measure_without_msg_exchange} of algorithm \ref{algorithm:synchronizer}  becomes $view\_timer_i$.measure$(k_{v} \cdot view\_duration$) where $k_{v}$ is an accurate coefficient, depending on view $v$ and clock drift bound $c$, to maintain the necessary and sufficient overlap of $\Delta$ time at each view after first epoch synchronization after GST. In our case, setting $\forall v \in [1,f+1], k_{v} = c^{v}$ is necessary and sufficient to maintain the overlap (we fix $k_{0} = 0$). Indeed, for any $v \in [0,f+1]$, after $\tau_{v} = 2\delta + 10 \delta \cdot \sum_{i \in [1,v]} k_{i}$ real time, the slowest process can enter in view $v+1$, while for any $v' \in [0,f]$, after $\tau'_{v'} = 10 \delta \cdot \sum_{i \in [1,v']} \frac{k_{i}}{c}$ real time, the faster correct process can enter in view $v'+1$. To maintain the overlap, we want $\forall v \in [0,f]$, $\tau'_{v+1}- \tau_{v} \geq \Delta$. This lead us to $\forall v \in [0,f]$, $k_{v+1} \geq c +  (c-1) \cdot \sum_{i \in [1,v]} k_i $ and finally $\forall r \in [1,f+1]$, $k_{v} \geq c^{v}$ after an immediate induction. Thus, if we want to tolerate clock drift after GST, synchronizing at each epoch only leads to a worst-case latency complexity of $O(10 \delta \cdot c^{f})$, while synchronizing at each view, like in \cite{Naor2020}, leads to a worst-case latency complexity of $O(10 \delta \cdot c)$.

\begin{table}[]
\begin{tabular}{|l|ll|ll|ll|}
\hline
Protocols  & \multicolumn{2}{l|}{Complexity with clock drift}                                                                                                                & \multicolumn{2}{l|}{Adaptative Complexity}                                                         & \multicolumn{2}{l|}{Expected Complexity}                                                           \\ \hline
           & \multicolumn{1}{l|}{Latency}                                                                                   & Communication                                  & \multicolumn{1}{l|}{Latency}                                         & Communication               & \multicolumn{1}{l|}{Latency}                                         & Communication               \\ \hline
This paper & \multicolumn{1}{l|}{$O( f \cdot c^f)$} & $O(f \cdot n)$                    & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ & \multicolumn{1}{l|}{$O(f)$} & $O(f \cdot n)$ \\ \hline
\cite{Naor2020}       & \multicolumn{1}{l|}{$O(b \cdot c)$}                    & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(b)$} & $O(b^2 \cdot n)$ & \multicolumn{1}{l|}{$O(1)$}                        & $O(n)$                        \\ \hline
\end{tabular}
\caption{Comparison between our solution and state-of-art solution \cite{Naor2020}. The only improvement is for worst-case communication complexity where we reach the Dolev-Reischuk bound}. We also meet the optimal worst-case latency complexity when there is no clock drift after GST.
\end{table}




==> sections/generalized_lower_bound.tex <==
\section{Generalized Dolev-Reischuk Bound}

Dolev-Reischuk lower bound~\cite{dolev1985bounds} claims that any Byzantine consensus protocol operating in a partially synchronous environment has $\Omega(f^2)$ communication complexity, where $f$ represents the number of tolerated Byzantine processes.
However, Dolev and Reischuk consider the Byzantine consensus problem satisfying \emph{strong validity:} if all correct processes propose the same value $v$, then only value $v$ can be decided by a correct process.
The question is whether the quadratic lower bound holds for Byzantine consensus problems satisfying some other variant of the validity property.
In this section, we define an attribute $\mathcal{A}$, which is defined as a set of executions, such that, if a partially synchronous Byzantine consensus protocol satisfies $\mathcal{A}$, then the Dolev-Reischuk lower bound applies to the protocol.

We fix $\Pi$, a Byzantine consensus protocol operating in a partially synchronous model (either $\mathcal{PS}_{\delta}$ or $\mathcal{PS}_{\mathit{GST}, \delta}$) among $n$ processes out of which  $0 < f < n$ can be faulty.
Protocol $\Pi$ satisfies the following properties:
\begin{compactitem}
    \item \emph{Termination:} All correct processes eventually decide.
    
    \item \emph{Agreement:} All correct processes decide the same value. \pierre{If we want to write agreement property as a safety property (that is not redundant with termination), we should write "no pair of correct processes disagree }
    
    \item \emph{Validity:} Some validity property. \pierre{(1)You meant some additional safety property ? } %\pierre{(2) Later, it seems to me that "very weak validity" is assumed, i. e. if all processes are correct and propose the same value $v \in \mathbb{V}$, then $v$ is the only value that can be decided, which seems weaker than $\mathcal{A}$, but I need to check first}
    
    %\pierre{(2) Another "hyper weak validity" could, i. e. if all processes are correct and propose the same value $v \in \mathbb{V}$, then $v$ is the only value that can be decided, which seems weaker than $\mathcal{A}$, but I need to check first}
\end{compactitem}
Let $\mathbb{V}$ denote the set of all values that can be proposed (and decided) in executions of $\Pi$.

Let us fix two disjoint groups of processes executing $\Pi$: (1) group $U$, where $|U| = n - \lceil f / 2 \rceil$, and (2) group $V$, where $|V| = \lceil f / 2 \rceil$.
For every value $v \in \mathbb{V}$, we define the set of executions $\mathit{execs}_{\Pi}(U, V, v)$ such that $e \in \mathit{execs}_{\Pi}(U, V, v)$ if and only if the following holds for $e$:
\begin{compactitem}
    \item All processes in the $U$ group are correct in $e$, whereas all processes in the $V$ group are faulty in $e$.
    
    \item No process in the $V$ group sends any message in $e$, i.e., these processes are silent in $e$.
    
    \item All processes in the $U$ group propose $v \in \mathbb{V}$ in $e$.
\end{compactitem}

We are ready to define when $\Pi$ satisfies attribute $\mathcal{A}$.

\begin{definition} [Satisfaction of attribute $\mathcal{A}$]
Protocol $\Pi$ \emph{satisfies attribute $\mathcal{A}$} if and only if there exist disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$, such that, for every value $v \in \mathbb{V}$ \pierre{I guess "for every value $v \in \mathbb{V}$" can be replaced by "for two different values $v, v' \in \mathbb{V}$" s. t. the result still holds with an even weaker attribute} and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, all correct processes decide $v$ in $e$.
\end{definition}

Intuitively, $\Pi$ satisfies $\mathcal{A}$ if and only if all correct processes decide the common proposed value in \emph{all} executions in which they propose the same value and faulty processes are silent.
Next, we prove that $\Pi$, a Byzantine consensus protocol satisfying $\mathcal{A}$, has $\Omega(f^2)$ communication complexity.

\begin{theorem} \label{theorem:generalized_dolev}
Let $\Pi$ be any Byzantine consensus protocol operating in a partially synchronous environment~\cite{dwork1988consensus} among $n$ processes out of which $0 < f < n$ can be faulty and let $\Pi$ satisfy $\mathcal{A}$.
The communication complexity of $\Pi$ is $\Omega(f^2)$.
\pierre{In fact we can say consensus protocol (non Byzantine) and $f$ processes can perform omission faults.} \jovan{Yes. But, I probably would not introduce that. It might introduce some confusion that is unnecessary. I would stick to Byzantine. What do you think?} \pierre{You are right. Perhaps at the end of the demonstration, we can mention that the "attack" from $U_i$ and $V$ used only omission faults.}
\end{theorem}
\begin{proof}
We fix a value $v \in \mathbb{V}$.
Let $e \in \mathit{execs}_{\Pi}(U, V, v)$ be an execution in which all correct processes (i.e., the processes in the $U$ group) propose and decide $v$.
By contradiction, suppose that correct processes send less than $(\lfloor f / 2 \rfloor)^2$ messages in $e$ (otherwise, the communication complexity of $\Pi$ would be $\Omega(f^2)$).
By the pigeonhole principle, there exists a process $P_i \in V$ that receives less than $\lfloor f / 2 \rfloor$ messages in $e$.
We denote by $U_i \subset U$ the set of correct processes that send messages to $P_i$ in $e$; note that $|U_i| \leq \lfloor f / 2 \rfloor$.

Now, we construct an execution $e'$ of $\Pi$:
\begin{compactitem}
    \item All processes in the $U \setminus{U_i}$ set are correct.
    Moreover, process $P_i$ is correct.
    
    \item Processes in the $V \setminus{\{P_i\}}$ set are faulty and silent, i.e., they do not send any message. 
    
    \item Processes in the $U_i$ set are faulty and behave exactly as they do in $e$, except that they do not send any message to $P_i$.
    
    \item Execution $e'$ is indistinguishable from $e$ to processes in the $U \setminus{U_i}$ set.
\end{compactitem}
Note that $e'$ has (at most) $f - 1$ faulty processes ($\lceil f / 2 \rceil - 1$ faults in the group $V$ and $\lfloor f / 2 \rfloor $ faults in the group $U$).
Moreover, all processes in the $U \setminus{U_i}$ set decide $v$ (since they do not distinguish $e'$ from $e$ until their decision).
Finally, $P_i$ does not receive any message in $e'$; moreover, $P_i$ decides $v$ in $e'$ (because of the termination and agreement properties satisfied by $\Pi$).

Lastly, we create an execution $e''$ in the following manner:
\begin{compactenum}
    \item We take an execution $e_{v'} \in \mathit{execs}_{\Pi}(U, V, v')$, where $v' \neq v$.
    
    \item We make process $P_i \in V$ correct.
    
    \item Messages sent by process $P_i$ are not received before processes in the group $U$ decide $v'$ (since $e''$ is indistinguishable from $e_{v'}$ to them).
    
    \item Messages sent to process $P_i$ are delayed until $P_i$ decides $v$ (since $e''$ is indistinguishable from $e'$ to $P_i$).
\end{compactenum}
Therefore, the agreement property is violated in $e''$.
We reach a contradiction with the fact that $\Pi$ solves the Byzantine consensus protocol, which concludes the proof of the theorem.
\end{proof}

We conclude the section by listing some noteworthy versions of the validity property which ensure that any Byzantine consensus protocol guaranteeing them satisfies attribute $\mathcal{A}$:
\begin{compactitem}
    \item Weak validity: If all processes are correct, then the value decided by a correct process was proposed by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing weak validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$; otherwise, there exists an execution in which (1) all processes are correct and all processes propose $v$, (2) messages from the group $V$ to the group $U$ are delayed, and (3) correct processes in the group $U$ decide a value different than $v$, which violates weak validity.
    
    \item Strong validity (variant 1): If all correct processes propose the same value $v$, then only value $v$ can be decided by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?} \pierre{Perhaps we can say that strong validity implies weak validity ?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing this version of validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since all correct processes have proposed $v$.
    
    \item Strong validity (variant 2): If a correct process decides a value $v$, then $v$ was proposed by a correct process.
    
    \emph{Why is $\mathcal{A}$ satisfied?} \pierre{Perhaps we can say that strong validity implies weak validity ?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing this version of validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since correct processes have proposed only $v$.
    
    \item External validity: Let the domain of the valid values be unknown.
    At the beginning of every execution, each correct process gets a value $v$ to propose accompanied with a proof $\sigma$ that $v$ is valid.
    Moreover, it is computationally impossible for a correct process to create a proof $\sigma'$ that some value $v'$ is valid, where $v'$ is not the proposed value of the process.
    Finally, if a correct process decides a value, then the value is accompanied by a proof that the value is valid.\footnote{External validity captures the validity property traditionally incorporated in blockchains in which each process proposes a block of (properly signed) transactions issued by clients.}
    
    \emph{Why is $\mathcal{A}$ satisfied?}
    Let $\Pi$ be any Byzantine consensus protocol guaranteeing external validity.
    We fix any two disjoint groups $U$ and $V$, where $|U| = n - \lceil f / 2 \rceil$ and $|V| = \lceil f / 2 \rceil$.
    For every value $v \in \mathbb{V}$ and every execution $e \in \mathit{execs}_{\Pi}(U, V, v)$, processes in the group $U$ must decide $v$ since correct processes do not ``discover'' any other valid value.
    Recall that a correct process is incapable of producing a proof for a non-proposed value and that a correct process cannot verify that a value is valid unless it obtains a proof for the value.
\end{compactitem}
If a Byzantine consensus protocol guarantees any of the aforementioned versions of validity, the protocol has $\Omega(f^2)$ communication complexity (by \Cref{theorem:generalized_dolev}).
In the case of $f = O(n)$, the communication complexity is $\Omega(n^2)$.

==> sections/intuition.tex <==
\section{Once Upon a Time $T$}

% (Later remove redundancies with introduction)
% Currently writing stream of consciousness, to be formatted later...

Most deterministic leader-based BFT consensus algorithms proceed in rounds.
In each round, processes collectively execute a \emph{round} sub-routine: one process acts as leader, the remaining processes act as followers and together they attempt to agree on a value.
If ``the stars align'', a value is agreed upon in this round and is then decided by every correct process.
This happens when i) the leader is correct and ii) all correct processes \emph{synchronously} execute the round for a sufficiently long period of time $T$, which depends on the specific algorithm being used.
Intuitively, this \emph{round} sub-routine can be regarded as its own abstraction solving a simpler version of the problem, with a weaker termination guarantee, i.e.:

\begin{compactitem}
    \item \emph{Good Case Termination:} If ``the stars align'', then all correct processes decide.
\end{compactitem}

Naturally, problems may occur. 
For any particular round the leader might be faulty (e.g. unresponsive) or the network might be behaving asynchronously if we are yet to reach GST.
Unfortunately, these two cases are indistinguishable: a leader's unresponsiveness can be due to the network being asynchronous and not its failure.
Worse, if the problem does lie in the leader, the round might not terminate irrespectively of how long correct processes execute it for (even if GST is reached).

The most widely adopted solution to potentially faulty leaders is to sequentially go through multiple rounds while changing the leader. % while ii) having all correct processes synchronized for $T$ time within each round.
After a round has been in execution without finishing for a long time ($>T$), the leader is suspected to be faulty and the round is aborted.
A new round is then started with a different leader.
\emph{Agreement} between rounds is ensured: if a correct process decides a value $v$ in some round that is aborted, no other correct process can decide anything but $v$ in any future round.
By cycling through all processes when choosing leaders, eventually a correct process will be picked.

\begin{figure}[htb]
    \centering
    \includegraphics[width=3.0in,height=1.0in]{example-image-a}
    \caption{Caption for image}
    \label{fig:sample_figure}
\end{figure}

Besides a correct leader, to ensure that a round is successful all correct processes must execute it synchronously, i.e. simultaneously and with a synchronous network, for a period of time $T$. This is called \emph{round synchronization}. After we reach GST, correct processes might be in very different states.


% Talk about: switching between leaders (i.e. ending/moving to the next round)
% ...We must abort rounds in which we suspect leaders to be faulty...
% Talk about: maintaining consistency between rounds
% ...A value might have been decided by other correct nodes during an aborted round, so Agreement must also be ensured between rounds...
% Talk about: eventually reaching a correct leader
% Talk about: maintaining correct processes synchronized during a round

%... As we go through leaders in a round-robin fashion, 

% With both these things, eventually the stars will align for a single round, which is when every correct process decides.
% The algorithm's latency and communication complexity are thus direct factors of i) the number of rounds it takes for this to happen, ii) the average time spent per round, and iii) the average communication complexity per round.



==> sections/unbounded_complexity_first_variant.tex <==
\section{Unbounded Communication Complexity Is Inherent In $\mathcal{PS}_{\delta}$}

In this section, we show that no Byzantine consensus protocol operating in $\mathcal{PS}_{\delta}$ exists with bounded communication complexity.
This result relies on the fact that no consensus protocol operating in $\mathcal{PS}_{\mathit{GST}, \delta}$ ensures bounded communication complexity before $\mathit{GST}$~\cite[Theorem 1]{spiegelman2021search}.

\begin{theorem} \label{theorem:unbounded_complexity_first_variant}
No Byzantine consensus protocol operating in $\mathcal{PS}_{\delta}$ exists that can tolerate a single failure and guarantee bounded communication complexity even in failure-free executions.
\end{theorem}
\begin{proof}
By contradiction, let there exist a Byzantine consensus protocol $\Pi$ operating in $\mathcal{PS}_{\delta}$ such that (1) $\Pi$ can tolerate a single failure, and (2) $\Pi$ has bounded communication complexity $X$ across all failure-free executions.
Next, we construct a Byzantine consensus protocol $\Pi'$ that operates in $\mathcal{PS}_{\mathit{GST}, \delta}$ by making $\Pi'$ behave in the same way as $\Pi$ in every execution.

$\Pi'$ solves the Byzantine consensus problem since $\Pi$ does so.
Moreover, for every failure-free execution $\alpha'$ of $\Pi'$, there exists the identical failure-free execution $\alpha$ of $\Pi$: if the maximum message delay in $\alpha'$ is $D$, then there exists the execution of $\Pi$ in which $\delta = D$ and all processes behave as in $\alpha'$.
Given that $\Pi$ has bounded communication complexity $X$ across all failure-free executions, $\Pi'$ has bounded communication complexity across all failure-free executions.
This contradicts Theorem 1 presented in~\cite{spiegelman2021search}, which concludes the theorem.
\end{proof}

\Cref{theorem:unbounded_complexity_first_variant} proves that it is inevitable to have unbounded communication complexity in solving the Byzantine consensus protocol in $\mathcal{PS}_{\delta}$.
Therefore, we turn our focus to the alternative variant $\mathcal{PS}_{\mathit{GST}, \delta}$ of the partially synchronous model.
\pierre{I think we have to stress, that it is not true if the unknown $\delta$ can be considered as a constant. Typically, the version of HotStuff where each correct process enters in a new view after timeout where the timer is increased exponentially has a communication complexity of $O((f+1+log_2(\delta))\cdot n)$ in $\mathcal{PS}_{\delta}$}


